Man-at-the-End Software Protection as a Risk Analysis Process

The last years have seen an increase of Man-at-the-End (MATE) attacks against software applications, both in number and severity. However, MATE software protections are dominated by fuzzy concepts and techniques, with security-through-obscurity omnipresent in the field. This paper presents a rationale for adopting and standardizing the protection of software as a risk management process according to the NIST SP800-39 approach. We examine the relevant aspects of formalizing and automating the activities in this process in the context of MATE software protection. We highlight the open issues that the research community still has to address. We discuss the benefits that such an approach can bring to all stakeholders. In addition, we present a Proof of Concept (PoC) of a decision support system that automates many activities in the risk analysis methodology towards the protection of software applications. Despite still being a prototype, the PoC validation with industry experts indicated that several aspects of the proposed risk management process can already be formalized and automated with our existing toolbox, and that it can actually assist decision making in industrially relevant settings

==> attack.tex <==
\begin{itemize}
    %\item useless intro
    %\item security requirements description (maybe move into intro/requirements chapter)
    \item brief description of attack paths/trees (refs to attack trees theory + other security applications)
    \item difficulties (i.e. why coarse attack steps = backward programming combinatorial explosion + no way to automatically model actual attack steps)
    \item general work-flow of attack finder + description
\end{itemize}

%This chapter presents the risk assessment method used by \esp to infer possible attacks against the application assets in the vanilla application, \ie the unprotected program. As detailed in Section~\ref{sec:esp:workflow:model}, \esp, prior to this phase, executes a preliminary analysis of the source code, enriching the \ekb with the description of the application structure, instancing the related meta-model classes described in Section~\ref{sec:model:app}. The risk assessment phase employs this information, in order to infer attacks tailored to the specific application examined. Each attack aims to breach a security requirement of an application asset; these are provided by the user, annotating the application source code as detailed in Section~\ref{sec:esp:impl:solDep}.

%The definition of security requirements stem from the \nist guide to risk management \cite{nistSP800-39}, which defines the \textit{confidentiality} and the \textit{integrity} of assets. In this thesis, two new additional requirements are introduced, in order to adapt to the application security scenario.

%\esp supports three security requirements for assets: \textit{confidentiality}, \textit{integrity}, \textit{execution correctness}. A confidential asset must not be understandable by an attacker: this is the case for example of an algorithm that must remain secret, in order to safeguard the software company IP, or of a data structure that holds personal information of the user, such as the credit card number in an e-commerce application. The integrity requirement specifies that an asset must not be modifiable by an attacker: for example, in the case of a soccer video-game, the variables holding the characteristics of the soccer players, or the match score, can be marked with the integrity requirement, in order to avoid an attacker to cheat. The execution correctness requirement is a stronger form of integrity for code: the latter must not be modified, but must also be called as expected by other functions. For example, an attacker that wants to remove a license check function, marked with this requirement, may modify the function in order to not perform the check, but can also avoid the function to be executed, removing any calls by other functions to the license check one.

%
%Weak confidentiality is a particular case of the previous requirements, breached when the attacker is able to get a datum value in every moment of the application execution. For example, e-banking websites typically employ a two-factor authentication: to access its account, and every time it executes a security-sensitive operation (\eg a money transfer to another bank account), the user must not only provide its credentials, but also a \otp, valid only to authorize a single operation. \glspl{otp} are typically generated either using a hardware dongle, or with a mobile application. In the second case, the \otp is generation is based on a pre-shared secret among the mobile application and the e-banking server, and on a factor that changes every time a new \otp is requested by the user: for example, a counter that is incremented every time a new \otp is generated. An attacker, which has already stolen the access credentials of a user, may be interested in being able to generate such passwords at will, hacking the \otp generator. Even in the most simple case, when the attacker wants to access the e-banking account, and then transfer all the money to its account, the attacker needs to obtain two \glspl{otp}: one to access
%
%Some data may be also tagged
%with the weak confidentiality property. This property is breached when the attacker
%is able to retrieve the datum at every moment of the application execution
%(thus for hard-coded data the weak confidentiality is the same as the normal
%confidentiality). This is mostly interesting for attacks that target the assets of a
%victim’s application (i.e., not the attacker’s copy) by means of a distributed approach
%aiming at continuously obtaining the data values. For instance, in case of
%an OTP (One-Time Password) generator1 that generates the next password by
%hashing the value of a fixed seed and a counter modified at each generation, the
%variable storing the counter can be marked with weak confidentiality. To predict
%the next passwords (not only the next one), it does not suffice that the attacker
%obtains once the value of victim’s counter, he has to obtain it just before every
%generation. Therefore, either he is able to access every time the victim’s application to read the counter value, or he has to obtain one counter, understand
%the counter update function, and reproduce it on his copy.
%

%\esp models attacks against such security requirements with \textit{attack paths}, which are sequences of simple tasks that an attacker may execute (\eg locating a variable in the binary, debugging a function at run-time), called \textit{attack steps}: this modelling approach has already been used by other works in literature for risk assessment of computer networks \cite{ekelhart,fenz}. Each attack step is associated with a set of postconditions, which model the result of a successful execution by the attacker of the simple task related to the step, and a set of preconditions, which must be fulfilled by the results of other steps preceding it in the path. Attack steps may contain also preconditions about the application structure: for example, an attack step modelling the debugging of a function, can be executed only if the analyzed asset is a code and not a variable.
%Attack steps are modeled as Horn clauses \cite{hornClauses} (see Section~\ref{sec:background:expSys:inf}), and are stored in the \ekb as rules written in the Prolog language.

%\esp, to infer the possible attack paths against the asset security requirements of the target application, relies on an external inference engine, where attack steps are modelled as logical rules. At the start of the risk assessment phase, \esp instructs the engine about the structure of the application, modelling each concept of the application meta-model (see Section~\ref{sec:model:app}) as an axiom, \ie a fact that engine knows to be true. Then, \esp queries the engine, for each asset security requirement, to prove that the attacker can breach it: to do this, the engine tries to find every possible chain of rules (\ie a sequence of attack steps forming an attack path), which can be ultimately proven with a subset of the aforementioned axioms about the application structure. The engine carries out this task using a backward programming algorithm (see Section~\ref{sec:background:expSys:inf}). Other works in literature \cite{ou,kagal} have already used a similar approach to assess risk for computer networks. To ease readability, in the remainder of this chapter attack steps and axioms are expressed with the mathematical proofs notation. 

%The attack steps are modelled with the following inference rules:
% \begin{equation*}
% \infer[id,]{C}{P}
% \end{equation*}
% Where:
% \begin{itemize}
% 	\item $id$ is the name that identifies the attack step;
% 	\item $P$ is a set of facts, called \emph{premises}: if these facts are verified, the attack step can be executed by the attacker;
% 	\item $C$ is a set of facts, called \emph{conclusions}: these facts will be verified if the attack step can be carried out by the attacker.
% \end{itemize}

% The user can influence the time needed to infer the possible attack steps with two parameters. First, he or she can set a hard time limit (expressed in seconds). Also, he or she can decide a limit for the backward programming algorithm, in term of number of traversed relationships among application parts (\eg the maximum distance among application parts in the call graph), when the algorithm is searching for an attack step that, with its conclusions, can satisfy a premise of another attack step.

% Finally, the attack paths are saved in the \esp \ekb, structured using the related classes described in the meta-model (Section~\ref{sec:model:att}). The attacks are then used in the risk mitigation phase of \esp: during the latter, the protections best suitable to protect the application assets, against the attack paths previously found by the inference engine.

% This chapter is a reworked version of the publication ``Towards Automatic Risk Analysis and Mitigation of Software Applications'' \cite{reganoProlog}. It is organized in the following sections:

% \begin{itemize}
% 	\item Section~\ref{sec:prolog:app} describes the preliminary of the application structure modeling in the inference engine, previously obtained by \esp parsing the source code;
% 	\item Section~\ref{sec:prolog:goals} defines the rules needed to model the attacker goals;
% 	\item Section~\ref{sec:prolog:att} details the methodology for modelling attack steps, and how the inference engine combines them in attack paths;
% 	\item Section~\ref{sec:prolog:risk} reports on the method used to assess the risk of the inferred attack paths;
% 	\item Section~\ref{sec:prolog:validation} contains a comparison of the obtained results \wrt the \esp requisites defined in \ref{sec:esp:problem}.
% \end{itemize}

%At the start of the risk assessment phase, the \esp models all the information regarding the application structure in form of Prolog axioms, \ie facts that the engine consider true by definition. Then, the \esp queries the engine to find, for each asset security requirement, a sequence of rules (\ie attack steps) that, given the aforementioned axioms, can prove the breach of an asset security requirement. Attack paths will thus start with an attack step having only preconditions on the applic

%given the aforementioned axioms, to infer all the possible logical sequences of rules that can lead to the


\subsubsection{Application structure modeling}
\label{sec:prolog:app}

\begin{itemize}
    \item application, code, datum facts
    \item relationships facts (containment, call graph)
    \item asset + security requirements facts
\end{itemize}

% This section presents the modelling of all the preliminary information needed by the inference engine to find possible attacks against the application, comprising assets with their security requirements and the application structure. All this information is automatically retrieved by \esp in the preliminary source code analysis phase of its workflow.

% First, the existence of an application $a$ is defined with the following fact:
% \begin{equation*}
% \infer{application(a)}{}
% \end{equation*}
% Then, the application structure must be formally modelled. Each basic component of the code can be either a code or a datum (a constant or a variable); for example, if the application $a$ contains a function $f$ and a global variable $d$, this can be modelled with the following facts, using by abuse of notation the symbol $\rhd$ to indicate the containment relationship:
% \begin{equation*}
% \infer{code(f)}{} \quad \infer{datum(d)}{} \quad \infer{f \rhd a}{} \quad \infer{d \rhd a} {}
% \end{equation*}
% The containment relationship permits to organize the application structure in a hierarchical way. For example, if the function $c$ contains a local variable $v$, and a code snippet $s$, we can define the function structure with the following facts:
% \begin{equation*}
% \infer{datum(v)}{} \quad \infer{\rhd f}{} \quad \infer{code(s)}{} \quad \infer{\rhd f}{}
% \end{equation*}
% Then, a code $c$ accessing a variable $v$ can be expressed with the following fact:
% \begin{equation*}
% \infer{accesses(c,v)}{}
% \end{equation*}
% Also the call graph of the application can be modelled; if a function $f_1$ containing a call to a function $f_2$, the following fact holds:
% \begin{equation*}
% \infer{calls(f_1,f_2)}{}
% \end{equation*}
% Finally, the assets and their security requirements must be defined. If the \esp user requests the confidentiality security requirement \infer{\confidentiality}{} for a function $f_1$, integrity \infer{\integrity}{} for a function $f_2$ , and execution correctness \infer{\excorr}{} for a function $f_3$, the following facts are asserted:
% \begin{equation*}
% \infer{code(f_1)}{} \quad \infer{code(f_2)}{} \quad \infer{code(f_3)}{} \quad
% \infer{\confidentiality(f_1)}{} \quad \infer{\integrity(f_2)}{} \quad \infer{\excorr(f_3)}{}
% \end{equation*}

\subsubsection{Attacker goals modeling}
\label{sec:prolog:goals}

\begin{itemize}
    \item goal = breach asset security requirement
    \item basic rules to reach breaching of each of 3 sec. req.
\end{itemize}

% After modelling the application structure, and the assets with their security requirement, the basic rules that define the goals of the attacker can be defined. \esp, for each asset security requirement, will query the inference engine to find a set of rules that lead to breaching the requirement, denoted formally as the logical negation of the requirement. For example, if the application contains a variable $v$ whose confidentiality must be safeguarded, the inference engine will try to find all the possible sequences of attack steps that lead to the following outcome, which is a goal $G$ of the attacker:
% \begin{equation}
% \neg \confidentiality(v) \iff G.
% \end{equation}

% Security requirements are characterized by the different ways in which the attacker can breach them. The confidentiality of an asset $a_1$ is breached if the attacker finds a way to retrieve its content (instructions if $a_1$ is a code, or data if $a_1$ is a variable): 
% \begin{equation*}
% \infer{\neg \confidentiality(a_1)}{contentRetrieved(a_1)}
% \end{equation*}
% The integrity of an asset $a_2$ is breached if the attacker manages to change it, modelled with the following rules:
% \begin{equation*}
% \infer{\neg \integrity(a_2)}{changed(y)}
% \end{equation*}
% To model the breaching of execution correctness, two rules are needed. Formally, the attacker breaches the execution correctness of a code, either by modifying its instructions, or by avoiding the execution of the code, removing at least one call to the function. Thus, if a function $f$ is marked with the execution correctness requirement, the latter can be modelled with the following rules:
% \begin{equation}
% \infer{\neg \excorr(f)}{changed(f)} \quad \infer{\neg \excorr(f)}{calls(g,f) & changed(g)}
% \end{equation}
% With the definition of the following facts in the inference engine, \esp informs the latter of the application structure and of the security requirements of the assets. Thus, the attacks able reach the attacker goals, \ie to breach the security requirements of the assets, will adapt to the application structure.

\subsubsection{Attack steps and paths modeling}
\label{sec:prolog:att}

\begin{itemize}
    \item just 1 example of attack tree building
    \item ref to more complex examples in SPRO+WISTP papers
    \item brief description of actual implementation
    \item complexity analysis
\end{itemize}

% This section elaborates on the formal modelling of attack steps, basic and indivisible tasks that an attacker may carry out, and that can be combined into complete attack paths against the application assets. 

% %For the purpose of this section, it is sufficient to mark each attack step with a general id $AS$, to distinguish them from regular inference rules. Indeed, this distinction is important for the \esp: attack steps identify actions executed by the attacker, which can be deferred in the risk mitigation phase, while regular rules are simple inferences used to connect logically attack steps together, but with no use in the aforementioned phase. Also, when presenting inferred attack paths to the user, including normal inferences would result in unnecessary clutter that would complicate user comprehension of the paths.

% First, a set of basic attack steps must be defined. First, the attacker may retrieve the content of a hard-coded asset $h$, \eg a constant or a set of instructions, by locating it in the binary, and inspecting the latter manually:
% \begin{equation*}
% \infer[statLocate(h)]{contentRetrieved(h)}{hardcoded(h)}
% \end{equation*}

% Conversely, the attacker may retrieve the instructions constituting a code asset $c$ at run-time, for example by means of step-by-step execution with a debugger, provided that the execution flow of the application can lead to the target code. Similarly, an attacker can read the value of a local variable $v$ locating it in memory at run-time. This leads to the following attack steps:
% \begin{equation*}
% \infer[dynLocate(c)]{contentRetrieved(c)}{code(c)}
% \end{equation*}
% \begin{equation*}
% \infer[dynLocate(v)]{contentRetrieved(v)}{datum(v) & v \rhd f }
% \end{equation*}

% If an attacker wants to locate a datum $d$ to retrieve its value, he may try to first identify and execute at run-time a function $f$ that uses the aforementioned datum, thus finding it in memory when the instruction of the function $f$ that accesses the datum $d$ is executed:
% \begin{equation*}
% \infer[dynLocate(d)]{contentRetrieved(d)}{code(c) & contentRetrieved(c) & accesses(c,v)    }
% \end{equation*}
% Also, if an attacker wants to locate a function $f$, and he or she has already retrieved a function $g$ that calls $f$, then by simply following the call, looking at the target address of the call instruction, he or she can retrieve the function $f$ in the binary:
% \begin{equation*}
% \infer[followCall(g,f)]{contentRetrieved(f)}{calls(g,f) & contentRetrieved(g)}
% \end{equation*}
% Thus, if such datum $d$ is a confidential asset, one of the possible attack paths, leading to the attacker goal $G$ of breaching $d$ confidentiality can be obtained by chaining the previous attack steps:
% \begin{equation*}
% \infer{G}{
% 	\infer{\neg \confidentiality(d)}{
% 		\infer[dynLocate(d)]{contentRetrieved(d)}{
% 			\infer[statLocate(c)]{contentRetrieved(c)}{\infer{hardcoded(c)}{\infer{code(c)}{}}} & \infer{accesses(c,v)}{}
% 		}
% 	}
% }
% \end{equation*}
% % In this example, the attacker first identifies the address of the function $c$ in the code section of the application binary, analyzing statically the latter. Indeed the $statLocate(c)$ attack step can be executed, because $c$, being a code, is hard-coded. Then he or she attaches a debugger to the application and sets a breakpoint at the address of the function $c$ previously located. Then, since the code $c$ accesses the variable $v$, by executing $c$ step-by-step the attacker is able to find the variable $v$ when $c$ accesses it, and thus, knowing $v$'s location in memory, can retrieve its content. Therefore, the confidentiality of the asset $d$ is breached, and the attacker goal $G$ is proved. Clearly, instead of this hybrid approach (\ie by resorting to both static and dynamic analysis), the attacker can breach $d$ confidentiality in a completely dynamic manner, finding the code $c$ observing the execution flow of the application. Similarly, the call graph of the application can be used to define other attack steps. For example, an attacker may locate a function $f_1$ at run-time, if he has previously located a function $f_2$ that calls $f_1$, and the function is executed.

% % For tampering attacks two types of attack steps may be modelled. As for the retrieval of content, tampering may be carried out statically only on hard-coded assets, while it can be executed dynamically on every kind of asset. Given a code or datum $x$, the attacker may change it statically or dynamically with the following attack steps, which require the attacker to know the location of $x$:
% % \begin{equation*}
% % \infer[statChange(x)]{changed(x)}{contentRetrieved(x) & hardcoded(x)} 
% % \end{equation*}
% % \begin{equation*}
% % \infer[dynChange(x)]{changed(x)}{contentRetrieved(x)}
% % \end{equation*}

% % Thus, attack paths that endanger the integrity and execution correctness security requirements of an asset can be obtained by chaining the steps required to locate the asset that must be tampered, and the steps in which the attacker actually tamper with the asset. Given a function $f$ whose execution correctness must be preserved, \ie $f$ must not be tampered with, and all the calls to $f$ must be executed, this attacker goal $G$ can be obtained with the following two example attack paths:
% % \begin{equation*}
% % \infer{G}{
% % 	\infer{\neg \excorr(f)}{
% % 		\infer{calls(g,f)}{} & \infer[statChange(g)]{changed(g)}{  \infer[statLocate(g)]{contentRetrieved(g)}{\infer{hardcoded(g)}{}}      }
% % 	}                            
% % }
% % \end{equation*}
% % \begin{equation*}
% % \infer{G}{
% % 	\infer{\neg \excorr(f)}{
% % 		\infer[dynChange(f)]{changed(f)}{\infer[followCall(g,f)]{contentRetrieved(f)}{\infer{calls(g,f)}{} &
% % 				\infer[statLocate(g)]{contentRetrieved(g)}{\infer{hardCoded(g)}{}}
% % 		}}
% % 	}
% % }
% % \end{equation*}
% % In the first attack path, the attacker first locates the function $g$. He can do it statically since $g$ is hard-coded. Then he or her changes it, removing from $g$ the call to the asset $f$. In this way, the execution correctness of $f$ is broken. In the second attack path, the attacker locates statically the function $g$ as before, but in this case uses its address to set a breakpoint in a debugger attached to the application. For example, this can be useful in the case of an indirect call, when the target address of the call (\ie the address of $f$) is not known a priori, since it is evaluated by the program at run-time. Thus, he will execute the application, which will stop at the breakpoint set at the start of function $g$. With an execution step-by-step of the function $g$, the attacker finds the call to function $f$, follows it an then retrieves the address of the address function, thus being able to change the contained instructions and breach the execution correctness of the asset $f$.

% % Thus, starting from apparently naive attack steps, the inference engine can combine them in rather complex attack paths. All the concept and relationships among them, modelling the application structure, are obtained automatically by \esp, thus these attack paths can be obtained in a completely automated fashion, with the users asked only for the security requirements of the assets.

% Other attack steps have been devised to model attacks on applications that include network connections in their execution flow, modelling sniffing, spoofing and remote code injection attacks. However, these attack steps cannot be employed in a completely automated workflow by \esp, since it would require the identification of the specific functions that perform such network activity. This is complicated to do automatically, especially if the application uses custom network libraries. Since the requirements for \esp (see Section~\ref{sec:esp:problem}) state that all workflow phases must be executed automatically, such network-based attack steps are not deemed relevant for the scope of this thesis. Still, use of the spoofing attack step to model attacks against an \otp generator has been reported in a conference publication \cite{basileOTP}.

% The chaining of the rules is executed by the inference engine via a custom backward programming algorithm, called by \esp for each asset security requirement. Given this goal, the algorithm starts by negating the asset security requirement and then finds all the possible attack steps that can lead to the asset security requirement negation: each parallel attack step leads to a separate attack path. Then, it goes on building all the possible paths: for each of the latter, the algorithm consider completely inferred a path when the last attack step requirements can be proved only with the axioms detailing the application. Therefore, \esp builds for each asset security requirement an attack graph, which contains four different attack paths to breach the execution correctness of a code $c_2$, which is called by another function $c_1$.

% %as the one depicted in Figure~\ref{fig:attackGraph}\footnote{The avoidedCalls fact has been added to the graph to ease comprehension, but would not be present in a real attack path.},
% %\tikzstyle{Function} = [rectangle,rounded corners,draw=black, top color=white,
% %bottom color=white!50,very thick, inner sep=0.4em, minimum size=1.5em, text
% %centered]
% %\tikzstyle{Variable} = [rectangle,draw=black, top color=white, bottom
% %color=white!50,very thick, inner sep=0.4em, minimum size=1.5em, text centered]
% %\tikzstyle{myarrow} = [->, >=latex', shorten >=1pt, thick]
% %\tikzstyle{mydashedarrow} = [->, >=latex', shorten >=1pt, dashed]
% %\tikzstyle{mythickarrow} = [->, >=latex', shorten >=1pt,line width=0.6mm]
% %\tikzstyle{mylabel} = [text width=7em, text centered]
% %
% %\begin{figure}[t]
% %\centering
% %\begin{tikzpicture}[node distance=0.3cm, auto]
% %\node [Function] (breached) {breached(executionCorrectness,$c_2$)};
% %\node [Function, above right = of {$(breached)+(+0.6,+0.5)$}]
% %(changedC2)
% %{changed($c_2$)};
% %\node [Variable, above right = of {$(changedC2)+(+1.5,-0.1)$}]
% %(statChC2)
% %{statChange($c_2$)};
% %\node [Variable, right = of {$(statChC2)+(+1.511,0)$}]
% %(statLocC2)
% %{statLocate($c_2$)};
% %\node [Variable, below right = of {$(changedC2)+(+1.5,+0.1)$}]
% %(dynChC2)
% %{dynChange($c_2$)};
% %\node [Variable, right = of {$(dynChC2)+(+1.511,0)$}]
% %(dynLocC2)
% %{dynLocate($c_2$)};
% %\node [Function, below right = of {$(breached)+(-0.4,-0.4)$}]
% %(avoided)
% %{avoidedCalls($c_2$)};
% %\node [Function, below right = of {$(avoided)+(-0.6,-0.4)$}]
% %(changedC1)
% %{changed($c_1$)};        
% %\node [Variable, above right = of {$(changedC1)+(+1.5,-0.1)$}]
% %(stChC1)
% %{statChange($c_1$)};
% %\node [Variable, right = of {$(stChC1)+(+1.511,0)$}]
% %(statLocC1)
% %{statLocate($c_1$)};
% %\node [Variable, below right = of {$(changedC1)+(+1.5,+0.1)$}]     
% %(dynChC1)
% %{dynChange($c_1$)};
% %\node [Variable, right = of {$(dynChC1)+(+1.511,0)$}]
% %(dynLocC1)
% %{dynLocate($c_1$)};
% %
% %\draw[mydashedarrow] ($(avoided.north)+(-0.1,0)$) --
% %(breached.south);    
% %\draw[mydashedarrow] (changedC1.north) -- (avoided.south);    
% %\draw[mydashedarrow] (changedC2.south) -- (breached.north);    
% %\draw[myarrow] (dynChC1.west) --
% %($(changedC1.east)+(-0.08,-0.2)$);
% %\draw[myarrow] (stChC1.west) --
% %($(changedC1.east)+(-0.08,+0.2)$);\draw[myarrow]
% %(dynChC2.west) --
% %($(changedC2.east)+(-0.08,-0.2)$);
% %\draw[myarrow] (statChC2.west) --
% %($(changedC2.east)+(-0.08,+0.2)$);
% %\draw[mythickarrow] (statLocC2.west) -- (statChC2.east);
% %\draw[mythickarrow] (dynLocC2.west) -- (dynChC2.east);
% %\draw[mythickarrow] (statLocC1.west) -- (stChC1.east);
% %\draw[mythickarrow] (dynLocC1.west) -- (dynChC1.east);
% %
% %\end{tikzpicture}
% %\caption{Attack graph built against the execution correctness of a code $c2$, which is called by the code $c1$.}
% %\label{fig:attackGraph}
% %\end{figure}

% %\subsection{Network attack steps}
% %\label{sec:prolog:network}
% %This section models two additional attack steps, modelling sniffing and spoofing attacks, thus being suitable to assess threats on applications that, during their execution, communicate with a remote server. For example, e-banking websites typically employ a two-factor authentication: to access its account, and every time it executes a security-sensitive operation (\eg a money transfer to another bank account), the user must not only provide its credentials, but also a \otp, valid only to authorize a single operation. \glspl{otp} are typically generated either using a hardware dongle, or with a mobile application. In the second case, the \otp is generation is based on a pre-shared secret among the mobile application and the e-banking server, and on a factor that changes every time a new \otp is requested by the user: for example, a counter that is incremented every time a new \otp is generated. An attacker, which has already stolen the access credentials of a user, may be interested in being able to generate such passwords at will, hacking the \otp generator. 
% %%
% %To help with the modelling of this network attack steps, the \otp example is used throughout the section, thus is needed to describe its execution flow. At the first installation on the e-banking service user device, the \otp generator downloads two random values from the server, using an encrypted connection: a \textit{seed} and a \textit{counter}. Then, every time the user requests a new \otp, the generator asks a \pin to the user, so that unauthorized users having gained access (\eg stealing) to the device running the generator can obtain access to the e-banking account of the user. If the \pin inserted is correct, the generator produces the \otp, with a method based on the values of the aforementioned seed and counter, which is known to both the application and the e-banking server; thus, the \otp inserted by the user when accessing the e-banking site can be validated against the \otp produced on the server with the same method and the same values of seed and counter. After the generation of the \otp, the counter is incremented both on the generator and on the server, and a new \otp can be produced. 



\subsubsection{Risk probability}
\label{sec:prolog:risk}

\begin{itemize}
    \item evaluation of risk of each attack path on unprotected application
    \item useful for expert manual assessment of proposed L1P solution
    \item not used by automatic risk mitigation phase (since risks are on unprotected app)
    \item formulas (already present on WISTP paper, maybe just a ref is sufficient)
\end{itemize}

% In this section, a method to assess the probability of the threats against the application assets is presented. \esp, when presenting the attack paths to the user, includes also such a  probability: this is useful for experts that want to manually analyze the protections inferred by \esp in the risk mitigation phase, since they can identify the assets that are most at risk, and consequently focus on the protections targeting the most threatened assets.

% Instead, it will not be used to drive the risk mitigation phase (see Section~\ref{sec:l1p:metrics:score}): the motivation behind this is that the probabilities inferred in this phase refer to the unprotected application, while the risk mitigation phase uses a set of formulas tailored to assess the effect of attacks on protected assets, to assess the effectiveness of the inferred mitigations.

% The risk probability is based on the types of attacks inferred, and on the presumed skills of the attacker, given the profile chosen by the user at the start of the \esp workflow. Given all the inferred attack paths \(AP_{i}\), all their attack steps \(AS_{i,j}\), and all the assets \(a_{k}\), the \emph{risk} $\Omega_{\mathrm{AP}_{i}}^\epsilon$ of an attack path \(AP_{i}\) executed by an attacker with expertise $\epsilon$ is defined as:
% \begin{equation*}
% \Omega_{\mathrm{AP}_{i}}^\epsilon = \pi(\mathrm{AP}_{i},\epsilon)\;\Gamma_{\mathrm{AP}_{i}}\;\label{eq:risk}
% \end{equation*}
% where $\Gamma_{\mathrm{AP}_{i}}$ represents the damage resulting from a successful attack path, and  $\pi({\mathrm{AP}_{i}},\epsilon)$ is the probability of an attacker being able to successfully carry out the attack path, given its expertise $\epsilon$. To do so, it must be able to execute all the attack steps needed to complete it. Thus, the probability of executing an attack path is evaluated taking into account the probabilities of all the attack steps constituting the path:
% \begin{equation*}
% \pi({\mathrm{AP}_{i}},\epsilon) = f\left(\pi({\mathrm{AS}_{i,1}},\epsilon),\pi({\mathrm{AS}_{i,2}},\epsilon),\dots\right).
% \end{equation*}
% The \esp user can decide the function $f$ that must be used to combine the probabilities of the attack steps belonging to the same path, choosing among a worst case analysis, with $f=min$, a best case analysis, with $f=max$, and an approximation of the probabilities composition, with $f=\cdot$.

% $\Gamma_{\mathrm{AP}_{i}}$ is a quantitative measure of the damage resulting from a successful attack path. It is evaluated as the sum of the damage $\Gamma_{\mathrm{AS}_{i,j}}$ from each attack step:
% \[
% \Gamma_{\mathrm{AP}_{i}} = \sum_j \Gamma_{\mathrm{AS}_{i,j}}= \sum_j \sum_{k} ( W_{a_{k}} b( a_{k},\mathrm{AS}_{i,j}) )
% \]
% %where $\Gamma_{\mathrm{AS}_{i,j}}$  is the cost of a single attack step
% where \(W_{a_{k}}\) is a user-defined asset weight, and \(b( a_{k},\mathrm{AS}_{j})\) is a function, evaluated by \esp, that returns the fraction of the security properties of the asset \(a_{k}\) that are breached by the attack step \(\mathrm{AS}_{j}\), that is, it returns \(1\) if all the security properties are compromised and \(0\) if none\footnote{Thus, the whole asset weight assigned by the user is gained by the attacker when all the security properties are compromised.}.
% %\(b( a_{k},\mathrm{AS}_{j})\) is .

% The attack step probabilities $\pi({\mathrm{AS}_{i,j}})$, for each combination of attack step type, and level of attacker skill, have been obtained during the \asp project, interviewing the software security experts involved in the project during \esp design phase.


% %
% %The \esp employs a worst case analysis, setting $f=min$, thus the probability of an attack path is approximated as the one of the most easy attack step. 
% %
% %$\Gamma_{\mathrm{AP}_{i}}$ is a quantitative measure of the damage resulting from a successful attack path, calculated as the sum of the damage $\Gamma_{\mathrm{AS}_{i,j}}$ from each attack step:
% %
% %\[
% %\Gamma_{\mathrm{AP}_{i}} = \sum_j \Gamma_{\mathrm{AS}_{i,j}}= \sum_j \sum_{k} ( W_{a_{k}} b( a_{k},\mathrm{AS}_{i,j}) )
% %\]
% %%where $\Gamma_{\mathrm{AS}_{i,j}}$  is the cost of a single attack step
% %where \(W_{a_{k}}\) is the user-defined asset weight, and \(b( a_{k},\mathrm{AS}_{j})\) is a function, deduced by our inference system, which returns the fraction of the security properties of the asset \(a_{k}\) that are breached by the attack step \(\mathrm{AS}_{j}\), which is, it returns \(1\) if all the security properties are compromised and \(0\) if none\footnote{In practice, we assume that the whole asset weight assigned by the user is gained by the attacker when all the security properties are compromised.}. Finally, the values obtained with the risk formulas are mapped on a three values score (low, medium, high) with an ad hoc mapping.

\subsubsection{Validation}
\label{sec:prolog:validation}

\begin{itemize}
    \item cite requirements, why they are solved and why we are so cool
\end{itemize}

% In this section, the methodologies presented in this chapter, used by \esp to infer possible attack paths against the application assets, are compared \wrt the \esp requisites listed in Section~\ref{sec:esp:problem}.

% Regarding the requisites on the usage scenario of \esp, detailed in Sec.~\ref{sec:esp:problem:framing}, they are satisfied by the risk assessment phase. First, the profile of the attacker is taken into account, when the risk of each attack path is evaluated. Second, the execution of the backward programming algorithm used by the inference engine can be constrained, using a hard time limit, and also setting a maximum length for the attack paths: a deeper and more time-consuming search is suitable prior to the distribution of the application, while, when patches are released and time is an issue, a shallow search for possible new attack paths derived from the introduction of the patch code can be performed, limiting the time needed using the aforementioned constraints. Third, the results of the mitigation phase, \ie attack paths, are easily readable, being modelled as ordered sequences of simple attack steps: furthermore, logical inferences that do not correspond to real tasks executed by the attacker are not included in the paths, to avoid confusion for the user. Furthermore, a risk level for each inferred attack path is presented to the \esp user, which can easily identify the most problematic threats to the application.

% Analyzing the requisites for the risk assessment phase, described in Sec.~\ref{sec:esp:problem:assessment}, they are mostly satisfied. First, \esp supports not only the security requirements defined by the \nist for risk monitoring \cite{nistSP800-39}, \ie confidentiality and integrity, but also a stronger form of the latter, called execution correctness, and applicable only to functions: this security requirement prescribes that the function marked with it must not only be preserved from modification, but it must be also called as originally devised by the application developer (\eg a license check that must not be circumvented). Furthermore, \esp is able to build attack graphs for every asset in the application, due to the definition of logical inference rules that define attack steps, \ie simple attacker tasks. The chaining of these steps in attack paths is subject to the application structure, which is automatically modelled with logical facts in the inference engine: thus, the relative requirement is satisfied. Finally, a probability of execution for each attack path is evaluated, based on the attacker skills, and the probability of execution of each attack step: the latter are based on information gathered among the software security experts involved in the \asp project. The complexity metrics of the software are not taken into account in the attack path probability evaluation: however, they are taken into account later in the \esp workflow, during the risk mitigation phase, when the effectiveness of the inferred protections in protecting the assets, against the attack path inferred in the risk assessment phase, is tested with a game-theoretic approach based on this metrics.

% Finally, in the validation phase of \esp at the end of the \asp project \cite{D1.06.9}, software security experts analyzed also the attack paths inferred in the risk mitigation phase. In particular, the ones inferred by \esp on the \asp use cases (see Section~\ref{sec:esp:results}) were compared with actual attacks executed by highly skilled white-hat hackers on the same test applications. In general, \esp attack paths covered the real methodologies of the aforementioned hackers. However, they were deemed as too general to model with a sufficient amount of detail such attacks. Indeed, new rules can be added to the inference engine, in order to better model real attacks on software: however, as in the case of network-related attacks, the main problem is inferring automatically the semantics of the code that enables the execution of such complex attack step. Thus, this is still an open problem, which the author is actively investigating, in particular focusing on automated binary exploitation frameworks \cite{angr, huang}, which could be used to actually assess the vulnerabilities of the applications in an automated manner. Their results could be still modelled as attack paths, thus being compatible with the remainder of the workflow.

==> contributions.tex <==
model of assets, attacks, protections, security properties, etc.
and their dependencies
to find attack paths and suitable protections
game theoretic algorithm to identify solutions
heuristics to prune the search space
backward reasoning to find attack paths
already declared in publications
evaluation models to estimate impact of attack paths and protections
metrics composition
metrics change estimation after protections
L2P
Minor
integration with the ACTC
GUI
reports that are validated by experts


==> discussion.tex <==
threats to validity/limitations/validation vs. requirements for each workflow step

\begin{itemize}
\item Knowledge base
\item Risk assessment
\begin{itemize}
    \item discuss why we analyze the vanilla version
    \item difficulties (i.e. why coarse attack steps = backward programming combinatorial explosion + no way to automatically model actual attack steps)
    \item validation vs. requirements
\end{itemize}
\item Asset protection: ref to analogous subsection in section IV
\item Asset hiding
\begin{itemize}
        \item excessive AH may decrease AP solution security level
        \item overhead
        \item AH refines a AP solution thus all AP difficulties also apply to AH
\end{itemize}
\end{itemize}

==> l1p.tex <==
\begin{itemize}
    \item useless intro
    \item talk about the difficulties (PI precedences, PI limitations, overheads, keep sec. properties, PI order matters, \dots)
    \item talk about what you need into the KB
    \item solution in two steps: find the suitable deployed PIs, find the right order (solution)
    \item general work-flow of L1P + description
\end{itemize}

%This chapter presents how \esp is able to assess the effectiveness of mitigations against the risks on application assets. \esp combines different protection techniques, such as the ones presented in Section~\ref{sec:background:softProt}, in a comprehensive \textit{protection solution}, able to safeguard a given application against possible attacks that can endanger its assets. This task is typically carried out manually, by software protection experts, that analyzes the application source code, reason on the possible attacks that can be carried out against the application assets, and decide the most suitable protection techniques to block the attacks. This decision is mainly based on their knowledge and past experience in the software protection field.

%Indeed, this is not an easy task, even for an expert. First, there are various possible security requirements for an asset, and there does not exist one protection able to preserve all of them: for example, code obfuscation techniques (Section~\ref{sec:background:softProt:antiRevEng:codeObf}) are able to preserve the confidentiality of a protected function or code region\footnote{A code region is a section of a function that is syntactically valid if parsed in isolation; a formal definition of code regions is provided in Section~\ref{sec:l2p:milp:app}.}, but are not capable of blocking attacker attempts to tamper with them, which is the scope of anti-tampering protections (Section~\ref{sec:background:softProt:antiTamp}). Also, the applicability of a protection is limited to one type of asset: different techniques are necessary to protect code areas or the values of variables and constants. Attackers have a broad range of tools at their disposal, such as debuggers, automatic code analysis tools, disassemblers and decompilers, leading to a plethora of different types of attacks, and, again, one protection cannot block all of them: thus, a simple mapping between protections and enforced security requirements is clearly not enough, and a set of protections must be applied to each asset in order to block all the possible attacks endangering its requirements. Another problem is assessing the real effect of a protection technique, when applied on a specific function or variable, in increasing the difficulty of executing possible attacks against them: again, a simple mapping between protections and blocked attacks is not sufficient, since the effectiveness of protections may vary in function of the structure of the code on which they are applied. For example, the effectiveness of \cff is directly related to the number of basic blocks in the \cfg of the protected code, since each basic block can be put in a different case of the \cff loop, leading to a wide \cfg difficult to analyze for an attacker. \todo{works in literature on empirical assessment}

%Furthermore, combining different protections techniques is a process that must be carried out with extreme care, and even the order in which the protections are applied to the same asset can have a beneficial or detrimental effect on the obtained security. For example, if \cff is applied on a function that has been previously protected with opaque predicates, the latter become more difficult to be removed, since the two branches introduced by each opaque predicate will be put in different cases of the \cff loop: on one hand, this increases the parallel cases of the flattened \cfg, hardening its analysis, while on the other hand identifying that the two branches pertain to the same opaque predicates takes more effort for the attacker, since this correlation is not evident anymore in the \cfg; however, this effect is not obtained if the opaque predicates are inserted on a code already flattened, since each of them will be inserted in one of the \cff cases, without having their branch split. A case of combination that ultimately leads to an application not working at all is the deployment of any kind of obfuscation after remote attestation (Section~\ref{sec:background:softProt:antiTamp:RA}): since the latter monitors attested code in order to find any attempts of tampering with it, the modifications introduced by an obfuscation technique will be mistaken for a tampering attack, triggering a reaction, for example the abrupt termination of the application. Therefore, all the possible interactions among used techniques must be taken into account when protecting an asset.

%When protections techniques are combined, also the relationships among assets must be taken into account. A simple example can be a whole function whose integrity must be preserved, which contains a sub-routine that should remain confidential: while theoretically these two assets can be seen as separated, having different security requirements, this containment relationship must be taken into account to avoid incompatible combinations of protections; taking again the example above, if the whole function integrity is protected with remote attestation, and afterwards the confidentiality of the contained code region is ensured with some kind of obfuscation, the remote attestation checks will be triggered and the application will not work. 

%Finally, it should also be noted that protections usually take a toll on application performances: an example is the anti-debugging technique (Section~\ref{sec:background:softProt:antiDeb}), which prevents an attacker from launching a debugger, by actually debugging the protected areas of code with a custom debugger out of the attacker control. However, a context switch is necessary every time the execution flow enters a protected code, thus slowing the application. Also, on-line techniques (Section~\ref{sec:background:softProt:antiTamp}) need to exchange data over the Internet, in order to communicate with their server counterpart: if this communication is executed across unreliable networks, such as the one used by mobile phones, this may lead to a slow-down of the application, for example if the application is protected with code mobility (Section~\ref{sec:background:softProt:antiTamp:codeMobility}) and the code needed to continue the execution is not downloaded on time; also, if the user of the mobile application has a limited data plan for his phone, this may lead to undesirable charges by the mobile ISP. Thus, when choosing the protections, the overhead introduced by them in the application must be taken into account, with the protected application that must be thoroughly tested after deployment of protections: this may lead to various time-consuming cycles of protection and testing, until the wanted trade-off between security and usability of the application is found.

%Summarizing, when protecting an application, an holistic approach is necessary: structure of the application and of the assets that must be protected, security requirements that must be preserved, possible attacks that can endanger them, the pros and cons of the available protection techniques, and the interactions among them must all be taken into account, in order to obtain an application that is secure, trying to leave user experience untouched. With this approach in mind, a set of algorithms have been devised to automate this cumbersome process, with the rather ambitious goal of modelling the mental processes of an expert in the act of protecting an application. The automated workflow may be useful for software security experts in protecting applications, presenting them with a protection solution they can further refine instead of starting from scratch, but also for software developers, allowing them to protect their applications without being versed in software security.

% Using a \emph{divide and conquer} approach, this complex problem has been subdivided into two smaller ones, each solved by a different \esp component:
% \begin{itemize}
% 	\item the identification of the protections that are able to protect an asset security requirement, being capable of blocking at least one attack endangering the requirement; this problem is solved by the \eape;
% 	\item the inferral of protection solutions for the target application, able to safeguard all the security requirements of all the assets comprised in the application, leaving the business logic of the application untouched, and avoiding to introduce too much overhead in the application execution; the algorithms automating this process are comprised in the \eapd.
% \end{itemize}

% This reasoning processes are a fundamental part of the \esp workflow, enabling it to infer the a-posteriori classes of the protection meta-model detailed in Section~\ref{sec:model:prot}, and ultimately leading to the individuation of the most suitable combination of protections that, if deployed on the program source code with the \esd, is able to safeguard the user-defined security requirements of a target application assets. To correctly infer the suitable combination for a specific target application, the \eape and \eapd need a \ekb containing the following information:
% \begin{itemize}
% 	\item generic software protection knowledge gathered from software protection experts, \ie the a-priori information in the software protection meta-model presented in Chapter~\ref{sec:model};
% 	\item a list of assets and security requirements, manually specified by the target application developer, either by annotating the code as presented in Section~\ref{sec:esp:impl:solDep}, or using the \eui;
% 	\item a user-defined set of maximum application performance overheads (see Section~\ref{sec:l1p:metrics:overhead}) that a solution can cause after being deployed on the target application with the \esd;
% 	\item structure and software metrics of the unprotected application source code, obtained respectively from the automatic analysis executed by the \esca via \cdt (Appendix~\ref{sec:esp:impl}) and the \emf via the \actc (Section~\ref{sec:l1p:metrics}), \ie a completely inferred application meta-model (Section~\ref{sec:model:app});
% 	\item \APs discovered by the \ebad against user-defined assets security requirements, \ie a completely inferred attack meta-model (Section~\ref{sec:model:att});
% 	\item optionally, a set of user-defined constraints to avoid the evaluation of all possible solutions by the \eapd: the user can specify a time limit, or a maximum number of evaluated solutions.
% \end{itemize}

% This section presents the workflow followed by \esp to infer appropriate protection solutions for a target application: each solution is associated with a score, which indicates the effectiveness in slowing an attacker executing the \glspl{ap} previously built by the \ebad. Among the found solutions, the best ones will be shown to the \esp user\footnote{The number of solutions shown to the \esp user can be set by him or her in the \eui.}, so that he or she can select one of them to be deployed on the application code via the \esd, which will produce a binary protected with the \glspl{dpi} comprised in the chosen solution.

% Figure~\ref{fig:l1pWorkflow} depicts the aforementioned workflow, highlighting the involved \esp components, along with calls among them, the meta-model objects they use, and the meta-model classes inferred in the various steps of the workflow (indicated with a circled red number), which are the following:
% \begin{enumerate}
% 	\item \esp calls the \eape which, for each specific asset security requirement (also called \PO) previously defined by the user, enumerates the \PIs that can defer at least one of the \APs that endanger the \PO, thus building and saving in the \ekb a set of \DPIs for each \PO;
% 	\item \esp calls the \eapd: in the following workflow steps, its two sub-components, the solution walker and the solution solver, will find the protection solutions, \ie combinations of \DPIs found in the previous steps, which will be shown to the user in the last workflow step; this step is further detailed in Section~\ref{sec:l1p:eape};
% 	%    \item the walker calls the \emf to predict the metrics on the analyzed solution (without actually deploying the latter on the target application, as described in Section~\ref{sec:l1p:metrics:prediction}), in order to evaluate the overheads of the solution; if one or more of them exceed the user-defined overhead limits, the solution, albeit correct, is deemed not feasible, and the workflow go back to the previous step; otherwise, the solution is considered feasible and is saved in \ekb;
% 	\item the \eapd calls its first sub-component, the solution solver;
% 	\item the solution solver calls the solution walker, which reads from the \ekb the previously built \DPIset, and generates a solution (\ie a subset of \DPIs from the aforementioned set, organized in an ordered sequence of \DPIs) that is both correct and effective, \ie if deployed on the target application, produces a protected binary that behaves correctly during execution, and protects all the \POs in the application; this reasoning process is presented in Section~\ref{sec:l1p:walker}; then, the walker returns the solution to the solver;
% 	\item each time the walker generates a valid solution, the solver calculates the score of such solution with a game-theoretic approach detailed in Section~\ref{sec:l1p:solver}, using the metrics predicted by the \emf and the \APs inferred by the \ebad; then, if all the possible solutions have been evaluated, or if at least one of the user-defined conditions for \eapd termination has been met (\eg maximum execution time or number of evaluated solutions), the solution solver terminates, otherwise another solution is asked to the walker (\ie the workflow returns to step 4);
% 	\item having added the inferred solutions to the \ekb, the \eapd can halt its execution, returning control to \esp;
% 	\item \esp gathers the inferred solutions from the \ekb, and presents them to the user.
% \end{enumerate}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=\linewidth]{images/l1pWorkflow.pdf}
% 	\caption{\esp protection decision process, with main software protection meta-model classes and \esp components involved in the process.}
% 	\label{fig:l1pWorkflow}
% \end{figure}

% When presented with the inferred solutions, the user can select one of them and can alternatively:
% \begin{itemize}
% 	\item deploy the selected solution on the target application, obtaining the protected binary: in this case, \esp will call the \esd, described in Appendix~\ref{sec:esp:impl:solDep};
% 	\item further refine the chosen solution with additional protections on non-asset \APs, in order to increase the effort needed by the attacker to locate the protected assets; with this choice, \esp will give the selected solution in input to the \ehal, presented in Chapter~\ref{sec:l2p}.
% \end{itemize}

\subsection{Enumerating the deployed protection instances}

\begin{itemize}
    \item useless intro
    \item detail on what info is stored in the KB for the PIs/protections
    \item how the DPIs are mapped/found (what are the constraints)
    \item tell that the DPIs are added to the KB, ready for the next phase
\end{itemize}

% This section details the internal processes of the \eape, corresponding to step 2 of the protection decision workflow (Section~\ref{sec:l1p:workflow}). The main task of this component is instancing in the \ekb the \DPIs that can safeguard one or more security requirements of an asset in the target application. In general, given a \PO, \ie the security requirement of a specific asset, the \eape infers that deploying the considered \PI on the aforementioned asset can be useful if (as specified by the expert a-priori knowledge in the \ekb) the protection implemented by the \PI is in general able to safeguard the \PO security requirement: in this case, a new \DPI is instanced in the \ekb, related to the asset and \PI taken into account.

% First of all, the \eape needs to enumerate the \PIs available in the system running \esp. As detailed in Section~\ref{sec:model:prot}, a \PI represents a specific protection technique implementation, stating the tool that must be used to deploy the technique, along with its configuration parameters: for example, the remote attestation technique may be deployed by \esp using the \asp implementation of such technique (Section~\ref{sec:background:softProt:antiTamp:RA}), specifying the algorithm that must be used to compute the hashes of attested regions (\eg Blake, SHA1). In particular, the \eape parses a set of \xml files, contained in the \ekb source code folder (see Appendix~\ref{sec:esp:impl}), specifying for each \PI:
% \begin{enumerate}
% 	\item the \PI name;
% 	\item the name in the \ekb of the implemented protection;
% 	\item the name in the \ekb of the protection tool that must be used by the \esd to deploy the protection (\eg Tigress or \actc);
% 	\item the protection tool parameters values characterizing the \PI; for protections deployed by the \actc, this is represented by the related \asp annotation (see Section~\ref{sec:esp:impl:solDep}), while for Tigress techniques implementation the options that must be included in the command line\footnote{As specified in the section \emph{"Options"} for each transformation page in the Tigress website; for example, \url{http://tigress.cs.arizona.edu/transformPage/docs/flatten/index.html\#options} lists the command-line options for the flattening transformation.};
% 	\item the formulas to compute the introduced overhead if the \PI is deployed on a \CR, depending on the metrics of the latter (see Section~\ref{sec:l1p:metrics:overhead}).
% \end{enumerate}

% The parsed \PIs are therefore saved in the \ekb: the user can disable one or more \PIs, using the \eui. Note that \PIs are not hard-coded in the \PIs as a-priori information, in order to ease the addition of other \PIs by the user, which simply needs to add a new \xml file (or edit an existing one) adding the requested information for the new \PI. For example, this is useful to drive \diablo, since it has a parameter that specifies the percentage of basic blocks to which the binary code obfuscations (Section~\ref{sec:background:softProt:antiRevEng:codeObf}) must be applied: a higher value for this parameter means a more thorough obfuscation, at the expense of an increased overhead. The default \xml file contains a set of \PIs for each binary code obfuscation, with different values for this parameter: however, a user can edit the related \xml file easily to specify its set of parameter values.

% Subsequently, the \eape can infer the \DPIs that are suitable to protect an application, and that must be considered by the \eapd when finding the possible protection solutions; for each \PO, a \DPI, representing the deployment of the \PI on the asset constituting the \PO, is added to the \ekb if:
% \begin{itemize}
% 	\item from the a-priori expert knowledge in the \ekb, the protection technique implemented by the \PI enforces the \PO security requirement;
% 	\item the \PI is applicable to the considered asset type; for example, Tigress variable obfuscation (Section~\ref{sec:background:softProt:antiRevEng:dataObf}) is applicable only to integer variables;
% 	\item specific requirements of the considered \PI are fulfilled; for example, the \asp implementation of code mobility (Section~\ref{sec:background:softProt:antiTamp:codeMobility}) can be applied exclusively to whole functions, so, if an asset is only a region of a function, the \eape builds a \DPI related to the \CR representing the whole function comprising the asset.
% \end{itemize}

% Also, the user can set the following constraints to limit the number of \DPIs inferred by the \eape, such as a minimum \class{Level} that a \class{Mitigation} of a \class{Protection} must have to be deemed useful in deferring an \AP. Finally, the \DPIs fulfilling the aforementioned requirements and user-defined constraints are added to \ekb, and will be considered by the \eapd for inclusion in the produced protection solutions, as reported in the following sections.

\subsection{Evaluating the states}
% \label{sec:l1p:metrics}

\begin{itemize}
    \item useless intro
    \item describe the attacker/defender model
    \item what is a state? (solution + list of attacks)
    \item we use SW metrics for evaluating the state scores and overheads: intro metrics + table with all the metrics
    \item intro to Collberg's potency
    \item describe the evaluation formula (uncertainty, remote instructions, alteration detection/avoidance + how to asses attacks impact + when an asset is broken?)
    \item how to estimate metrics/overheads without building everything: neural networks + STM paper
\end{itemize}

% This section provides insights on the evaluation of software complexity metrics done by the \emf, and their subsequent use by the \eapd. Software metrics can be defined as an ``attempt to quantify aspects of a software system'' \cite{encyclopediaSoftEng}: in particular, complexity metrics try to grasp the difficulty of carrying out tasks on software, for example maintenance, debugging, testing or applying modifications \cite{softwareComplexity}. Indeed, one of those tasks can be attacking a software: therefore, increasing the complexity of a protected program is a desirable result. There are various  attempts in literature to leverage complexity measures in order to assess a protection efficacy in defying attacks on a given function or code snippet: a notable example is the \emph{potency}, defined by Collberg in \cite{collberg1997taxonomy}, which is a measure of effectiveness for code obfuscation techniques (see Section~\ref{sec:background:softProt:antiRevEng:codeObf}). Given an obfuscation technique $\tau$ that, when applied to a specific program $P$, produces an obfuscated version $P^\prime$ of the latter, the potency $\tau_{pot}(P)$ of $\tau$ in protecting $P$ against reverse engineering can be evaluated with the following formula:
% \begin{equation}
% \tau_{pot}(P)=\frac{E(P^\prime)}{E(P)}-1
% \end{equation}
% Where $E(P)$ is a complexity measure evaluated on the original program $P$, and $E(P^\prime)$ is the same measure computed on the obfuscated program $P^\prime$. Indeed, an obfuscation technique is effective when $E(P^\prime)>E(P)$, since it produces a more complex program that is more difficult to reverse engineer by an attacker \wrt the original application. In the aforementioned paper, Collberg proposes seven complexity measures (\eg size of the program, nesting level of conditional and looping constructs) to evaluate the potency of a transformation; other appropriate measures have been proposed by Tonella \etal in \cite{tonellaPoster} (\eg call graph and data dependency graph size).

%Besides the qualitative relations that we need to model between
%protections and attacks, it is also useful to model the relation quantitatively where possible.
%This can facilitate more accurate evaluations of the strength of protections given
%an application, its assets, and potential attacks. In literature, many metrics to measure
%that strength have already been proposed. For example, software complexity metrics
%have been proposed to quantify the potency of obfuscations, i.e., the extent with which
%obfuscations make manual code comprehension tasks and automatic de-obfuscation
%techniques harder [13, 14, 15]. Other authors have proposed combining many different
%metrics for assessing the strength of a wider range of protections [16, 17, 18] or have
%evaluated which metrics are better predictors of obfuscation quality [19].
%
%In order to assist the security expert to estimate the effectiveness of such solutions, the concept
%of potency introduced by Collberg et al. [13] can be used. The potency is essentially
%a value stating how good the security of a protected asset is based on the value of
%selected software metrics. In his work, Collberg proposed the use of seven static and
%dynamic metrics. Since metrics need to be measured on the protected asset, evaluating
%the potency of a protection over a specific asset means that the protection needs to be
%actually applied, the program possibly rebuilt and some complexity metrics needs to
%be extracted by an ad-hoc tool. This process can be time-consuming, especially if the
%application is big and/or if the number of candidate solutions to choose from is high.
%To avoid the actual application of protections, we developed an estimator that uses a set
%of neural-networks trained to predict, with a high degree of accuracy, the variations of
%the metric values used to compute the potency. Therefore, with this tool a defender is
%able to accurately estimate the potency of a solution starting only from the unprotected
%assets’ complexity metrics without rebuilding the application each time [31].

% As elaborated in Section~\ref{sec:l1p:metrics:score}, the \eapd leverages the concept of potency to evaluate the effectiveness of a solution in countering the attacks inferred by the \ebad. To evaluate metrics on the unprotected binary involved in the solution assessment, as already reported in Section~\ref{sec:esp:impl:arch}, the \emf relies on \diablo: such metrics on the unprotected program are obtained by calling \diablo via the \actc, without applying any protection. 

% The remainder of this section is organized as follows:

% \begin{itemize}
% 	\item Section~\ref{sec:l1p:metrics:metrics} lists the metrics evaluated by the \emf on the target application and on its functions;
% 	\item Section~\ref{sec:l1p:metrics:prediction}, mainly derived from the publication ``Estimating Software Obfuscation Potency with Artificial Neural Networks'' \cite{reganoMetric}, explains how the \emf predicts values assumed by a function or snippet metrics after the deployment of a specific sequence of protections, without actually applying such transformations to the code;
% 	\item Section~\ref{sec:l1p:metrics:overhead} presents how the \eapd, when generating a solution, estimates the impact of chosen protections on the target application performances, should the assessed solution be deployed on the application;
% \end{itemize}

% \subsubsection{Software protection complexity metrics}
% \label{sec:l1p:metrics:metrics}

% \esp supports 21 complexity metrics, as reported in Table~\ref{table:esp:metrics}. \diablo can analyze a binary to calculate metrics on the whole application and for each \CR: for \esp, especially the latter kind of metrics are interesting, \eg to evaluate the effectiveness of a protection applied to a specific asset, taking into account how the asset metrics are changed by the assessed protection. Among those metrics, 18 express generic information about code complexity, while the other five metrics are devised to express the result of specific protections after their deployment to the evaluated code. Also, depending on whether the evaluation of the metrics involves running the program, the following three types of metrics can be identified:

% \begin{itemize}
% 	\item static metrics: computed without executing the binary;
% 	\item dynamic coverage metrics: computed executing the binary, identifying the basic blocks executed, and considering only them in the evaluation of the metrics;
% 	\item dynamic size metrics: computed as the coverage metrics, but taking also into account the number of time each basic block is executed.
% \end{itemize}

% \begin{table}
% 	\begin{tabular}{lllll}
% 		\toprule
% 		\Center{Metric} & \Center{Protection} & \Center{Static} & \Center{Dyn. Size} & \Center{Dyn. Coverage} \\
% 		\midrule
% 		No. of assembler instructions & All & Yes & Yes & Yes \\
% 		No. of source operands & All & Yes & Yes & Yes \\
% 		No. of destination operands & All & Yes & Yes & Yes \\
% 		\acrfull{hl} & All & Yes & Yes & Yes \\
% 		No. of edges in the \cfg & All & Yes & Yes & Yes \\
% 		\acrfull{cc} & All & Yes & Yes & Yes \\
% 		Control flow indirection metric & All & Yes & Yes & Yes \\
% 		No. of mobile blocks & Code mobility & Yes & No & No \\
% 		Total size of mobile basic blocks & Code mobility & Yes & No & No \\
% 		Size of attestation data & Remote attestation & Yes & No & No \\
% 		No. of attested basic blocks & Remote attestation & Yes & No & No\\
% 		Size of attested basic blocks & Remote attestation & Yes & No & No\\
% 		\bottomrule
% 	\end{tabular}
% 	\caption{Software complexity metrics supported by \esp.}
% 	\label{table:esp:metrics}
% \end{table}

% Unfortunately, at the time of writing, \esp supports only static metrics to evaluate the overhead and the protection level introduced by the deployment of a \PI on a specific \CR or datum in the target application. A first problem for the use of dynamic metrics is that, for \diablo being able to evaluate dynamic metrics, an example use case of the application is needed from the user: it should resemble as much as possible the expected usage of the application by its users, and should be specified in the \actc configuration file. \esp is currently not able to automatically infer the inputs needed for executing the target application: theoretically, it would be possible to integrate in \esp a fuzzer to execute the application various time, and subsequently compute an average of the obtained dynamic metrics; however, there is no guarantee that this random input execution would summarize the typical application usage. This first problem could be nonetheless partially solved by tasking the \esp user to manually specify a use case in the \actc configuration file. A second problem and still not completely solved, is that, to obtain the metrics of a protected code, the solution must be actually deployed, obtaining the protected binary, so that \diablo can be launched on it to compute the metrics: this involves applying the protection and compiling the code every time the overhead and the score of a solution must be evaluated: this, especially for large application, cannot be done in a reasonable time, since the number of solutions can be high and the time needed to compile the application is not negligible. Furthermore, the evaluation of dynamic metrics involves the execution of the protected application: again, is not feasible to execute the application every time a solution must be assessed. A partial solution to this problem, presented in Section~\ref{sec:l1p:metrics:prediction}, is the use of a machine learning approach to estimate the metrics of the protected application, instead of evaluating them via an actual deployment of the protections. However, this approach has been proved effective only to predict static metrics, thus \esp, at least for now, bases its reasoning processes only on static metrics; however, as detailed in Section~\ref{sec:esp:results}, this limitation has not impeded \esp to perform well in protecting real applications.

% In the following, details about the specific metrics used are given, starting from protection-independent ones. The \emph{number of assembler instruction} indicates the actual size in the binary corresponding to a \CR: for example, this information is useful to indicate the amount of code that an attacker should analyze to understand an asset that should remain unintelligible. The total \emph{number of source and destination operands} represent the amount of different register, memory locations and constants that are respectively read or written by the code: these metrics give another measure of the code complexity, since, to comprehend a code, an attacker should understand the purpose of all the operands involved in the code execution. \acrfull{hl} \cite{halstead} is the arithmetic sum of the three preceding metrics. 

% Other interesting complexity metrics can be evaluated taking into account the analyzed \CR \cfg. A first measure is the \emph{number of edges} comprised in the aforementioned graph, since it corresponds to the number of jumps comprised in the examined code, which should be taken into account when trying to reconstruct the code flow to comprehend its purpose. Similarly, McCabe's \acrfull{cc} \cite{mccabe} measures the number of linearly independent paths, from each entry point to each exit point, in the analyzed \CR: each path represent a possible different execution of the \CR, which an attacker must analyze to ultimately understand the code. Another metric computed on the \cfg is the \emph{control flow indirection metric}: it measures the number of indirect edges in the \cfg, \ie the number of jumps whose target is evaluated at run-time as a result of previous calculation in the code (\eg a jump with the target address in memory written in a \cpu register), thus being difficult to be evaluated by an attacker without executing the program.

% Regarding protection-dependent techniques, \esp supports five of them. Two are related to the code mobility technique (see Section~\ref{sec:background:softProt:antiTamp:codeMobility}), and measure the amount of code that is moved to the server, measured either in \emph{number of basic blocks} or in Bytes (\emph{Total size of mobile basic blocks}): since this code is not available in the binary, being download with a per-needed basis at run-time, these metrics indicate the amount of code the attacker will be able to analyze only during execution. The last three metrics are related to remote attestation, an on-line anti-tampering technique described in Section~\ref{sec:background:softProt:antiTamp:RA}. The \emph{size of attestation data} indicates the size of the attestation measurements evaluated by the technique on the protected code: it has little use for security purposes, but is indeed useful to evaluate the increase in application memory usage caused by the deployment of this technique. The remaining two metrics measure the amount of code monitored by the technique, indicating the amount of code, expressed either as a \emph{number of attested basic block} or with the total number of Bytes monitored (\emph{size of attested basic blocks}): this measures are interesting from a security point of view, since they express the amount of code that an attacker cannot tamper with, without the technique identifying such changes and executing the proper reaction to modification.

% \subsubsection{Complexity metrics prediction}
% \label{sec:l1p:metrics:prediction}
%When evaluating the effect of a protection solution, both \eapd and \ehal need to make calculations based on metrics of the \CRs protected by the solution: it is needed in particular to evaluate the solution score (see Section~\ref{sec:l1p:metrics:score} for the score calculated by the \eapd) and the overhead introduced by the solution (see Section~\ref{sec:l1p:metrics}).
%
%Obviously, the \emf can evaluate such metrics by actually applying the solution to the code via the \esd, and subsequently obtaining the metrics on the protected code by calling \diablo via the \actc, as it does for the unprotected code metrics: this means compiling the program to obtain the binary on which the static metrics must be evaluated. The \emf is tasked to do so every time a solution is evaluated; however, all the metrics on all the \CRs could be obtained with the above method, testing each  possible combination (setting a maximum length) of protections by applying it an all the application \CR. Given a program $P$, and a number $n_{pi}$ of \PIs (see Section~\ref{sec:model:prot}) supported by \esp, the time $t_{test}(n_{pi},L)$ that, using this approach, would be needed to obtain metrics values of all the \CRs (see Section~\ref{sec:model:app}) in each of the possible programs, resulting from the deployment of all the possible combinations of protections $comb(n_{pi},L)$ comprising at most $L$ protections.
%\begin{equation}
%t_{test}(n_{pi},L)=(t_{comp}(P)+t_{metr}(P))\cdot comb(n_{pi},L)
%\end{equation}
%Where $t_{comp}(P)$ and $t_{metr}(P)$ are the times needed to respectively compile and evaluate all the metrics on the given program $P$. The following rough estimation of the number of combinations is evaluated assuming that all the \PIs taken into account can be present only once in the combination, and that all orders of protections in the combination are acceptable\footnote{Neither of the assumptions hold in reality: some protections, \eg binary code obfuscations, can be applied more than once to the same code, and there are order of applications of protections that lead to incorrect results (\eg applying remote attestation and then a protection that changes the attested code would lead the appraiser to believe that the code has been tampered with).}:
%\begin{equation}
%comb(n_{pi},L) \approx \sum_{l=1}^{L}\left( \binom{n_{pi}}{l} \cdot l! \right) 
%= \sum_{l=1}^{L}\left( \frac{n_{pi}!}{n_{pi}! - l!} \cdot l! \right)
%\end{equation}
%Considering only the code protections developed in \asp, \esp supports 13 different \PIs, which is the value assumed by $n_{pi}$ in the above equation; if the maximum length of combination $L$ is set to three, the number of possible combination of \PIs $comb(n_{pi},L)$ can be estimated as 455; if the time to compile the program and calculate the metrics is estimated in one minute (which would make $P$ a rather simple program), it would take approximately more than seven hours to evaluate all the metrics for all the possible combinations; the needed time increases to almost five days with $L$ set to four.
%
%%tempo per calcolare metriche per tutte le soluzioni possibili = (tempo compilazione + tempo esecuzione + tempo calcolo metriche) * numero di possibili combinazioni di pi
%%
%%nPi = numero pi diverse disponibili
%%L = lunghezza combinazione su singolo asset
%%
%%numero di possibili combinazioni di L pi = combinazioni (nPi, L) * permutazioni(L) = (nPi! / ((nPi - L)! * L!) * L!
%%
%%nPi=13 L=4
%%(13! / (9! x 4!)) * 4! = 17160
%%
%%nPi=13 L=3
%%(13! / (10! x 3!)) * 3! = 286
%%
%%nPi=13 L=2
%%(13! / (11! x 2!) * 2! = 156
%%
%%nPi=13 L=1
%%(13! / 12!) = 13
%
%Therefore, evaluating all the possible metrics with the aforementioned approach is not feasible. To overcome this problem, the \emf implements an approach based on \acrfull{ml}, a branch of \acrfull{ai} that encompasses techniques to build applications that can be trained to perform specific tasks, by feeding them with examples of execution of such tasks. More formally, ``a computer program is said to learn from experience $E$ with respect to some class of tasks $T$ and performance measure $P$, if its performance at tasks in $T$, as measured by $P$, improves with experience $E$'' \cite{ml}. The \emf, in order to predict the metrics, uses a \ml technique known as \acrfull{ann}. Essentially, an \ann is a directed and weighted graph, with its nodes (called \emph{artificial neurons}) organized in layers of nodes. In general, each neuron receives a set of inputs, multiplies each of them with a set of neuron-specific weight, giving the result to a neuron-specific \emph{activation function} that produces the neuron output. The \ann inputs are feed to neurons in the first layer, which will produce their output with the activation function; such outputs will be given to as input to neurons in the next layer, with the computation continuing until the final layer is reached, which typically contains only one neuron whose output will be the \ann one. An \ann can be trained to perform a task with a training algorithm (\eg the backpropagation algorithm \cite{backprop}), which, given a set of solved instances of the task, \ie a set of inputs and expected outputs typically called \emph{training set}, is able to adjust the input weights of the \ann neurons and their activation functions. The performances of the trained \ann can be assessed using another set of solved instances, called \emph{test set}, comparing, for each instance of the task, the output produced by the \ann with the expected one.
%
%To solve the metrics prediction problem, the \emf uses a set of \glspl{ann}; each of them is able to predict a specific metric, given all the metrics on a \CR, after the application of a specific \PI on the given \CR. Formally, the prediction of one of these \glspl{ann} can be expressed with the following formula, where $c^0$ is the unprotected \CR, $c^p$ is the same \CR protected with the \PI $p$, and $m_i(c)$ is i-th metric in the set of $n$ available metrics $M_c$ evaluated on the \CR $c$:
%\begin{equation}
%f_{i,p}(M_{c^0}) \approx m_i(c^p), M_{c^0} = m_0(c^0), m_1(c^0), \dots m_n(c^0)
%\end{equation}
%In this way, the effect of a single \DPI on the metrics of \CR can be assessed. However, a solution may contain more than one \DPI applied to the same \CR: in this case, the global effect of the solution on the metrics of a \CR can be assessed by serially connecting the appropriate \glspl{ann}. For example, if a \CR $c$ is protected with a \PI $p_1$, and then with a \PI $p_2$, a metric $m_i(c^{p_1,p_2})$ can be predicted as follows:
%\begin{equation}
%f_{i,p}(M^*_{c^{p_1}}) \approx m_i(c^{p_1,p_2}), M^*_{c^{p_1}} \approx m_0(c^{p_1}), m_1(c^{p_1}), \dots m_n(c^{p_1})
%\end{equation}
%With the metrics in the set $M^*_{c^{p_1}}$, given in input to the \ann, have been predicted in turn with the appropriate \glspl{ann} with the unprotected $c$ metrics given in input:
%\begin{equation}
%M^*_{c^{p_1}} = f_{0,p}(M_{c^0}), f_{1,p}(M_{c^0}), \dots f_{n,p}(M_{c^0})
%\end{equation}
%Each \ann has been trained with metrics evaluated by \diablo on all \CRs in the source code of 21 \foss packages in the Linux Debian\footnote{\url{https://www.debian.org/}} distribution repository, listed in Table~\ref{tab:codeRegions}, obtaining all the metric before and after the application of each \PI on all the available \CRs. \diablo has been called on the object files of such program, previously compiled with \gcc configured with three different optimization levels (\lstinline|-Os, -O2, -O0|). In particular, the obtained \CRs where 35510, of which 90\% has been used for training the \ann, and the remaining 10\% to test them.
%
%\begin{table}[t]
%	\centering
%	\scalebox{.8}{
%		\begin{tabular}{llrrrr}
%			\toprule
%			\header{1}{packet} & \header{1}{version} & \header{4}{code regions}\\
%			\cmidrule(lr){3-6}
%			& & \header{1}{\lstinline|-Os|} & \header{1}{\lstinline|-O2|} & \header{1}{\lstinline|-O0|} & \header{1}{total}\\
%			\midrule
%			bc              & 1.06.95    &   495 &   462 &   520 & 1477\\
%			bzip2           & 1.0.6      &   186 &   165 &   225 & 576\\
%			ccrypt          & 1.10       &   158 &   140 &   156 & 454\\
%			dash            & 0.5.8      &  1171 &  1079 &  1229 & 3479\\
%			ed              & 1.10       &   226 &   205 &   245 & 676\\
%			findutils       & 4.7.0      &  1165 &  1178 &  1393 & 3736\\
%			flex            & 2.6.1      &   965 &   859 &  1041 & 2865\\
%			libdvdread      & 5.0.3      &   524 &   481 &   553 & 1558\\
%			libjpeg         & 8d         &  1041 &   851 &  1571 & 3463\\
%			libnet          & 1.1.6      &   576 &   586 &   563 & 1725\\
%			libstarlink-pal & 0.5.0      &  1137 &  1144 &  1265 & 3546\\
%			netcat          & 1.10       &    71 &    61 &    60 & 192\\
%			qmail           & 1.06       &   149 &   131 &   122 & 402\\
%			time            & 1.7        &    38 &    31 &    41 & 110\\
%			udo             & 6.4.1      &  2243 &  1998 &  2273 & 6514\\
%			unrtf           & 0.21.9     &   455 &   437 &   459 & 1351\\
%			vnstat          & 1.15       &   420 &   348 &   417 & 1185\\
%			watchdog        & 5.15       &   282 &   244 &   293 & 819\\
%			wbox            & 5          &    81 &    86 &    95 & 262\\
%			whitedb         & 0.7.3      &   154 &   123 &   155 & 432\\
%			zenlisp         & 2013.11.22 &   247 &   191 &   250 & 688\\
%			\cmidrule{1-6}
%			\textsc{total}      &            & 11784 & 10800 & 12926 & 35510\\
%			\bottomrule
%		\end{tabular}
%	}
%	\caption{Code regions in the metrics prediction data set.}
%	\label{tab:codeRegions}
%\end{table}
%
%The obtained \glspl{ann} perform well, with a coefficient of determination\footnote{\url{https://it.mathworks.com/help/stats/coefficient-of-determination-r-squared.html}} $R^2$ over 90\% for every protection technique. For example, Figure~\ref{fig:metricsPrediction}  shows the error plot for the predictions, on all available \CR in the test set (ordered by metric unprotected value), of the \CC and \HL metrics after the application of branch functions with \diablo (see Section~\ref{sec:background:softProt:antiRevEng:codeObf}). It is interesting noticing that the line related to the real \HL metrics values line show a numerous number of spikes, which are well approximated by the predicted values line.
%
%\begin{figure}[t]
%	\centering
%	\begin{minipage}{0.45\textwidth}
%		\begin{tikzpicture}
%		\begin{axis}[axis lines = left, xlabel = code region id, ylabel = CC, legend style = {at = {(0.05, 0.95)}, anchor = west}, mark size = 0.5pt, width = \linewidth, ymax = 50, yscale = 0.6, ylabel near ticks]
%		\addplot[Blue!35, mark = none, thick] table[header = true, col sep = semicolon, x expr = \coordindex, y index = 1] {3.ESP/data/cc.csv};
%		\addplot[Red, mark = none, thick] table[header = true, col sep = semicolon, x expr = \coordindex, y index = 2] {3.ESP/data/cc.csv};
%		\legend{targets, predictions}
%		\end{axis}
%		\end{tikzpicture}
%	\end{minipage}
%	\begin{minipage}{0.45\textwidth}
%		\begin{tikzpicture}
%		\begin{axis}[axis lines = left, xlabel = code region id, ylabel = HL, legend style = {at = {(0.05, 0.95)}, anchor = west}, mark size = 0.5pt, width = \linewidth, ymax = 1700, yscale = 0.6, ylabel near ticks]
%		\addplot[Blue!35, mark = none, thick] table[header = true, col sep = semicolon, x expr = \coordindex, y index = 1] {3.ESP/data/hl.csv};
%		\addplot[Red, mark = none, thick] table[header = true, col sep = semicolon, x expr = \coordindex, y index = 2] {3.ESP/data/hl.csv};
%		\legend{targets, predictions}
%		\end{axis}
%		\end{tikzpicture}
%	\end{minipage}
%	\caption{\CC and \HL predictions for ``branch functions, high overhead'' PI.}
%	\label{fig:metricsPrediction}
%\end{figure}

% \subsubsection{Protection overhead estimation}
% \label{sec:l1p:metrics:overhead}

% When protecting a software, the detrimental effect of the applied techniques on its performances must be taken into account, in order to obtain a software that, while exposing a good resistance against possible threats to its asset, has still an acceptable user experience. Indeed, since in general protection techniques add instructions, increase the complexity of a program \cfg with convoluted code constructs (\eg the large number of jumps needed to flatten a code), or exchange messages over the Internet (\eg remote attestation requests and responses), a certain performance decrease is an inevitable effect of software protection.

% Measuring the \emph{overhead} of a solution is therefore essential for the \eapd: while it may be great in protecting the application assets against the attacks inferred by the \ebad, its deployment by the \esd could result in a protected binary whose execution is practically unfeasible, being too slow, or occupying too much memory on the device used do run the program. The same problem is faced by the \ehal, which deploys protection on non-asset \CRs: it could theoretically protect the whole program, but is constrained in the number of applicable protection by the overhead introduced by the latter.

% To evaluate the overhead caused by the deployment of a protection on a specific \CR, the \emf uses a set of protection-specific formulas, obtained during the \asp project by the protection techniques developers. The formulas are essentially linear combinations of complexity metrics evaluated after the deployment of the specific protection. When assessing the overhead introduced by a solution, \esp evaluates it for each \CR protected by the solution. In particular, \esp takes into account five types of overhead:

% \begin{itemize}
% 	\item client \cpu overhead: the percentage of additional instructions executed by the client device \cpu when executing the protected \CR, compared with the instructions executed by the same device \cpu when running the original code;
% 	\item server \cpu overhead: the percentage of additional instructions, constituting the routines of the assessed protection in the \ascl (see Section~\ref{sec:background:softProt:antiTamp}), executed by the server \cpu in order to service the requests made by the client due to the deployment of an on-line protection, \wrt the number of \ascl instruction executed without servicing any client protection requests (\ie with no on-line protections deployed to the server);
% 	\item client memory overhead: the amount of the client device memory needed to store the data needed by the protection, measured in Bytes;
% 	\item service memory overhead: the amount of the server memory needed to store the data needed by the protection service routines in the \ascl, measured in Bytes;
% 	\item network overhead: the average amount of bandwidth occupied on the client device Internet connection, during the application execution, due to messages exchanged by the on-line protection technique with the \ascl.
% \end{itemize}

%All of the overhead estimation formulas are available in the \PI description files described in Section~\ref{sec:esp:impl}. An example formula is the one to estimate the client \cpu time overhead. It can be obtained starting from the definition of $\omega_{client}^{cpu}$, \ie the client \cpu overhead described above, where $C$ is the original code, and $C^{P}$ is the same code protected with an undefined protection technique $P$:
%\begin{equation}
%\omega_{client}^{cpu}(C,P)=\left(\frac{I(C^P)+\phi^P}{I(C)}-1\right)\cdot 100
%\end{equation}
%$\phi^P$ is a constant, related to the specific protection technique used, which represents an eventual fixed number of instructions added to the protected code, unrelated from any of the latter metrics. An example of this constant is $\phi^{AD}$, the fixed number of additional instructions introduced by the anti-debugging technique described in Section~\ref{sec:background:softProt:antiDeb}: these are due to the context switches that the \cpu must execute every time the program flow enters in a protected \CR, since the technique moves such code inside a debugger (another process \wrt the protected application): the number of instructions needed to execute one context switch is set in the \esp to 20000 assembly instruction, an estimation obtained by protection developers from an empirical assessment of the anti-debugging technique executed during the \asp project.

% In the protection decision workflow (Section~\ref{sec:l1p:workflow}), the \emf is tasked to assess the global overheads introduced into the target application by a solution, after its deployment on the target: this is needed to ensure that such overheads are limited\footnote{The overhead global limits for the protected target application must be set by the \esp user.}, so that the produced binary does not present a performance degradation so conspicuous that the application becomes unusable. The \emf can predict the metrics of the assets, which are modified by the deployment of the solution, using the neural networks described in Section~\ref{sec:l1p:metrics:prediction}, and use such predictions to estimate the values of the overheads, by feeding the predicted metrics to the overhead formulas presented above in this section. This leads to the estimation of overheads for each asset: however, a global overhead value is needed, summarizing the medium slow-down introduced by the protections, in order to assess the feasibility of the solution. The \emf obtains a global value for each kind of overhead, combining the relative overhead values computed on each function comprised in the application source, using the following weighted sum where each overhead is first multiplied to a weight, indicating the percentage of instructions of the related function \wrt the total number of instructions constituting the application code. It should be noted that also the overheads introduced by protections on variables are considered: since these protections introduce more code in the function containing the protected variable, such as for example the additional instructions needed to decode variables obfuscated with the technique described in Section~\ref{sec:background:softProt:antiRevEng:dataObf}, the metrics of the function will be impacted by such protections, and can be used to assess the overhead introduced by such techniques as it is done for their code counterparts.

% \subsubsection{Protection index}
% \label{sec:l1p:metrics:score}

% To build the solution solver mini-max algorithm, first a score for its states must be defined. As said before, the protection decision process is modelled as a zero-sum game: there is a unique score for the states in the mini-max tree, representing the global level of security of the application, \ie the effort needed by an attacker to breach the user-defined security requirement of the assets in the application. Indeed, modelling this effort is not trivial, since it depends on a series of factors. First, the profile of the attacker must be taken into account: for example, a seasoned attacker, proficient in the assembly language, will need considerably less effort to understand the purpose of an algorithm in the binary, in respect with a newbie that has never seen assembly before. However, if an attack simply involves using an automated attack tool, the effect of the attacker profile on the difficulty of carrying out the attack may be less broad. Also, the inherent characteristics of the assets must be taken into account, but also the relationships among them: intuitively, comprehending a code with a complex \cfg is harder than understanding a simple code with few basic blocks; however, this holds also when an attacker wants to understand the purpose of a local variable in a function, a task that will be considerably harder if the variable is accessed in various points of a complex function comprising many instructions in a convoluted \cfg. 

% Thus, a set of measures to model the security level of the application are needed, in order to grasp all these nuances. Protections deployed on the application must increase at least one of the measures, while successful attacks will decrease one or more measures. The solution solver, to evaluate the \emph{protection index}, \ie the score of mini-max tree leaves, uses the following measures, computed for each asset:
% \begin{itemize}
% 	\item \emph{uncertainty}: the confusion an attacker feels when trying to understand the purpose and logic of an asset, for example an obfuscated one (Section~\ref{sec:background:softProt:antiRevEng});
% 	\item \emph{remote instructions}: the increased difficulty an attacker encounters, when parts of the target application code are not under his control, having been moved to a safe remote location, \eg using code mobility (Section~\ref{sec:background:softProt:antiTamp:codeMobility});
% 	\item \emph{alteration detection}: the capability of a protected application to detect when the attacker is attempting to tamper with it, increasing the difficulty of these types of attacks, since the attacker must tamper the protected assets without tripping off any alarm, \eg avoiding the detection enforced by remote attestation (Section~\ref{sec:background:softProt:antiTamp:RA});
% 	\item \emph{alteration avoidance}: the ability of a protected application to negate a modification, for example blocking tools used by the attacker to tamper with the application code, as it is done by the anti-debugging technique (Section~\ref{sec:background:softProt:antiDeb}).
% \end{itemize}
% The attacker will try to lower the protection index, by executing attacks that impact one or more of these measures. For example, an attacker that sniffs the traffic of an application protected with code mobility, has a good chance to identify the remote instructions downloaded by the application: thus, if an \AP containing a sniffing \AS is played by the attacker, the \emph{remote instructions} metrics is lowered accordingly. Indeed, the profile of the attacker has an impact on the probability of success of this attack: while sniffing the traffic is not complicated (using for example a free tool like Wireshark\footnote{\url{https://www.wireshark.org/}}), understanding that the application is downloading the instructions, and consequently identify them in the traffic captures, is definitely more difficult, and requires knowledge of the protection technique by the attacker. Another example is trying to understand of an obfuscated asset code, thus having an high uncertainty measure: the attacker may resort to static or dynamic analysis tools, in order to obtain more understandable representation of the code (\eg \cfg, execution traces), which will, in turn, decrease the uncertainty of the attacker regarding the logic of the asset code. The attacker expertise can be set by the user via the \eui. Indeed, knowing the possible type of attacker is fundamental when the protections are decided: if the target program is a mobile app, sold for a low price, protecting it with heavy measures is useless, since the reward of breaking the application will be  probably not enough to interest an experienced attacker; the only result would be an unnecessarily slow application, and, if proprietary protections are taken into account, the cost of their licenses could exceed the profits gained with application sales.

% Attacks and protections try respectively to breach and defend the assets security requirement: this link is embedded also in the measures: each of them specifies also the risk of the attacker being able to breach a specific security requirement. Uncertainty is strictly related to confidentiality, since for example an attacker that becomes certain of the logic of a code has succeeded in reverse engineering it. Similarly, remote instructions of a code, moved to a trusted server out of the attacker reach, have more possibility to remain confidential. Alteration detection and alteration avoidance are clearly related to integrity and execution correctness\footnote{The execution correctness is a stronger form of integrity for code, leading to complex attack paths that require more effort for the attacker, as explained in Chapter~\ref{sec:prolog}.}, since they express the capability of an application to detect or stop attacker attempts to tamper with the protected assets.

% Also, as explained before, these measures must be linked to the characteristics of the asset code: therefore, they are linked to the software metrics (Section~\ref{sec:l1p:metrics}) of the asset. In particular, the initial values of these measures, after the single defender move (\eg the deployment of one of the solutions found by the walker) are evaluated as weighted sums of the software metrics. Thus, the protections increase the protection index because they increase the metrics: this behaviour takes its roots from the concept of transformation potency proposed by Collberg, as explained in Section~\ref{sec:l1p:metrics}. For example, the uncertainty measure of an asset is based on the \HL and \CC of its code, two measures that are increased by code obfuscation techniques (\eg the \cff technique presented in Section~\ref{sec:background:softProt:antiRevEng:codeObf} increases the \CC, since the resulting \cfg contains a high number of parallel paths). 

% Given a target application $A$, its global protection index $P(A)$ in a state of the mini-max algorithm is evaluated by the solution solver using the following formula:
% \begin{equation}
% P(A)=\sum_{i}^{\#assets} w_i \cdot \left(\sum_{j}^{\#measures} \beta_j \cdot s_{ij}  - L \cdot l_{ij}\right)
% \end{equation}
% where $w_i$ is a user-defined weight representing the importance of the $i$-th asset, $s_ij$ is the value of the $j$-th security measure evaluated on the $i$-th asset, and $\beta_j$ is a user-defined coefficient for the $j$-th security measure. The attacker succeeds in violating the $i$-th asset if at least one measure, after the successful execution of one or more \APs against the asset, goes below a user-defined constant threshold $T$; this is expressed in the formula with a user-defined constant $L$ and the $l_{ij}$ boolean variable, evaluated as following:
% \begin{equation}
% l_{ij} = 
% \begin{cases}
% 1, & \text{if } s_{ij} < T\\
% 0, & \text{otherwise}\\
% \end{cases}
% \end{equation}
% Since the attacker wins if he succeeds in breaching at least one security measure (\ie one asset security requirement), the $L$ constant should be set to a very big value, so that the mini-max algorithm will avoid selecting moves that lead to such losing states. Also, if the user has not set a security requirement for an asset (\eg it is not important that a function is understood by an attacker, as long as is not able to modify it), the related measures $s_{ij}$ are excluded from the formula.

% Finally, a way to quantify the impact of successful \APs on security measures is needed, so that the mini-max algorithm can update the score accordingly. This impact of an \AP is assessed taking into account the inherent difficulty of \ASs constituting the \AP and the probability, given the attacker expertise, of successfully execute such \ASs, but also the ability of protections in thwarting specific types of attack tools, and the increased resistance against specific \AS due to synergies among protections. All this information, stored in \ekb, derive from experts knowledge gathered during the \asp project. When the attacker plays an \AP, each of the constituting \AS is executed following the order specified by the \AP, updating the measures of the affected asset. In particular, after the execution of the $k$-th \AS in the played \AP, targeting the $i$-th asset, the $j$-th measure will take the following value:
% \begin{equation}
% s^\prime_{ij} = \big{(} 1-(\pi_k\cdot(1-\omega_k)\cdot\lambda_k)\big{)} \cdot s_{ij}
% \end{equation}
% where:
% \begin{itemize}
% 	\item $s_{ij}$ and $s^\prime_{ij}$ are the impacted measure values, respectively before and after the assessed attack step execution;
% 	\item $0\leq \pi_k \leq 1$ is the attacker probability of successfully execute the $k$-th \AS, depending from the type of \AS and the selected attacker expertise;
% 	\item $0\leq \lambda_k \leq 1$ assesses the impact of the \AS type against the security measure (\eg dynamic analysis, carried out for example using a debugger, as an high impact on the confusion measure);
% 	\item $0\leq \omega_k \leq 1$ represent the mitigation effect of protections applied on the $i$-th asset against the type of \AS.
% \end{itemize}

% The global mitigation effect $\omega_k$ of the \DPIs applied on the $i$-th asset against the $k$-th \AS in the assessed \AP, used to evaluate $s^\prime_{ij}$, can be obtained by combining the mitigation effects of each \DPI applied to the $i$-th asset, as in the following formula:
% \begin{equation}
% \omega_k = 1 - \sum_{p}^{\text{\#DPIs on i-th asset}}(1-\omega_{k,p})
% \end{equation}

% The protection mitigation effect $\omega_k$ must take into account also the ordering of protections in the solution played by the defender, with a bonus for encouraged precedences and a malus for discouraged ones (Section~\ref{sec:l1p:walker}), and is obtained by combining the mitigation effects of each \DPI applied to the $i$-th asset. Given the $p$-th \DPI applied on an asset endangered by the $k$-th \AS in the \AP, the relative $\omega_{k,p}$ mitigation effect is obtained with the following formula:
% \begin{equation}
% \omega_{k,p}=1 - (1 - m_{k,p}) \cdot \frac{(1 - E)^e}{(1-D)^d}
% \end{equation}
% where:
% \begin{itemize}
% 	\item $0 \leq m_{k,p} \leq 1$ is the level of mitigation introduced by the $p$-th protection against the $k$-th \AS, if $p$ is the only protection applied to the endangered asset;
% 	\item $0 \leq E \leq 1$ and $0 \leq D \leq 1$ are respectively the user-defined bonus for encouraged precedences and malus for discouraged ones;
% 	\item $e$ and $d$ are respectively the number of encouraged and discouraged precedences, \ie the number of \DPIs, applied on the same asset as the $p$-th one, preceding the latter in the solution, which are respectively favoured or hindered by the deployment of the $p$-th \DPI.
% \end{itemize}

% Default values for the various constants used by the solution solvers have been found empirically, assessing the solutions found by the \eapd on the \asp use-case applications \wrt solutions devised manually on such applications by experts of the software security companies involved in the aforementioned project (Section~\ref{sec:esp:results}).

\subsection{Exploring the solution space}
% \label{sec:l1p:walker}

\begin{itemize}
    \item useless intro
    \item talk about solutions + constraints (overheads + protection order)
    \item talk about solution space size -- see complexity analysis on ASPIRE deliverable
    \item talk about POs and code correlation sets
    \item put workflow picture from Leon's thesis or ASPIRE deliverable
    \item describe the algorithm + cite Knuth
    \item complexity analysis: how humongous is this solution space?
\end{itemize}

% This section details the solution walker algorithm, part of the \eapd, tasked with steps 4 and 5 of the protection decision workflow presented in Section~\ref{sec:l1p:workflow}. While the \eape is able to build a set of \DPIs by analyzing each asset in isolation, finding the \PIs that are suitable to defer the attacks found by the \ebad against the asset security requirement, the solution walker considers the application as a whole, taking into account the complete code structure and the relationships among the various \CRs constituting the application: the goal of this algorithm is to produce a comprehensive protection solution, combining a subset of the \DPIs inferred by the \eape, able to protect the application from all the possible attacks against all the assets comprised in the target program. In doing so, the solution walker considers the interactions among the protections included in the solution, in order to avoid the introduction of inconsistencies that may alter the business logic of the application or even lead to a non-working protected binary. Also, the overhead introduced by the protections comprised in the built solution is taken into account: the \esp user can set limits to the global overheads (detailed in Section~\ref{sec:l1p:metrics:overhead}) introduced by the application, and the solution walker will output only solutions that stay below this user-defined upper bounds, thus producing a combination of protections that preserve the application user experience (clearly, if global overhead limits set by the user are correct). So, since the ordering among protections is important, the problem the solution walker aims to solve is finding a protection solution, \ie an ordered set of \DPIs, with at least one \DPI safeguarding a \PO, to protect the whole application, and with an order among \DPIs that does not introduce any inconsistencies in the resulting protected binary.
%In Figure~\ref{fig:walkerWorkflow}, the detailed workflow of the solution walker algorithm is presented.


%\todo{togliere adjust the singletons in the permutations e call a solution solver (quest'ultima forse)}
%\begin{figure}
%    \centering
%    \includegraphics[width=0.7\linewidth]{6.L1P/figs/walkerWorkflow}
%    \caption{Workflow of the \eapd solution walker algorithm.}
%    \label{fig:walkerWorkflow}
%\end{figure}
% First of all, given the application code structure, and the available \DPIs, the algorithm computes the \emph{code correlation sets}: two code regions are if they share at least one line of code. This is necessary, since, as stated in the introduction of this chapter, the relationships among assets must be taken into account, to avoid possible inconsistencies in the resulting solution that may lead to an application not behaving correctly, like in the case of the containment relationship. Another relationship that must be considered is the use of a variable or constant by a \CR: for example, if a code region is protected with anti-debugging (see Section~\ref{sec:background:softProt:antiDeb}), and its execution depends on the value of a string literal that has been encoded with Tigress literals obfuscation (Section~\ref{sec:background:softProt:antiRevEng:dataObf}), every time that the code moved into the debugger has to access the constant value, a call to the encoder function outside the debugger will be needed to obtain the literal; this will lead to a context switch for each call, which, while not posing a threat for the correctness of application execution, can lead to an unbearable overhead for the application, if the number of calls is conspicuous, and it is therefore advisable to protect also the string encoder with anti-debugging. Also, using code correlation sets can speed up the solution walker algorithm, since it reduces the number of crosschecks among \DPIs in the same solution needed to avoid possible incompatibilities among them. Code correlation sets are built by the solution walker recursively following such relationships among \CRs and data: these are found automatically in the first step of the \esp workflow, \ie with the source code analysis executed by the \esca via \cdt (Appendix~\ref{sec:esp:impl}). Thus, the problem of finding a suitable ordered combination of protections for all the application assets is divided in finding one ordered combination for each code correlation set: the solution can be therefore redefined as a partially ordered set of \DPIs, since only the ordering of \DPIs applied to assets in the same code correlation set is important.

% In the second step of the workflow, the solution walker chooses, for each \PO, the number of \DPIs tasked to protect it: a different tuple of integers is generated every time this step is executed, until all the possible tuples are considered. At least one \DPI for each \PO must be included in the solution, in order to provide at least a minimum protection for each asset in the program. To speed up the computation, the solution space can be reduced by setting a maximum number of \DPIs for each \PO. 

% Then, for each tuple of integers, the solution walker executes the third step in its workflow, first building for each \PO all the possible sets of \DPIs with the length specified for the related \PO in the tuple, and then building all the possible combinations of these sets of \DPIs, with one set for each \PO. Every time this workflow step is executed, one of these combinations of \DPIsets is built, and the next step in the workflow is called, until all the possible combinations have been considered. It should be noted that certain protections are \emph{singletons}, \ie can be applied only once to an asset: an example of singleton protection is code mobility (Section~\ref{sec:background:softProt:antiTamp:codeMobility}), which protects a code by moving it to a remote server, an operation that obviously can be done only once. Thus, if a \DPI employs a singleton protection, the solution walker will apply it at most one time on each asset: this means checking that this \DPI is included at most one time among all the sets targeting the \POs related to the same asset. To do so, also the containment relationships must be considered, since if for example anti-debugging is used to protect a whole function, also all the code regions contained in it will be moved in the self-debugger: thus, is not possible to apply the same technique on contained code regions, if the container function has been already protected with the same technique.

% Then, the solution walker executes the last step in its workflow: given a combination of \DPIs protecting all the \POs of the application, the solution walker generates all the admissible orderings of for the \DPIs, excluding the ones containing \emph{forbidden precedences}, which is cases when applying one protection technique on an application part already protected with another one will lead to a non-working protected binary, such as in the example presented before of the obfuscation of a code already monitored by remote attestation. To reduce the number of different orders that must be considered by the walker, the latter can be instructed to avoid also \emph{discouraged precedences}, \ie cases when applying one protection to a code or datum already protected by another technique, while not leading to an inconsistency in the resulting binary, will likely have some unwanted effect: for example, obfuscating a code that will be then protected with code mobility is not only completely useless from a security point of view, since the code will be moved to a trusted remote server, but it is also detrimental for the server performances, since the obfuscation will slow down the execution of the moved code. As already explained before, to check that the ordering does not contain any forbidden precedences (and discouraged precedences, if the walker is instructed by the user to do so), the walker needs to verify all the precedences among all the \DPIs protecting assets in the same code correlation set. The walker will produce all the possible orderings for the given combination of \DPIs; then, the walker will return to the previous step, generating another combination of \DPIs to be ordered.

% Summarizing, the final result of the walker is a set of valid solutions, able to offer at least some degree of protection to each \PO in the application, and that, if deployed, produce a working protected binary. However, this is not sufficient to deem a solution as effectively being usable to protect the application, since the solution must not penalize excessively the protected application performances. However, the performance overhead introduced deploying a protection on an application asset do not depend solely on the technique used and, but also on the specific characteristic of the protected asset. For example, if the integrity of a code area is safeguarded using remote attestation, the effort needed to compute its hashes, \ie the additional instructions that must be executed by the \cpu of the device running the application due to the deployment of this technique, will be directly dependent on the size of the protected code.  

%Second, the protections included in the solution must be effective in protecting the asset from the specific \APs inferred by the \ebad against each asset. However, the a-priori information in the \ekb regarding the generic effectiveness of a protection in deferring possible attacks is not sufficient: also in this case, the characteristics of the asset must be taken into account. For example, a \CR whose confidentiality must be preserved may have a complex \cfg, already difficult to be comprehended by an attacker: in this case, inserting opaque predicates may not be too much beneficial, since their effect in complicating an already convoluted \cfg would be limited. Instead, if a function has a straightforward \cfg, constituted by a limited number of basic blocks with many sequential instructions inside them, opaque predicates may be effective in splitting these long basic blocks, generating a more complex \cfg.

% So, to solve both problems, a quantitative measure of the characteristics of the assets is needed, in order to both assess the solution effectiveness in complicating the execution of attacks, and the overhead introduced in the application. \esp solves this problem by using a set of software metrics, presented in  Section~\ref{sec:l1p:metrics}, evaluated by the \emf using \diablo. The solution walker, after building a solution, calls the \emf to obtain the global overhead introduced in the application; these will be evaluated by the \emf using a set of \PI-specific formulas (Section~\ref{sec:l1p:metrics:overhead}) based on the values of the aforementioned metrics.
% If the computed overhead is above a user-defined threshold, defining the maximum acceptable slow-down for the application, deployment of the solution is deemed unfeasible, thus the latter is discarded by the walker: its workflow goes back to the previous step, and another solution is built. Otherwise, the analyzed solution is deemed to have a feasible overhead, and the walker passes it to the solution solver (Section~\ref{sec:l1p:solver}): this algorithm produces a score, also based on the aforementioned metrics, summarizing the solution effectiveness in deferring the possible \APs that can be ported against the protected binary.

\subsection{Efficiently finding the optimal solution}
% \label{sec:l1p:solver}

\begin{itemize}
    \item useless intro (again)
    \item cite briefly again the problems + Barak paper
    \item intro to game/chess theory
    \item short comparison between standard mini-max and our sick version
    \item talk about pruning/reduction techniques
    \item talk about transposition tables
    \item talk about the code correlation set version
    \item complexity analysis
\end{itemize}

% This section presents the solution solver algorithm, which is tasked to decide, among the asset protection solutions inferred by the solution walker algorithm (see Section~\ref{sec:l1p:walker}), the ones that are best suitable to deferring the possible \APs that can endanger the \POs, \ie the user-defined security requirements of the application assets. In doing so, the solver assigns to each evaluated solution a score, called protection index, whose computation is described in Section~\ref{sec:l1p:metrics:score}.

% As already described in the introduction of this chapter, this problem is not trivial: the relationships between the protected assets code structure and security requirements, the possible attacks against them, the deployed protections with the interactions among them must all be modelled in order to find a quantitative way to score the solutions, so that they can be compared and the best solutions, \ie the ones with most chances to effectively defer the attacker, can be presented to the user for subsequent deployment on the target application. The basic idea behind the solution to this problem is modelling the protection decision process in a \mate scenario as a game, with characteristics similar to chess. The checkerboard is the application code, the white player (who moves first) is the defender tasked to produce a protected version of the application that must be publicly released afterwards, and the black player is the attacker that must breach at least an asset security requirement. The defender moves its pieces, \ie the protections, by deploying them on the application; the attacker moves are instead executions of attack paths against the protected application. It should be noted that, due to the characteristics of the \mate scenario, there is one fundamental difference between the chess and the protection decision game: in chess, player moves are alternated, while in a \mate scenario, the defender has the first move, protecting the application before its release, but afterwards the attacker has theoretically infinite moves. Thus, at the protection decision game the defender wins if it defers as much as possible the breaching of assets security requirements, choosing the combination of protections most effective in increasing the effort needed to carry out successful attacks: since perfect protections do not exist (this has been proven formally for obfuscation techniques by Barak\etal\cite{barakImpossibility}), an attacker with infinite time (and subsequently moves) will, in the end, be able to break all the protections chosen by the defender. However, a well-protected application may cause the attacker to throw in the towel after some failed attack attempts. Also, the economic model behind the attacker willingness to breach the application may, in fact, limit the time: for example, an attacker may want to break a licensing scheme of a commercial application, in order to build a crack to use it without a proper license, and thus sell the crack on the black market; however, if a new version of the application is released before the attacker can succeed in building the crack, even if it in the ends succeeds in creating the crack, it would be incompatible with new application version, and thus would not have any value on the black market (or at least a greatly reduced one).

% Using this parallel with chess, all the abundant research on the automation of this game can be adapted for protection decision purposes. This research has its roots in the broader field of game theory, which, as defined by Myerson in \cite{gameTheory}, is \emph{``the study of mathematical models of strategic interaction between rational decision-makers''}, and has been applied to solve problems in many fields, for example in economy, \eg to model strategies of companies \cite{gameTheoryEconomy}, or for military purposes, \eg to analyze possible choices for nuclear deterrence during the cold war \cite{gameTheoryMilitary}. Indeed, research has been also on possible applications of game theory for cybersecurity, as presented in a recent survey \cite{gameTheoryCybSec} by Cuong\etal: reviewed works include uses of game theory to model attack and defence of smart grid systems, computer networks and cryptographic schemes.

% Building computer programs able to play chess, a problem known as \emph{chess programming}, has been first introduced by Shannon in 1949 \cite{shannonChess}. In this seminal paper, two of the core concepts of chess programming are applied to this problem for the first time: the mini-max algorithm (presented in 1928 by Borel in \cite{borelMinimax}), used to model the evolution of a game in various states (\eg different disposition of pieces on the checkerboard) through moves of the players, and the use of an evaluation function, \ie an heuristic to estimate the probability of a player winning a game in a specified state. These concepts are still at the base of modern chess engines, such as IBM Deep Blue \cite{deepBlue}, a special-purpose computer that in 1996 was the first one able to win a chess game against a human chess world champion, Garry Kasparov, and Stockfish\footnote{\url{https://stockfishchess.org/}}, an open-source engine which at the time of writing is at the top of the \emph{CCRL 40/4} chess engine ratings\footnote{\url{http://ccrl.chessdom.com/ccrl/404/}}.

% For zero-sum games like chess, where the gain resulting from one player's move is exactly the same as the damage for the other player (so that their sum is zero), a single score for a position can be used, ranging   between $-1$ (black player's checkmate) and $+1$ (white player's checkmate). Thus, given a game state, if it is the white player turn to move, it will try to find a move that leads to another game state with a score higher than the precedent one; the opposite applies if it is the black player's turn. The same holds for the protection decision game: the defender's protections will increase the score, while the attacker will execute \APs to decrease it. For chess, the score of a state is linked to various factors, for example the number of pieces still in game for each player, their location on the chessboard, and if the players have performed castling. In Shannon's paper, the following example evaluation function is provided, in order to evaluate the likelihood of a white player winning a chess game in a state $P$:
% \begin{equation}
% \begin{split}
% f(P) = & 200(K-K^\prime)+9(Q-Q^\prime)+5(R-R^\prime)+3(B-B'+N-N^\prime)\\
% &+(P-P^\prime)-0.5(D-D^\prime+S-S^\prime+I-I^\prime)+0.1(M-M^\prime)+...
% \end{split}
% \end{equation}
% in which $K$,$Q$,$R$,$B$,$B$,$P$ indicate respectively the number of white kings, queens, rooks, bishops, knights and pawns still in play; $D$,$S$,$I$ are penalties for doubled, backward and isolated white pawns; $M$ is a bonus for the mobility of white pieces, \ie the number of legal moves available to the white player; the primed versions of this variables indicate their relative black pieces counterparts.

% The mini-max algorithm implements a worst-case analysis: when the opponent has to move, it will always choose the best move, \ie the one that, given the current state, will lead to a new state that is the most favorable for him or her; translated to chess, if the opponent is the black player, he will choose every time the move that leads to the state with the lowest score possible. Thus, since the opponent will choose, among the moves available, the ones that maximize the loss for the player, the mini-max algorithm chooses the move that leads, after the opponent move, to the minimum of the losses maximized by the opponent. Figure~\ref{fig:l1p:mini-max} sketches the reasoning process of a mini-max algorithm, trying to find the best move for a player that must maximize the score; due to computational limitations, the algorithm is able to foresee only the possible outcomes after two moves, the one made by the algorithm and the next move made by the opponent. The figure renders the mini-max reasoning process using a tree: each node is a game state, with the root the initial one, while the edges are the possible moves, each one leading from one state to another. The algorithm starts to compute the scores associated with the possible outcomes. Then, it assigns a score to each node in the layer immediately above the leaves (Figure~\ref{fig:l1p:mini-max1}): having the nodes only three layers, these are the possible states in which the opponent must move, immediately after the player move that is subject to evaluation by the mini-max algorithm. Using a worst-case analysis, the algorithm infers that the opponent will choose the move that minimizes at most the score: so, each node in the opponent layer will be associated with the lowest score among its immediate successors (Figure~\ref{fig:l1p:mini-max2}), which means assigning $3$ to the left node in the second layer, and $4$ to the right node. Then, the process is repeated, but this time the player must move, so each node (in the figure only the root) will be assigned with the maximum of the scores of its children (Figure~\ref{fig:l1p:mini-max3}). In this way, the move is made taking into account also the reaction of the opponent; clearly, the number of forecast moves can be higher, with various alternating minimizing and maximizing phases, but the principle behind the algorithm holds.

%wins if reaches a state with a $+\infty$ score; thus, the algorithm tries to find the move that leads to state with the highest possible score, knowing that the opponent will choose the moves that minimize the score as possible, trying to win the game reaching a state with a $-\infty$ score. Since computational resources are limited, the algorithm is able to foresee at most four moves, two for each player. The algorithm starts by evaluating all the possible outcomes of the possible combination of foreseen moves, \ie the scores of the tree leaves. These leaves are direct outcomes of the fourth and last move: since the players alternate their moves, the fourth move will be made by the opponent, which will try to minimize the score. Using a worst-case analysis, the algorithm infers that the opponent, given one of the states in the fourth layer of the tree, will choose the move that leads to the tree leaf with the lowest value: for example, looking in figure at the node on the left of the fourth layer, the opponent can choose between a move that leads to a state with score $10$, and another that will lead to the player victory, with a score $+\infty$; obviously, the opponent will choose the move with score $10$, which is, in turn, the score assigned to the node, as marked in figure with a red arrow. In this way, all the possible fourth moves by the opponent are foreseen; then, the algorithm can infer all the possible third moves, choosing again the 

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{6.L1P/figs/minimax}
%    \caption{Example of execution of a mini-max algorithm.}
%    \label{fig:l1p:mini-max}
%\end{figure}

%\begin{figure}[t]
%	\centering
%	\begin{minipage}[b]{0.25\linewidth}
%		\centering
%		\includegraphics[width=\linewidth]{6.L1P/figs/minimax1}
%		\subcaption{Step 1.}
%		\label{fig:l1p:mini-max1}
%	\end{minipage}
%	\begin{minipage}[b]{0.25\linewidth}
%		\centering
%		\includegraphics[width=\linewidth]{6.L1P/figs/minimax2}
%		\subcaption{Step 2.}
%		\label{fig:l1p:mini-max2}
%	\end{minipage}
%	\begin{minipage}[b]{0.25\linewidth}
%		\centering
%		\includegraphics[width=\linewidth]{6.L1P/figs/minimax3}
%		\subcaption{Step 3.}
%		\label{fig:l1p:mini-max3}
%	\end{minipage}
%	\caption{Example execution of a mini-max algorithm.}
%	\label{fig:l1p:mini-max}
%\end{figure}

% The mini-max algorithm and the evaluation functions are the foundations on which the solution solver algorithm is built.

% \subsubsection{Solution solver mini-max algorithm}
% \label{sec:l1p:metrics:mini-max}

% The solution solver uses a mini-max algorithm in order to find the score for each solution built by the walker (Section~\ref{sec:l1p:walker}), assessed in a worst-case scenario, \ie when the attacker chooses the best \AP to breach at least one security requirement of an asset in the lowest possible time. Figure~\ref{fig:solvertree} sketches a mini-max tree built by the solution solver: the root represents the best solution score found so far, the first layer contains the solutions built by the walker, and the remaining layers the possible \AP mounted by the attacker against the application assets, given the solution chosen by the defender. It should be noted that an \AP can be repeated an infinite number of times by an attacker (\ie an attacker can concentrate on a specific attack for a longer time), thus the tree is theoretically infinite: the mini-max algorithm stops after a user-defined number of layers in the mini-max tree, \ie number of \APs tried by the attacker, such as a chess engine forecasts a limited number of moves; clearly, a deep search will result in more precise scores, but will take a longer time for the solver to produce them. More precisely, the time needed for the execution of the solver grows exponentially with the number of layers in the tree: if the \ebad infers $a$ \APs against the application assets, the user sets a number $l$ of mini-max tree layers, and the solution walker builds $s$ different solutions, the mini-max tree will contain $s \cdot a^l$ states, whose score must be evaluated using the formulas described in Section~\ref{sec:l1p:metrics:score}. Thus, times needed to evaluate the solution scores can become unfeasible for bigger applications, containing many assets: the solution walker mini-max implementation uses a set of strategies to reduce the number of the states that must be evaluated; in fact, the tree in figure is unbalanced, since some of the possible states are not considered due do these strategies.
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth,trim=0cm 2cm 0cm 2cm,clip=true]{6.L1P/figs/minimaxTree}
%	\caption{Example of a mini-max tree built by the solution solver.}
%	\label{fig:solvertree}
%\end{figure}
% First of all, the code correlation sets, described in Section~\ref{sec:l1p:walker}, are used to split the trees: since an \AP against an asset can impact only the measures of the targeted assets, and of the other ones contained in the same correlation set (\eg if the attacker debugs a function, it does automatically the same for all the \CR contained in the function), a separate smaller tree can be used to model sequences of \APs targeting the same code correlation set; due to the exponential nature of the mini-max algorithm, this greatly reduces the computation time.

% Also, the following standard enhancement strategies, typical of chess programming (used by all the modern chess engines), are implemented to further speed-up the solution solver:
% \begin{itemize}
% 	\item \emph{Alpha-Beta pruning}: a branch-and-bound technique, where $\alpha$ and $\beta$ are respectively a lower and higher bound; if a move leads to a state with a score lower than $\alpha$ or higher than $\beta$, it is considered respectively too bad (a better move surely exists) or too good to be true (due to the worst-case scenario considered, the attacker will never choose the moves that lead to this state), thus the mini-max does not consider it anymore, pruning from the tree this state and all its children;
% 	\item \emph{Reduction}: a technique that avoids further analyzing a state, if the outcome of the subsequent moves is already clear; for example, if a state contains a security measure that is almost broken, it is clear that the attacker will succeed in breaking with few more \APs, thus winning the game, and therefore the solution solver will deem the state as undesirable without further searches (\ie not considering possible children);
% 	\item \emph{Transposition table}: a large hash table, containing information about a state already encountered before, but with another sequence of moves (a \emph{transposition}, in chess jargon).
% \end{itemize}

% This techniques need a set of user-defined parameters (\eg $\alpha$ and $\beta$ for pruning), whose value can greatly affect the quality of the found solution, but are difficult to find: however, the user can launch the mini-max algorithm with a shallow depth, obtaining a solution in no time, in order to assess a medium value for the solution score, and base the parameters on this medium value. For example, the optimal solution score must be comprised between $\alpha$ and $\beta$ for the mini-max algorithm being able to find it: so, if a fast execution leads to a best solution with score $50$, probably the optimal solution score will be near that value, thus $\alpha$ and $\beta$ can be set accordingly, \eg to $40$ and $60$. Then, the solution solver can be launched with a deep search, which will lead to the optimal solution (or at least to an approximation of it).

\subsection{Discussion}

threats to validity/limitations/validation vs. requirements for asset protection phase

% \label{sec:l1p:validation}
% This section compares the asset protection methodologies described in this chapter with the \esp requirements detailed in Section~\ref{sec:esp:problem}.

% Regarding the risk framing requirements (see Section~\ref{sec:esp:problem:framing}), they are completely satisfied by the \esp asset protection phase. First, attacker skills are taken into account in the solution score computed by the solution solver algorithm (see Section~\ref{sec:l1p:solver}). Also, the protection solutions are presented to the user in a detailed and human-readable format, specifying for each user-defined asset the protection techniques that must be used to safeguard each of its security requirements, the protection tool that must be used to deploy the technique to the asset, along with the configuration parameters needed to drive the tool in this process, and the order of application of each protection to the asset. Finally, the algorithms that implement the asset protection methodologies described in this chapter can be fully customized by the user, with a set of parameters that influence the time needed to execute them, and the accuracy of the produced results. A deep exploration of the solution space may be performed prior to the distribution of the application to the public, thus obtaining a solution near the optimum. Conversely, a fast solution search may be performed each time a patch for the software must be released, when time is an issue, thus refining the existing protection solution with additional protections to defer possible attacks enabled by the introduction or modification of code performed by the patch. Thus, the asset protection phases adapt to the software life-cycle. 

% Regarding the risk mitigation requirements (see Section~\ref{sec:esp:problem:mitigation}), they are satisfied by the methodologies presented in this chapter. The main objective, deferring the possible attacks against the application assets, is completely accomplished, covering all the attack paths inferred during the risk assessment phase of \esp (see Chapter~\ref{sec:prolog}). The protection solutions are obtained taking into account the application structure and the complexity metrics of the code comprising the user-defined assets. Furthermore, \esp supports automated protection tools for each of the techniques employed in the asset protection phase, thus the deployment of the obtained protection solutions can be completely automated. Overheads are also taken into account when the solutions are inferred, thus the user experienced is not hampered, with protected binaries obtained after the deployment of such solutions still responsive to the user. 
% %However the effectiveness of protections in deferring the attacks needs to be validated, with evidence obtained from empirical assessments of the protection techniques employed by the \esp. At the time of writing, two of such techniques have been assessed, \cite{reganoEmpiric}

% Requirements related to risk monitoring (Section~\ref{sec:esp:problem:mitigation}) are respected, since the solution score is evaluated by the solution solver (see Section~\ref{sec:l1p:solver}) simulating a penetration testing on the application protected with the evaluated solution, with a game-theoretic approach that employs the attack paths inferred in \esp risk assessment phase to evaluate the resistance against threats gained by assets after the deployment of the protection in the evaluated solution on the target application.

% In the validation phase of the \asp project, the experts analyzed the protection solutions inferred by \esp in this phase on the project use-case applications. They were pleased by such solutions, deeming their deployment to the applications effective in deferring possible attacks against the comprised assets. Furthermore, they evaluated the solution as free from inconsistencies that would lead to non-working applications. The overheads introduced were considered acceptable, with a limited impact of the protections employed on user experience.


==> l2p.tex <==
\lstset{language = C, basicstyle = \footnotesize\ttfamily, tabsize = 4, numbers = left, numberstyle = \tiny}

\begin{itemize}
    \item useless intro
\end{itemize}

% This section describes the \esp asset hiding phase. Its main objective is to mitigate a side-effect of software protections, the introduction of \textit{fingerprints}. This term encompasses various characteristics of protected code that an attacker can identify in the binary, thus being able to quickly find the assets in the application. The asset hiding phase refines the protection solution, \ie the combination of protections, inferred in the \esp risk mitigation phase, deploying additional protections on areas of code not marked as assets by the user, thus aiming to confuse the attacker and leading him or her to focus its attack on these code areas that are not sensitive from a security point of view.

% Additional protections are inferred by \esp with the following workflow:
% \begin{enumerate}
% 	\item \textit{\acrshort{milp} model instantiation}: given an asset protection solution (see Section~\ref{sec:l1p:solver}) and the target application source code structure (see Section~\ref{sec:model:app}), \esp infers a \acrfull{milp} problem tailored for the aforementioned code structure, modelling the attacker confusion due to the additional asset hiding protections;
% 	\item \textit{\milp model solving}: an external \milp solver (at the time of writing, \esp supports IBM ILOG CPlex\footnote{\url{https://www.ibm.com/analytics/cplex-optimizer}} and lpsolve\footnote{\url{http://lpsolve.sourceforge.net/}}) is tasked with the solution of the model built in the previous phase of the workflow;
% 	\item \textit{\milp solution translation}: given the model solution obtained in the previous phase, the corresponding additional protection solutions are inferred and used to refine the original asset protection solution.
% \end{enumerate}

\subsection{Protection fingerprints}
\label{sec:l2p:fing}

\begin{itemize}
    \item protection fingerprint definition
    \item static vs. dynamic fingerprints
    \item some examples (CFF flattened graph with figure, virtualization custom bytecode, on-line protections system calls/network packets)
\end{itemize}

% One of the first activities performed by attackers, when they target an application, is identifying the assets in the application binary, in order to focus their attacks on smaller areas of code. This attacker behaviour has been verified empirically, with a study performed on attack reports of professional white-hat hackers \cite{ceccatoTaxonomy}.

% A protection fingerprint is a peculiar characteristic assumed by a code area of the application, after the deployment of one or more protection techniques to it, which can reduce the effort needed by the attacker to locate the protected code area in the binary. Thus, when an attacker targets a protected application, he or she can look for such fingerprints, and can consequently find the assets in the application. In this way, the attacker can focus his or her efforts on the assets code.

% Fingerprints can be subdivided among static and dynamic ones. The first kind of fingerprint can be observed by an attacker using static code analysis tools and code representations, \eg the \cfg of the disassembled application. The second kind of fingerprint is instead noticeable by the attacker during the application execution, examining the latter with a debugger or by analyzing execution traces, collected during execution, after the program termination.

% A first example of static fingerprint is the one introduced into the \cfg of code areas protected with \acrlong{cff}, a code obfuscation technique described in Section~\ref{sec:background:softProt:antiRevEng:codeObf}. Indeed, the protected \cfg assumes a peculiar structure, with a loop with a nested switch statement, with a high number of parallel paths in the \cfg. A depiction of a \cfg protected with \cff is depicted in Fig.~\ref{fig:l2p:cff}. 

% %\begin{figure}[ht]
% %	\centering
% %	\begin{tikzpicture}[sibling distance = 45, level distance = 30]
% %	\node[BasicBlock] (start) {variables declaration} child 
% %	{
% %		node[BasicBlock] (head) {loop head} edge from parent[Flow, level 
% %		distance = 30]
% %		child { node[BasicBlock] (switch0) {case 0} edge from parent[draw = none] }
% %		child { node[BasicBlock] (switch1) {case 1} edge from parent[draw = none] }
% %		child { node[BasicBlock] (switch2) {case 2} edge from parent[draw = none] }
% %		child
% %		{
% %			node[BasicBlock] (switch3) {case 3} edge from parent[draw = none] child[xshift=-2.4cm] { node[BasicBlock] (stop) {return} edge from parent[draw = none,level distance = 22]  }
% %		}
% %	};
% %	
% %	\path[Flow, in = 135, out = 170] (head) edge (switch0);
% %	\path[Flow, in = 135, out = 215] (head) edge (switch1);
% %	\path[Flow, in = 135, out = 260] (head) edge (switch2);
% %	\path[Flow, in = 135, out = 330] (head) edge (switch3);
% %	\draw[Flow, in = 135, out = 330] (head.east) -| ($(switch3.east) + (0.1, 0)$) -| ($(switch3.east) + (0.1, -0.5)$) -| (stop.north);
% %	
% %	\path[Flow, in = 190, out = 45] (switch0) edge (head);
% %	\path[Flow, in = 235, out = 45] (switch1) edge (head);
% %	\path[Flow, in = 300, out = 45] (switch2) edge (head);
% %	\path[Flow, in = -10, out = 45] (switch3) edge (head);
% %	\end{tikzpicture}
% %	\caption{Control flow graph before and after the control flow flattening obfuscation.}
% %	\label{fig:l2p:cff}
% %\end{figure}

% \begin{table*}[ht]
% 	\centering
% 	\begin{tabularx}{\linewidth}{lccX}
% 		\toprule
% 		technique                 & replication & enlargement & shadowing\\
% 		\midrule
% 		anti-debugging            & \High & \High & \None\\
% 		branch functions          & \Low  & \High & \Masking{control flow flattening}{\High}, \Masking{opaque predicates}{\Low}\\
% 		%        call stack checks         & \Low  & \High & \None\\
% 		code mobility             & \High & \High & \Masking{anti-debugging}{\High}, \Masking{branch functions}{\Low}, \Masking{control flow flattening}{\High}, \Masking{opaque predicates}{\Low}, \Masking{virtualization obfuscation}{\High}\\
% 		control flow flattening   & \High & \High & \Masking{opaque predicates}{\Low}\\
% 		%        control flow tagging      & \High & \High & \None\\
% 		opaque predicates         & \High & \High & \Masking{control flow flattening}{\High}\\
% 		virtualization obfuscation & \Low & \Low & \Masking{anti-debugging}{\High}, \Masking{branch functions}{\Low}, \Masking{control flow flattening}{\High}, \Masking{opaque predicates}{\Low}, \Masking{virtualization obfuscation}{\High}\\
% 		static remote attestation & \Low & \High & \None\\
% 		\bottomrule
% 	\end{tabularx}
% 	\caption{Asset hiding strategies for the protection techniques employed by \esp.}
% 	\label{tab:strategies}
% \end{table*}

% Another kind of technique that exposes an evident static fingerprint is virtualization obfuscation, described in Sec.~\ref{sec:background:softProt:antiRevEng:codeObf}. This technique is based on the translation of the code that must be protected into a bytecode, interpreted and executed by a virtual machine specially designed for the protection. Static analysis technique may fail when applied to code protected with such techniques: for example, opcodes of the virtual machine instructions may be invalid for the \cpu architecture, thus leading a disassembler to produce invalid instructions for the code areas protected by the technique. This failure may arise suspect in the attacker, which may be lead to further investigate such protected areas.

% Finally, protections that introduce calls to external libraries can be suspicious for the attacker. For example, on-line protection techniques, such as the one described in \ref{sec:background:softProt:antiTamp}, need to either use external network \glspl{api} or the native socket system calls of the \os. In both cases, the attacker may recognize such calls: especially for applications that do not need a network connection for their business logic, this may lead the attacker to analyze these protected areas of code. Being observable by analyzing the application binary code, fingerprints of this kind are static.

% However, due to the remote connections established at run-time, the on-line protection techniques exhibit also dynamic fingerprints. For example, applications protected with code mobility (see Section~\ref{sec:background:softProt:antiTamp:codeMobility}), when their execution flow reaches a code area moved to the remote server employed by the protection technique, need to download such code from the aforementioned server: also in this case, the opening of such connections, again especially in applications that would not need a remote connection, if not protected with this technique, can raise suspicion in the attacker, and may lead him or her to analyze the code opening such connection in more detail. Also, the attacker may try to eavesdrop the suspicious traffic, thus recovering the asset code moved to the server, if an encrypted connection is not employed.

% Also, code obfuscation techniques introduce dynamic fingerprints on protected code. For example, opaque predicates (see Section~\ref{sec:background:softProt:antiRevEng:codeObf}) may introduce paths in the \cfg that are never traversed by the program flow. An attacker performing a dynamic analysis of the binary, for example with code coverage tools, may identify such paths never taken, and may analyze them, finding the embedded opaque predicates. A methodology for automatically identify and remove opaque predicates in code have been proposed by Dalla Preda\etal\cite{dallaPredaOpaque}.

\subsection{Asset hiding strategies}
\label{sec:l2p:strat}

\begin{itemize}
    \item AH strategies (replication, enlargment, shadowing) to increase critical section
    \item difficulties (excessive AH may decrease AP solution security level + overhead + AH refines a AP solution thus all AP difficulties also apply to AH)
    \item information needed in KB
\end{itemize}

% As reported by software security experts involved in the \asp project, the main solution in the software protection industry to defer the identification of assets by attackers is applying obfuscation to a large part of the program code, protecting also areas of code that do not contain assets. However, this process is performed manually and can be time-consuming. The protected application must be tested to ensure that the additional obfuscation of code has not introduced an excessive overhead in the application, thus the obfuscation and application testing process can be repeated multiple times, until an optimal trade-off between security and overhead is reached. Thus, automating this process, by designing ad-hoc strategies to hide the location of the assets in the binary from attackers, could be useful for security experts.

% This section presents the three \emph{asset hiding strategies} designed for this purpose: fingerprint replication, enlargement and shadowing.

% The \emph{fingerprint replication} involves the insertion in the application of additional fingerprints, devised to have a similar structure to the ones introduced in the \esp asset protection phase. In practice, this is obtained by applying the same protections used in the aforementioned phase on code areas not containing assets. This strategy aims at delaying the attacker, increasing the number of code areas that he or she has to analyze, and potentially making he or she lose time in the analysis of code not holding any value security-wise.

% The \emph{fingerprint enlargement} strategy is based on the extension of the scope of protections deployed on the asset protection phase, deploying them also on code areas adjacent to the assets. In this way, the attacker that finds the location of an asset has to analyze a higher amount of code, thus increasing the time needed to breach the asset security requirements. 
% %
% Finally, the \emph{fingerprint shadowing} strategy conceals the fingerprints introduced in the code during the asset protection phase, deploying other protections on top the ones deployed on assets in the aforementioned phase. 

% For each asset hiding strategy, the effectiveness in hiding the fingerprints introduced by the protection techniques employed by \esp has been evaluated by the software security experts involved in the \asp project, leading to the results reported in Table~\ref{tab:strategies}. The application of each strategy for each protection technique is rated \High when it can be very effective in hiding the fingerprint introduced by the technique, or \Low when applying the strategy for the protection may lead to minimal results.

% For some protection techniques, not all the available strategies are appropriate. For instance, static remote attestation (see Section~\ref{sec:background:softProt:antiTamp:RA}) is not suitable to shadow any kind of fingerprint, since it does not modify the code on which is deployed, but enforces checks on its integrity using ad-hoc external functions typically running on separate threads, as in the case of the implementation of this technique supported by \esp. Instead, different binary obfuscation techniques (see Section~\ref{sec:background:softProt:antiRevEng:codeObf}) may be effectively combined to obtain less noticeable fingerprints. An example is the insertion of opaque predicates in a code region previously protected with \cff, since this may alter the typical \cfg resulting from this technique, depicted in Figure~\ref{fig:l2p:cff}. 

% Indeed, there are protections for which the application of some asset hiding strategies may have the undesired effect of decreasing the global security level of the application. For example, this happens if virtualization obfuscations fingerprints (see Section~\ref{sec:background:softProt:antiRevEng:codeObf}) are replicated or enlarged throughout the code. Such fingerprints are evident for the attacker, as stated in the previous section, due to the custom VM bytecode introduced in the application binary, and the replication and enlargement techniques would be suitable to hide the location of the assets safeguarded by this technique. However, protecting a large amount of code with virtualizations obfuscation may reduce the effort needed by the attacker to reconstruct the mapping between the bytecode instructions and the assembler ones, since he or she would have more bytecode that can be analyzed for this purpose. Thus, the use of this technique in the asset hiding phase must be limited.

% Also, another factor that must be taken into account, when assessing the suitability of a strategy for a protection technique, is the effect of the application of the strategy to the application performances. For example, the system calls introduced in protected code by anti-debugging techniques (see Section~\ref{sec:background:softProt:antiDeb}) may be easily recognizable by an attacker (\eg using tools like strace\footnote{\url{https://www.systutorials.com/docs/linux/man/1-strace/}} in Linux). Thus, using the replication strategy to introduce additional debugging system calls can lead the attacker to analyze non-critical code. Conversely, anti-debugging has non-negligible overhead due to the debugger-debuggee context switches, thus replicating too much this technique fingerprints may lead to an unusable protected application.

% Summarizing, the following factors must be taken into account when deciding the asset hiding additional protections:
% \begin{itemize}
% 	\item effectiveness of each strategy in hiding the protection fingerprints introduced in the asset protection phase;
% 	\item decreased efficacy of some protections techniques in securing the assets, when treated with specific asset hiding strategies;
% 	\item application performance overheads introduced by the asset hiding protections;
% 	\item forbidden precedences among protections, which, as in the asset protection phase (see Section~\ref{sec:l1p:walker}), must not be introduced in the protection solution, since they would lead to a non-working protected application.
% \end{itemize}

% Indeed, computing a good asset hiding solution is not a trivial task, due to the high number of factors influencing the decision of additional protections used for this purpose.

\subsection{Mixed Integer-Linear Programming model}
\label{sec:l2p:milp}

\begin{itemize}
    \item brief useless intro
\end{itemize}
% This section presents the \milp problem that has been devised to model the process of deciding the additional protections that must be used to refine the solution inferred by \esp in the asset protection phase (see Chapter~\ref{sec:l1p}).

% \acrlong{milp} is a branch of operation research, encompassing optimization problems that contain variables constrained to integer values. While there are no previous applications of \milp problems to IT security in literature, decision-making processes in other fields of IT have been often modelled with this optimization technique, especially to tackle resource allocation problems. Indeed, the asset hiding decision process is a problem of this kind, since the overhead introduced by the additional protection constrains the generation of the asset hiding solution. For example, Metwally\etal use \milp problems in cloud IaaS scenarios to efficiently allocate resources in data centers\cite{metwallyMILP}. Also, the book by Sankaralingam \etal on computer architectures \cite{compArchOpt} contains various applications of \milp problems in this field, for example the efficient generation of instruction sets for application-specific processors. Furthermore, various decision processes in the telecommunications field are solved using this optimization technique \cite{bezzinaFemtoc,liKimOptical}. 

\subsubsection{Application structure and protections}
\label{sec:l2p:milp:app}

\begin{itemize}
    \item modeling of KB application structure in MILP model
    \item code region with containment/precedence/adjacency relationships
    \item protections, protection/PI/DPI spaces, AP/AH solutions posets
    \item forbidden/discouraged precedences, singleton protections
    \item overheads as precomputed linear combination of metrics (this should be added also in a possible threat to validity section)
    \item cut everything needed only in constraint formulas
\end{itemize}

% This section reports on how the data contained in the \esp \ekb needed to drive the asset hiding phase, in particular the target application code structure and the protection techniques supported by \esp, is formalized in mathematically in order to employ it in the \milp problem. \esp can analyze code written in the C and C++ programming languages.

% \emph{Code Regions}
% A code region, denoted in the with $\codeRegion{}$, is a piece of code that is syntactically valid if parsed in isolation, and is individuated by specifying the source code file containing it, the starting and ending lines of the code comprised in the code region.
% %
% The functions $\source{}$, $\sLine{}$ and $\eLine{}$ return respectively a reference to the source file (\eg a path or an ID), the starting and ending line of a code region $\codeRegion{}$.
% All the code regions that can be defined in the source code of the target application form the \emph{code region space} $\codeRegionSpace$, while the ones that are taken into account to carry out the \LDP phase form the \emph{reduced code region space} $\reducedCodeRegionSpace \subseteq \codeRegionSpace$. All the code regions protected after the \LUP phase belong to $\reducedCodeRegionSpace$, since they constitute the starting point for the asset hiding phase.

% A \CR may contain another one, thus a \emph{containment relation} is needed in the code region space. 
% A code region $\codeRegion{i}$ strictly contains $\codeRegion{j}$ if $\source{i}=\source{j} \land \sLine{i}\leq\sLine{j} \land \eLine{i}\geq\eLine{j} \land (\sLine{i}<\sLine{j} \lor \eLine{i}>\eLine{j})$, \ie if they are comprised in the same source file and $\codeRegion{i}$ includes the lines of code constituting the $\codeRegion{j}$. Thus, this relation allows to represent the \CR comprised in a source code file with a tree-like structure, with non overlapping siblings nodes, and ancestor nodes strictly containing their descendants. Thus, a function or class method is represented as a code region completely wrapping its body. Similarly, an application is a forest of code region trees, each of them representing one of the application source code files. An example of \CR tree, obtained from a C snippet, is depicted in Fig.~\ref{fig:codeRegionsExample}.

% %\begin{figure}[t]
% %	\centering
% %	\begin{minipage}[b]{0.4\linewidth}
% %		\centering
% %		\begin{lstlisting}[xleftmargin=1.8cm]
% %if (y == 7)
% %	n = 1;
% %else
% %{
% %	r = 7 + y;
% %	x = FALSE;
% %	y++;
% %	n <<= 3;
% %}
% %n--;
% %		\end{lstlisting}
% %		\subcaption{C source code.}
% %	\end{minipage}
% %	\begin{minipage}[b]{0.4\linewidth}
% %		\centering
% %		\begin{tikzpicture}[every node/.style = {CodeRegion}, sibling distance 
% %		= 35, level distance = 28, label distance=-7]
% %		\node [label={[fill=none, draw=none, text opacity=1,fill 
% %			opacity=0, minimum height = 0, minimum width = 0, 
% %			font=\tiny]90:1--10}] {$\codeRegion{1}$}
% %		child { node [label={[fill=none, draw=none, text opacity=1,fill 
% %				opacity=0, minimum height = 0, minimum width = 0, 
% %				font=\tiny]90:1--9}] {$\codeRegion{2}$}
% %			child { node [label={[fill=none, draw=none, text 
% %					opacity=1,fill opacity=0, minimum height = 0, minimum width 
% %					= 0, font=\tiny]90:2--2}] {$\codeRegion{4}$} }
% %			child { node [label={[fill=none, draw=none, text 
% %					opacity=1,fill opacity=0, minimum height = 0, minimum width 
% %					= 0, font=\tiny]90:5--8}] {$\codeRegion{5}$}
% %				child { node [label={[fill=none, draw=none, text 
% %						opacity=1,fill opacity=0, minimum height = 0, minimum 
% %						width = 0, font=\tiny]90:5--5}] {$\codeRegion{6}$} }
% %				child { node [label={[fill=none, draw=none, text 
% %						opacity=1,fill opacity=0, minimum height = 0, minimum 
% %						width = 0, font=\tiny]90:6--6}] {$\codeRegion{7}$} } 
% %				child { node [label={[fill=none, draw=none, text 
% %						opacity=1,fill opacity=0, minimum height = 0, minimum 
% %						width = 0, font=\tiny]90:7--7}] {$\codeRegion{8}$} } 
% %				child { node [label={[fill=none, draw=none, text 
% %						opacity=1,fill opacity=0, minimum height = 0, minimum 
% %						width = 0, font=\tiny]90:8--8}] {$\codeRegion{9}$} } 
% %			} 
% %		}
% %		child { node [label={[fill=none, draw=none, text opacity=1,fill 
% %				opacity=0, minimum height = 0, minimum width = 0, label 
% %				distance=-13.5, font=\tiny]90:\quad10--10}] {$\codeRegion{3}$} 
% %		};
% %		\end{tikzpicture}
% %		\subcaption{code region tree.}
% %	\end{minipage}
% %	\caption{Code regions tree representing a C source code.}
% %	\label{fig:codeRegionsExample}
% %\end{figure}

% A partial order among code regions in the same tree can also be established. A code region $\codeRegion{i}$ \emph{precedes} (or \emph{follows}) the code region $\codeRegion{j}$ iff $\source{i} = \source{j} \wedge \parent{i} = \parent{j} \wedge \eLine{i} < \sLine{j}$. These relationships are indicated
% with the notation $\codeRegion{i} \Prec \codeRegion{j}$ (or $\codeRegion{i} 
% \Succ \codeRegion{j}$).

% Also, a way to tell if two code regions are adjacent is needed, when deciding if the enlargement technique can be deployed, since two adjacent code regions can be merged and protected with the same pass. The function $\prox{i}{j} \in \biSet$ is used for this purpose:

% \begin{equation*}
% \prox{i}{j} = 
% \begin{cases}
% 1 & \text{if $\left(\codeRegion{i} \Prec \codeRegion{j}\right) \wedge \left(\nexists \codeRegion{k} : \codeRegion{i} \Prec \codeRegion{k} \Prec \codeRegion{j}\right)$}\\
% 0 & \text{otherwise}
% \end{cases}
% \end{equation*}


% \emph{Protections}
% Protections and their application to code regions must be formally modelled, since asset hiding strategies are implemented by applying protections to the code.
% First, the symbol $\protection{i}$ denotes a \emph{protection} technique, while a protection instance (a protection with all the related configuration parameters, see Section~\ref{sec:model:prot}) is represented with the symbol $\protectionInstantiation{j}$; thus, $\protectionInstantiation{j}  \in \protection{i}$. The function $\prot{j} = \protection{i}$ returns the protection technique implemented by the protection instance $\protectionInstantiation{j}$.
% %
% The \emph{protection instantiation space} $\protectionInstantiationSpace$ is 
% the set of all the PIs contained in, which is $\protectionInstantiationSpace = 
% \bigcup_i P_i$. % = \{ p_i \}_i$. 
% The symbol $\protectionInstantiationSpaceLOneP$ indicates the restriction of $\protectionInstantiationSpace$ to the \glspl{pi} only used in the \LUP phase.
% Finally, the notation $\appliedProtectionInstantiation{}{}$ indicates an \acrfull{dpi}, representing the use of a \PI $\protectionInstantiation{}$ to protect the code region $\codeRegion{}$.

% An \emph{\LUP solution} is the output of the asset protection phase, and is defined formally as a poset of deployed \glspl{pi} (see Chapter~\ref{sec:l1p}). The order of two deployed \glspl{pi} $\appliedProtectionInstantiation{i}{j}$ and $\appliedProtectionInstantiation{k}{l}$ only matters if $\codeRegion{j}$ and $\codeRegion{l}$ share at least one line of code, \ie $\codeRegion{j} = \codeRegion{l}$, $\codeRegion{l}\in\ancestors{j}$ or $\codeRegion{l}\in\descendants{j}$.
% %
% Similarly, the \emph{\LDP solution} is the poset of deployed \glspl{pi} generated by the \LDP phase, refining the \LUP solution. To ease comprehension of the model, two helper functions are introduced. $\lOneP{}{} \in \biSet$ verifies if $\appliedProtectionInstantiation{}{}$ is in the \LUP solution. $\rLOneP{}{} \in \biSet$ checks if $\protectionInstantiation{}$ is deployed to some code regions contained in $\codeRegion{}$, \ie code regions that are descendants of $\codeRegion{}$.


% \begin{equation*}
% \lOneP{}{} =
% \begin{cases}
% 1 & \text{if $\appliedProtectionInstantiation{}{}$ is in the \LUP solution}\\
% 0 & \text{otherwise}
% \end{cases}
% \end{equation*}

% \begin{equation*}
% \rLOneP{}{} =
% \begin{cases}
% 1 &\text{if $\exists \codeRegion{i} \in 
% 	\operatorname{descendants}(\codeRegion{}): \lOneP{}{i} = 1 $}\\
% 0 &\text{otherwise}
% \end{cases}
% \end{equation*}

% Also, a distinction must be made between horizontal and vertical enlargement.
% The first is enforced enlarging a \DPI in the \LUP solution to contiguous code regions, \eg referring to the code depicted to Fig.~\ref{fig:codeRegionsExample}, if the \DPI 
% $\appliedProtectionInstantiation{i}{7}$ is enlarged to the code regions $\codeRegion{6}$, $\codeRegion{8}$ or $\codeRegion{9}$. Vertical enlargement instead happens when a \DPI is enlarged to a code region that contains it, \eg in Fig.~\ref{fig:codeRegionsExample}, if 
% $\appliedProtectionInstantiation{i}{7}$ is enlarged to $\codeRegion{5}$, $\codeRegion{2}$ or $\codeRegion{1}$. 
% %For coherence purposes, before vertically enlarging an deployed \PI, it must have been horizontally enlarged to all the siblings of the originally protected code region.
% %\todo{l'ultima frase mi pare superflua e sbagliata, e se ci sono buchi tra le code region sibling?}

% \emph{Dependencies Among Protections}

% As already detailed in Section~\ref{sec:l1p:walker}, some orderings among the protections in a protection solution are not valid, since applying protections using such orderings would lead to a non-working application. Thus, a partial ordering is needed among protections $\protection{i}$. Formally, a protection $\protection{i}$ is a \emph{forbidden precedence} of
% another protection $\protection{j}$ if $\appliedProtectionInstantiation{i}{k}$ cannot be present before $\appliedProtectionInstantiation{j}{l}$ in a valid solution, for all the intersecting code regions $\codeRegion{k}$ and $\codeRegion{l}$. % or $\codeRegion{k}\in\descendants{\codeRegion{l}}$. 
% Also, a \emph{singleton} protection (see Section~\ref{sec:l1p:walker}) cannot be deployed more than once to the same code region. An example of this kind of protection is code mobility (see Section~\ref{sec:background:softProt:antiTamp:codeMobility}), since code can be moved to the trusted server only once.

% Regarding the protection overheads, they are computed by \esp for all the code regions $\codeRegion{} \in \reducedCodeRegionSpace$ during the generation of the model, using the formulas described in Section~\ref{sec:l1p:metrics:overhead}, and in the model are comprised in the set ${\overh{j}}$. Given a \DPI $\appliedProtectionInstantiation{}{}$, $\overheadd{j}{}{}{}$ indicates that ${\overh{j}}$ computation is based on the metrics $\metric{1}{}, \metric{2}{}, \dots$ computed on $\codeRegion{}$. Since overheads are precomputed prior to model generation, and their dependency to metrics is not needed in the definition of the model, the compact notation $\overhead{j}{}{}$ will be used in the remainder of the chapter for the sake of readability.

\subsubsection{Domain Parameters}
\label{sec:l2p:param}

\begin{itemize}
    \item constant $\protectionInstantiationSpaceMax$ (max number of deployment of a PI to the same code region) to bound the problem
    \item confusion index proportional to attacker delay = MILP goal is maximizing confusion index
    \item asset hiding strategies formulas composing the confusion index
\end{itemize}

% The MILP model is built taking into account the reduced code region space $\reducedCodeRegionSpace = \{ \codeRegion{1}, \codeRegion{2}, \dots \}$ and the \PIset used in the \LUP solution $\protectionInstantiationSpaceLOneP = \{ \protectionInstantiation{1}, \protectionInstantiation{2}, \dots \}$. 

% The constant $\protectionInstantiationSpaceMax$ specifies the maximum number of times a \PI can be deployed on the same code region. The symbol $\overheadMax{i}$ indicates the user-defined upper bound for the $i$-th overhead type.

% The \milp model goal is maximizing the delay introduced by the \LDP solution to tasks performed by the attacker.
% %
% Thus, a way to estimate the delay introduced by every \DPI is needed. The \emph{confusion index} is introduced for this purpose. It is a parameter built to be proportional to the delay, but it is not intended to estimate the actual time needed by an attacker to find the application assets. In other words, while increasing the confusion index induces an increase in time needed by the attacker, other properties, \eg a formula to translate it into a measure of attacker time, cannot be deduced. This represents a limitation of the current model. However, a mapping could be devised in the future, executing empirical assessments of the time needed by an attacker to find the assets in a protected application.

% The set $\techniques$ contains the \LDP strategies, \ie $\techniques = \{ \replication, \enlargement, \shadowing \}$ where $\replication$ is fingerprint replication, $\enlargement$ is fingerprint enlargement, and $\shadowing$ is fingerprint shadowing.
% % 
% A strategy-specific formula returns, for each \DPI, the confusion index. The latter is dependent from the code region complexity metrics (see Section~\ref{sec:l1p:metrics:metrics}). The confusion indices associated to each deployed \PI are used  in the objective function as multiplicative factors, also called \emph{bonuses} in the remainder of the chapter.

% Strategy formulas can be unary, such as $\confusionLong{\replication}{i}{\metric{1}{},\metric{2}{},\dots}$ and  $\confusionLong{\enlargement}{i}{\metric{1}{},\metric{2}{},\dots}$, which return the confusion index introduced by applying  $\appliedProtectionInstantiation{i}{}$ to enforce the strategy $s \in \{ \replication, \enlargement \}$. Alternatively, formulas may be binary. For example fingerprint shadowing is associated with this kind of formulas, where $\confusionShadowingLong{i}{j}{\metric{1}{},\metric{2}{},\dots}$ returns the confusion index introduced by shadowing the $\appliedProtectionInstantiation{j}{}$ fingerprint, using the \DPI $\appliedProtectionInstantiation{i}{}$.
% $\confusionShadowingLong{i}{j}{\metric{1}{},\metric{2}{},\dots}$ are bounded between $0$ and $1$:
% $\confusionShadowingLong{i}{j}{\metric{1}{},\metric{2}{},\dots}=1$, if applying $\appliedProtectionInstantiation{i}{}$ on top of $\appliedProtectionInstantiation{j}{}$ completely masks the fingerprint of $\appliedProtectionInstantiation{j}{}$, and $\confusionShadowingLong{i}{j}{\metric{1}{},\metric{2}{},\dots}=0$ implies that applying $\appliedProtectionInstantiation{i}{}$ on top of $\appliedProtectionInstantiation{j}{}$ have not effect in masking the $\appliedProtectionInstantiation{j}{}$ fingerprint. Confusion indices are computed during the MILP model generation phase, thus the simplified notation $\confusion{\replication}{i}{}$, $\confusion{\enlargement}{i}{}$ and $\confusionShadowing{i}{j}{}$ will be used when the reference to metrics of code region $\codeRegion{}$ is not needed.

\subsubsection{Linear Problem}
\label{sec:l2p:milp:milp}

\begin{itemize}
    \item MILP variables needed in the objective function
    \item brief discussion of constraints needed to obtain a valid AH solution, without any formulas (ref to STM paper)
    \item MILP objective function
\end{itemize}

% In this section, the \acrfull{milp} problem to decide the asset hiding protection is defined. Its goal is the maximization of the confusion index using the strategies in the set $\techniques$. The model is a specialization of the well-known Knapsack Problem (KP), using multiple capacity constraints to limit the introduced overhead. The examples provided in the model presentation are referred to the code region tree in 
% Figure~\ref{fig:codeRegionsExample}.

% \emph{Variables}
% First, the \milp variables are introduced.
% %
% The variable $\mainVariable{i}{j} \in \biSet$ is set to $1$ iff the \PI $\protectionInstantiation{i}$ will be deployed either directly to the code region $\codeRegion{j}$, or to another that contains it, \ie in $\codeRegion{k}\in\ancestors{j}$. For instance, if $\mainVariable{i}{2}=1$, then the \LDP solution either contains $\appliedProtectionInstantiation{i}{2}$, or $\appliedProtectionInstantiation{i}{1}$, since a protection deployed on a code region is implicitly deployed to all the code regions inside it.
% %\todo[inline]{uniformare exploration algorithm che mi pare abbia cambiato nome}
% %This decision is made by the exploration algorithm, described later in Section~\ref{sec:exploration}. 

% %Note that the \LDP solution will always contain all the \LUP deployed \glspl{pi} or their enlargement, so that $\lOneP{\appliedProtectionInstantiation{i}{\codeRegion_j}} = 1 \implies \mainVariable{\appliedProtectionInstantiation{i}{\codeRegion_j}} = 1$ holds.

% %We force the \LDP solution as a poset, we express in 
% The ordering between two \glspl{pi} deployed to the same code region is modelled using the binary variable $\orderVariable{i}{j}{k}$, \ie $\orderVariable{i}{j}{k}=1$ iff $\protectionInstantiation{j}$ and $\protectionInstantiation{k}$ are both deployed on $\codeRegion{i}$ and in this order. 
% It is zero if the protections are deployed in the reverse order or if either $\mainVariable{j}{i} = 0$ or $\mainVariable{k}{i} = 0$. 
% Clearly, it is not possible for two inverse variables $\orderVariable{i}{j}{k}$ and $\orderVariable{i}{k}{j}$ to be both equal to 1. Referring to the example code, given $\mainVariable{1}{1}=1$ and $\mainVariable{2}{1}=1$, if the $\orderVariable{1}{1}{2}=1$ then $\protectionInstantiation{1}$ will be deployed
% to $\codeRegion{1}$ before $\protectionInstantiation{2}$, and $\orderVariable{1}{1}{2}$ will be forced to 0. 

% This behavior is imposed introducing the following constraints, \ie if both $\mainVariable{j}{i}$ and $\mainVariable{k}{i}$ are equal to 1, only one of the two variables $\orderVariable{i}{j}{k}$ and 
% $\orderVariable{i}{k}{j}$ must be equal to 1, otherwise both $\orderVariable{i}{j}{k}$ and $\orderVariable{i}{k}{j}$ must be equal to 0:
% \[
% 0 \leq -2 \orderVariable{i}{j}{k} -2 \orderVariable{i}{k}{j} + \mainVariable{j}{i} + \mainVariable{k}{i} \leq 1, \forall i, j, k
% \]

% A second set of constraints avoid the insertion of cycles in the ordering of protections deployed to the same code region (for more than three protections). In other words, loops like $\orderVariable{i}{j}{k} = \orderVariable{i}{k}{l} = \orderVariable{i}{j}{l} = 1$ are avoided. This is obtained with the following constraints:
% \[
% \orderVariable{i}{j}{k} - \orderVariable{i}{k}{l} - \orderVariable{i}{j}{l} \le -1,\forall i, j, k, l : j \ne k \ne l
% \]

% Also, the model forces $\orderVariable{i}{j}{k} = 0$ if $\protectionInstantiation{j}$ is a forbidden precedence for $\protectionInstantiation{k}$.

% The binary variables $\proxVariable{i}{j}{k}$, which are defined only for adjacent code regions $\codeRegion{i}$ and $\codeRegion{j}$, are used to decide if two code regions must be merged when deploying protections (horizontal enlargement). % such that $\prox{i}{j}=1\ \wedge\ \eLine{i} < \sLine{j}$.
% If $\proxVariable{i}{j}{k} = 0$ and $\mainVariable{k}{i} = \mainVariable{k}{j} = 1$, two separate \glspl{dpi} $\appliedProtectionInstantiation{k}{i}$ and $\appliedProtectionInstantiation{k}{j}$ will be comprised in the \LDP solution.
% % 
% If $\proxVariable{i}{j}{k} = 1$, the \LDP solution will contain a \DPI 
% $\appliedProtectionInstantiation{k}{l}$, where $\codeRegion{l}$ comprises the union of code regions $\codeRegion{i}$ and $\codeRegion{j}$. In the example, if $\appliedProtectionInstantiation{1}{7}$ is in the \LUP solution and $\proxVariable{6}{7}{1}=1$, then the \LDP solution will contain $\appliedProtectionInstantiation{1}{10}$, where $\codeRegion{10}$ is a code region $\codeRegion{6}\cup\codeRegion{7}$. 
% If, otherwise, $\proxVariable{6}{7}{1}=0$, then the \LDP solution will contain $\appliedProtectionInstantiation{1}{6}$ and $\appliedProtectionInstantiation{1}{7}$.

% Furthermore, $ \proxVariable{i}{j}{k} = 1$ implies $\mainVariable{k}{i} = \mainVariable{k}{j} = 1$, obtained imposing the following set of constraints:
% \begin{gather*}
% 2 \proxVariable{i}{j}{k} - \mainVariable{k}{i} - \mainVariable{k}{j} \leq 
% 0, \quad \forall i, j, k : \prox{i}{j} = 1
% \end{gather*}

% Some other variables are needed to correctly process the bonuses used in the objective function. Replications must be avoided, \ie since the same operation can be interpreted as a consequence of more strategies, \eg enlargement and shadowing. Furthermore, containment relations must be managed, so that while $\mainVariable{i}{j}=1$ forces $\mainVariable{i}{k}=1$ for all its descendants $\codeRegion{k}$, the bonus is considered only for the larger code region.

% Thus, the additional binary variables  $\enlargementVariable{i}{j}{k} \in \biSet$ are introduced, representing enlargements spanning both horizontally and vertically to increase the code that must be protected. To compute the bonuses of descendants in a proper way, the $\enlargementVariable{i}{j}{k}$ keep track of protections deployed due to enlargements.
% %
% An example can be made considering a deployed \PI $\appliedProtectionInstantiation{1}{7}$ in the \LUP solution, which, during the \LDP phase, is first vertically enlarged to $\codeRegion{5}$; then, $\codeRegion{5}$ is enlarged to $\codeRegion{4}$. In this case $\enlargementVariable{4}{5}{1}=1$, since $\protectionInstantiation{1}$ has been deployed to $\codeRegion{4}$ to enlarge the \LUP \DPI $\appliedProtectionInstantiation{1}{7}$, and  $\codeRegion{4}$ is a sibling of $\codeRegion{5}$, which contains the originally protected code region $\codeRegion{7}$.
% %
% Generalizing, the variable $\enlargementVariable{i}{j}{k}$ set to $1$ means that the \LDP solution contains a \PI $\protectionInstantiation{k}$ deployed to a code region containing both $\codeRegion{i}$ and $\codeRegion{j}$, due to an enlargement of the \PI $\protectionInstantiation{k}$ that in the \LUP solution was originally deployed either to $\codeRegion{j}$ or one of its descendants.
% %The reason for this additional set of variables is to keep track of the reason for the application of a \PI on a given code area to properly manage the bonuses of descendant code regions in the objective function.

% The $\enlargementVariable{i}{j}{k}$ summarizes complex enlargements, thus they can be obtained as composition of the $\proxVariable{i}{j}{k}$, which define simple enlargements:
% \begin{equation}\label{eq:enlargementVariables}
% \enlargementVariable{i}{j}{k} = \bigwedge_{\proxVariable{l}{m}{k} \in \proxSet{i}{j}{k}} \proxVariable{l}{m}{k}
% \end{equation}
% where $\proxSet{i}{j}{k}$ reports the individual $\proxVariable{}{}{}$ affected by the complex enlargement:
% \begin{equation}
% \proxSet{i}{j}{k} = \{ \;  \proxVariable{l}{m}{k} \, : \,  
% \rLOneP{k}{j} \wedge \left(\codeRegion{i} \PrecEq \codeRegion{l} \Prec \codeRegion{m} \PrecEq 
% \codeRegion{j} \vee \codeRegion{j} \PrecEq \codeRegion{l} \Prec 
% \codeRegion{m} \PrecEq \codeRegion{i}\right)   
% \; \}
% \end{equation}

% For example, if $\appliedProtectionInstantiation{1}{6}$ is in the \LUP solution and $\appliedProtectionInstantiation{1}{8}$ is the consequence of two enlargements, first from $\codeRegion{6}$ to $\codeRegion{7}$ ($\proxVariable{6}{7}{1}=1$) and then from $\codeRegion{7}$ to $\codeRegion{8}$ ($\proxVariable{7}{8}{1}=1$), this leads to  $\proxSet{6}{8}{1}=\{\proxVariable{6}{7}{1},\proxVariable{7}{8}{1}\}$ and  $\enlargementVariable{6}{8}{1}=\proxVariable{6}{7}{1}\wedge\proxVariable{7}{8}{1}=1$.

% It is also necessary to identify if a \DPI derives from an enlargement or replication, in order to compute the bonuses properly, because these two techniques are mutually exclusive. To this purpose, the auxiliary binary variables $\techniqueVariable{i}{j}$ are introduced in order to identify which $\mainVariable{}{}$ are set to $1$ in the \LDP model solution due to fingerprint enlargements.
% %
% We have $\techniqueVariable{i}{j}=1$ when $\protectionInstantiation{i}$ has been deployed to $\codeRegion{j}$ for enlarging an \DPI in the \LUP solution or $0$ if another technique has been used, which is

% \begin{equation}\label{eq:techniqueVariables}
% \techniqueVariable{i}{j} = \bigvee_{\enlargementVariable{j}{k}{i} \in 
% 	\enlargementSet{i}{j}} \enlargementVariable{j}{k}{l}
% \end{equation}
% %
% where $\enlargementSet{i}{j}$ includes the variables that may indicate if \glspl{pi} deployed to the siblings $\codeRegion{k}$ of $\codeRegion{j}$ are consequence of complex enlargements.
% %
% \begin{align*}
% \enlargementSet{i}{j} = \{ \; \enlargementVariable{j}{k}{i} \, : \,\rLOneP{i}{k} = 1 \wedge\parent{j} = \parent{k} \; \}
% \end{align*}

% Fingerprint shadowing and replication (or enlargement) are not mutually exclusive, thus when enlarging or replicating a \DPI a fingerprint of another \DPI may be shadowed. In this case, replicating the bonuses cannot happen, thus is not needed to this case not need to manage this case explicitly. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \emph{Objective Function}
% The following objective function is used by the \milp model, aiming to maximize the confusion index:

% \begin{align*}
% o.f.~\max \Bigg( &
% \sum_{\codeRegion{i} \in \reducedCodeRegionSpace} 
% \sum_{\protectionInstantiation{j} \in 
% 	\protectionInstantiationSpaceLOneP} \bonus{\replication}{j}{i} 
% (\mainVariable{j}{i} - \techniqueVariable{j}{i}) + \\
% & \sum_{\codeRegion{i} \in \reducedCodeRegionSpace} 
% \sum_{\protectionInstantiation{j} \in 
% 	\protectionInstantiationSpaceLOneP} \bonus{\enlargement}{j}{i} 
% \rLOneP{j}{i} \mainVariable{j}{i} +\\
% & \sum_{\codeRegion{i} \in \reducedCodeRegionSpace} 
% \sum_{\protectionInstantiation{j}\in 
% 	\protectionInstantiationSpaceLOneP}
% \sum_{\codeRegion{k} \in \reducedCodeRegionSpace} 
% \bonus{\enlargement}{j}{i} 
% \enlargementVariable{i}{k}{j} + \\
% & \sum_{\codeRegion{i} \in \reducedCodeRegionSpace} 
% \sum_{\protectionInstantiation{j} \in 
% 	\protectionInstantiationSpace} 
% \bonus{\shadowing}{j}{i}
% \Bigg)
% \end{align*}

% The first summation takes into account the replication strategy and it uses the $\bonus{\replication}{j}{i}$ factor. As anticipated, the $\techniqueVariable{j}{i}$ variables distinguish if enlargement or replication have been deployed. Subtracting the $\techniqueVariable{j}{i}$ ensures that replication contributions are properly computed. The bonus is computed recursively on each code region tree:
% $$\bonus{\replication}{j}{i} = \confusion{\replication}{j}{i} - 
% \sum_{\codeRegion{k} \in \descendants{i}} \bonus{\replication}{j}{k}$$
% It should be noted that confusion indices of all the descendant code regions are subtracted to avoid duplications, since the summation in the objective function will consider them because it spans over all the code regions.

% The second and third summations respectively report the contribution of the vertical and 
% horizontal enlargement. 
% The enlargement bonus $\bonus{\enlargement}{j}{i}$ must ensure that only the deployed \glspl{pi} that are consequence of some enlargement of deployed \glspl{pi} in the \LUP solution are considered.
% To this purpose, the vertical enlargement uses the $\rLOneP{j}{i}$ as an explicit multiplying factor.
% The horizontal enlargement uses the $\enlargementVariable{i}{k}{j}$ variables, which have been defined ad hoc. %also consider because the latter can be equal to $1$ only if $\protectionInstantiation{j}$ is deployed to a descendant of $\codeRegion{k}$ in the \LUP solution. 
% As before, the enlargement bonus is computed recursively and the confusion indices are subtracted:
% $$\bonus{\enlargement}{j}{i} = \confusion{\enlargement}{j}{i} - \sum_{\codeRegion{k} \in \descendants{i}} \bonus{\enlargement}{j}{k}$$


% %The factors $\bonus{\replication}{j}{i}$ and $\bonus{\enlargement}{j}{i}$ can 
% %be declared in several ways, but a simple recursive definition 
% %is:
% %
% %\begin{equation*}
% %    \begin{cases}
% %        \bonus{\replication}{j}{i} & = \confusion{\replication}{j}{i} - 
% %        \sum_{\codeRegion{k} \in \descendants{i}} \bonus{\replication}{j}{k}\\
% %        \bonus{\enlargement}{j}{i} & = \confusion{\enlargement}{j}{i} - \sum_{\codeRegion{k} \in \descendants{i}} \bonus{\enlargement}{j}{k}
% %    \end{cases}
% %\end{equation*}


% Finally, the fourth summation takes into account the fingerprint shadowing, and 
% similarly to the other summations use a shadowing bonus 
% $\bonus{\shadowing}{j}{i}$.
% %
% The $\bonus{\shadowing}{j}{i}$ bonus indicates how well the $\appliedProtectionInstantiation{j}{i}$ fingerprint is masked by the protections deployed on top of it. 
% As for $\confusionShadowing{k}{j}{i}$, the $\bonus{\shadowing}{j}{i}$ bonuses are in $[0,1]$, where $\bonus{\shadowing}{j}{i}=1$ means that the fingerprint of $\appliedProtectionInstantiation{j}{i}$ is completely masked and  $\bonus{\shadowing}{j}{i}=0$ means no shadowing at all. % by the protections deployed on top of it in the \LDP solution. 
% Since the value of $\bonus{\shadowing}{j}{i}$ is between $0$ and $1$, it is ensured that when a fingerprint has been already completely masked, no additional bonus is given if protections are added. % when adding protections that mask the aforementioned fingerprint. 

% The bonus $\bonus{\shadowing}{j}{i}$ is evaluated by summing up the $\confusionShadowing{k}{j}{i}$ of all the $\appliedProtectionInstantiation{k}{i}$ deployed to shadow $\appliedProtectionInstantiation{j}{i}$, which are recognized because $\orderVariable{i}{j}{k}=1$. 
% If the summation exceeds $1$, the bonus $\bonus{\shadowing}{j}{i}$ is set to $1$.

% Since $\bonus{\shadowing}{j}{i}$ increases the objective function value, its evaluation is obtained by introducing the following set of constraints:

% $$\begin{array}{lclcl}
% 0&\leq&\bonus{\shadowing}{j}{i}& \leq & 1\\
% &    &\bonus{\shadowing}{j}{i}& \leq & \sum_{\protectionInstantiation{k} \in \protectionInstantiationSpace}\confusionShadowing{k}{j}{i} \cdot \orderVariable{i}{j}{k}
% \end{array}$$

% %Hiding of highly critical assets may be prioritized, 
% Simply increasing the bonuses, assets and strategies may be prioritized, e.g. by weighting the objective function summations or by using multiplicative factors that take into account the importance of the asset.

% Finally, the $\enlargementVariable{i}{j}{k}$ (defined in Equation~\ref{eq:enlargementVariables}) and $\techniqueVariable{i}{j}$ (defined in Equation~\ref{eq:techniqueVariables}) are linearized as follows:

% \begin{equation*}
% \begin{cases}
% \enlargementVariable{i}{j}{k} \le \frac{\sum_{\proxVariable{l}{m}{k} \in \proxSet{i}{j}{k}} \proxVariable{l}{m}{k}}{\left| \proxSet{i}{j}{k} \right|} & \text{if $\left| \proxSet{i}{j}{k} \right| > 0$}\\
% \enlargementVariable{i}{j}{k} = 0 & \text{otherwise}
% \end{cases}
% \end{equation*}

% %Analogously, we can linearise the $\techniqueVariable{i}{j}$ variables, defined in Equation~\ref{eq:techniqueVariables}: %, but, since they lower the o.f. value, we must invert their inequalities:

% \begin{equation*}
% \begin{cases}
% \techniqueVariable{i}{j} \ge \frac{\sum_{\enlargementVariable{l}{m}{i} 
% 		\in \enlargementSet{i}{j}} \enlargementVariable{l}{m}{i}}{\left| 
% 	\enlargementSet{i}{j} \right|} & \text{if $\left| \enlargementSet{i}{j} 
% 	\right| > 0$}\\
% \techniqueVariable{i}{j} = 0 & \text{otherwise}
% \end{cases}
% \end{equation*}

% \emph{Additional Constraints}
% As described in Chapter~\ref{sec:background}, the \LDP solution must not exceed the user-defined overheads.
% Therefore a set of inequalities are introduced, constituting the KP-problem capacity constraints:

% \begin{equation*}
% \sum_{\codeRegion{j} \in \reducedCodeRegionSpace} 
% \sum_{\protectionInstantiation{i} \in \protectionInstantiationSpaceLOneP} 
% \mainVariable{i}{j} \localOverhead{o}{i}{j} \le \overheadMax{o}, \quad 
% \forall o
% \end{equation*}
% %
% where $\localOverhead{o}{i}{j}$ is a constant defined as:
% %
% \begin{equation*}
% \localOverhead{o}{i}{j} = \overhead{o}{i}{j} - \sum_{\codeRegion{k} \in 
% 	\descendants{j}} \localOverhead{o}{i}{k}
% \end{equation*}

% It should be noted that also in this case, the code regions' overheads added by the descendants must be subtracted, since they would be counted more than once during the double summation.

% Containment among code regions may also have consequences on the order and applicability of protections. First, if the set of protection deployed to a code region is different from the 
% ones deployed to its parent, then the deployed protections associated with the 
% child but not to the parent must be deployed before the protections that are 
% deployed to both. Second, if a set of \glspl{pi} is deployed to a code region, the same set of \glspl{pi} must be deployed to all its descendant code regions and in the same order. 
% %On the other hand, if a \PI is deployed to a code region but not to one of its ancestors, it must be first deployed on the code region itself before applying all the other \glspl{pi}, if needed. In order to define these constraints we will use the following set:


% Consequently, the MILP model contains three additional sets of constraints, which use the following set of variables that regulate the possibility to merge adjacent code regions:
% \begin{equation*}
% \orderSet{i}{j} = \{ \; \proxVariable{k}{l}{i} \, : \, \parent{k} = \parent{l} =  \codeRegion{j} \; \}
% \end{equation*}


% The first set of constraints ensures that deployed a \PI to a code region 
% implies that it must be deployed to all the merged children code regions, and 
% formally, they are the AND of variables in $\orderSet{i}{j}$:
% \begin{equation*}
% \left| \orderSet{i}{j} \right| \mainVariable{i}{j} - 
% \sum_{\proxVariable{k}{l}{i} \in \orderSet{i}{j}} 
% \proxVariable{k}{l}{i} \leq 0, \forall i, j, k, l
% \end{equation*}
% That is, $\mainVariable{i}{j}=1$ forces the $\proxVariable{k}{l}{j}=1$ for all the adjacent children $\codeRegion{k}$ and $\codeRegion{l}$ of $\codeRegion{j}$.

% The second set of constraints guarantees that if two \glspl{pi} are deployed to a code region, they are  deployed in the same order to all the children code regions, which is:
% \begin{equation*}
% \orderVariable{i}{j}{k} \leq \orderVariable{l}{j}{k}, \forall i, j, 
% k, l : \parent{l} = \codeRegion{i}
% \end{equation*}

% Finally, the third set ensures that, when merging adjacent code regions \glspl{pi} must be deployed in the same order, which is:
% \begin{align*}
% \left( \left(\proxVariable{i}{j}{k} = 1\right) \wedge 
% \left(\orderVariable{i}{k}{l} = 1\right) \right)&\rightarrow \\\left( 
% \left(\proxVariable{i}{j}{l} = 1\right) \wedge 
% \left(\orderVariable{j}{k}{l} = 1\right) \right)&,\forall i, j, k, l
% \end{align*}
% For the sake of readability, the last constraints contains the traditional logical operators $\wedge$ and $\rightarrow$. Such expressions can be easily linearized via standard techniques.

\subsection{Translation algorithm}
\label{sec:l2p:algo}

\begin{itemize}
    \item brief description of translation algorithm (from MILP solution to AH solution in KB) from STM paper
\end{itemize}

% The \emph{translation algorithm} generates the final asset hiding solution, which is, the ordered 
% list of protections to apply on every code region.
% It takes as input the values assumed by the $\mainVariable{i}{j}$, $\orderVariable{i}{j}{k}$ and $\proxVariable{i}{j}{k}$ variables, whose values have been obtained by solving the \milp problem presented in Section~\ref{sec:model}. These variables express the protections that must be deployed on every code region, the order of deployment, and if the protections need to be deployed on adjacent code region as a whole or as individual applications of the same protection. 
% For instance, variables corresponding to protections that are enabled on ancestors need to be enabled for all the descendants as well. However, in practice, they must be deployed only once on the ancestor.

% Moreover, code regions that are non-overlapping (sibling of the same ancestors, which may be adjacent or not) need to be merged according to the $\proxVariable{i}{j}{k}$ variables.

% In order to globally determine the protections that must be deployed, the 
% translation algorithm has been developed to perform:
% \begin{itemize}
% 	\item \emph{generate lists}, every code region is associated with a set of protections $\mainVariable{i}{j}$ that needs to be deployed on it. However, 
% 	protections must be deployed according to the order given by the 
% 	$\orderVariable{i}{j}{k}$ variables. The algorithm transforms the information in these variables into a list of deployed \glspl{pi} associated to each node.
% 	\item \emph{remove duplicate}, if a protection is deployed to an ancestor, the protection is removed from the list of \glspl{pi} deployed to each of its descendants. %of a code region and globally cover the whole parent code region, the protections are associated with the parent node and removed from the children;
% 	\item \emph{horizontal enlargement}, if a protection needs to be deployed to two or more adjacent code regions (because of the $\mainVariable{i}{j}$) and can be merged (due to $\proxVariable{i}{j}{k}$ values), a new code region is generated that spans all the adjacent code regions to merge. This node becomes an intermediate ancestor, \ie a child of the original parent and the parent of all the merged node.
% \end{itemize}

% After these operations are completed, the translation algorithm outputs the asset hiding solution, \ie a coherent set of lists of protections to apply on every code region, \ie a poset of \glspl{pi}.

\subsection{Validation}
\label{sec:l2p:validation}

\begin{itemize}
    \item cite requirements, why they are solved and why we are so cool
\end{itemize}


% In this section, the asset hiding phase described in this chapter is compared with \esp requisites listed in Section~\ref{sec:esp:problem}.

% Requisites for the \esp usage scenario, defined in Section~\ref{sec:esp:problem:framing}, are mostly respected by the asset hiding phase. First, the time needed to execute this phase can be influenced with a set of configuration parameters: a hard time limit, and a maximum number of non-asset code regions taken into account when generating the \milp model. A longer execution of the algorithm may be adopted prior to the target application release, in order to find a better hiding solution, while shorter times are suitable when patches are released and time is an issue. Thus, the asset hiding phase can adapt to the target application life-cycle. Also, asset hiding solutions are human-readable, being presented with the same format of asset protection ones; furthermore, for each \DPI added in the solution, \esp presents the user with the strategy (or strategies) for which the \DPI has been chosen. 

% A limitation of the current approach is that the attacker skills are not taken into account when the additional protections are decided. This is due to the lack of experimental assessments of the asset identification capabilities of the attackers, which the authors intend to execute in the future. After this assessments, the data needed to take into account the attacker profile in the asset hiding decision process would be obtained, and furthermore, a method to obtain an actual estimation of the time needed to find the assets could be devised.

% Regarding the requirements for the risk mitigation phase (Section~\ref{sec:esp:problem:mitigation}), \esp respects them. First, since the identification of the assets is a necessary preliminary step for attacks, the asset hiding phase defers the attacks, hiding the fingerprints of the asset protection phase that ease the detection assets by attackers. Furthermore, the asset hiding protections are chosen to maximize the confusion induced by them in the attacker, which is evaluated through formulas that are dependent on the metrics of the code regions on which the formulas are deployed. Overheads are taken into account in this phase, inferring solutions that, when deployed, lead to protected binaries that are still usable. Finally, as the asset protection phase, all the protection techniques used in this phase are implemented by automatic protection tools, so also this phase is completely automated.

% Finally, in the \asp project validation phase \cite{D1.06.9} the asset hiding phase was deemed as a useful addition to the \esp workflow. The experts validated the additional protections inferred in this phase, stating that the proposed solutions for the \esp use cases were free from inconsistencies, and would be useful to defer an attacker in the process of finding the protected assets in the target application binary. Furthermore, they considered it an advancement in respect with the current way of handling fingerprints by software security practitioners, which is essentially based on various obfuscation attempts on the application binary, a time-consuming process that is needed to find a good trade-off between asset concealment and introduced overhead.

==> preamble.tex <==
% *** CITATION PACKAGES ***
%
%\ifCLASSOPTIONcompsoc
  % IEEE Computer Society needs nocompress option
  % requires cite.sty v4.0 or later (November 2003)
%  \usepackage[nocompress]{cite}
%\else
  % normal IEEE
%  \usepackage{cite}
%\fi
\RequirePackage[T1]{fontenc}
\RequirePackage{graphicx}
\RequirePackage{mathptmx}      % use Times fonts if available on your TeX system
\RequirePackage{flushend}
\RequirePackage[numbers,sort&compress]{natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}

\usepackage{moreverb}



\usepackage[pdftex,svgnames,dvipsnames]{xcolor}

\usepackage{tabularx}

\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{algorithm}

\usepackage{url}
\usepackage{xspace}

\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathrsfs}

\usepackage{booktabs}
\usepackage{float}
\usepackage[]{microtype}

\usepackage{proof}
\usepackage{paralist}

\usepackage[binary-units]{siunitx}

\usepackage{ifthen}

\usepackage{times}
\usepackage{tablefootnote}

% \usepackage[inline,shortlabels]{enumitem}

\usepackage{fontawesome}
\usepackage{subcaption}
\usepackage{multirow}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[pscoord]{eso-pic} % The zero point of the coordinate system is the lower left corner of the page (the default).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings}

\lstset{
    tabsize=2,
    basicstyle=\ttfamily\small,
    stringstyle=\ttfamily,
    title=\lstname,
    numbers=none,
    numberstyle=\scriptsize,
    numbersep=3pt, stepnumber=2,
    firstnumber=1,
    numberfirstline=true,
    escapeinside={(*@}{@*)},
    morekeywords={ips,ipd,pd,ps,proto,conn,url,http_access,http_reply_access,acl,allow,deny,resolution_strategy,default_action,policy_data,external_data,rule_data},
    frameround=fttt,
    aboveskip={-1\baselineskip},
}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{mdwtab}

%\usepackage{fixltx2e}
\usepackage{stfloats}

\newcommand{\fw}[1]{$f\!w_{#1}$}
\usepackage[]{units}
\usepackage{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovedisplayskip}{2pt}
\setlength{\belowdisplayskip}{2pt}
\setlength{\abovedisplayshortskip}{2pt}
\setlength{\belowdisplayshortskip}{2pt}
\widowpenalty10000
\clubpenalty10000



\DeclareMathOperator{\confidentiality}{\mathcal{C}}
\DeclareMathOperator{\integrity}{\mathcal{I}}
\DeclareMathOperator{\excorr}{\mathcal{E}}
\DeclareMathOperator{\Prec}{\prec}
\DeclareMathOperator{\PrecEq}{\preceq}
\DeclareMathOperator{\Succ}{\succ}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage[]{todonotes}
% \newcommand{\todoAll}[1]{\todo[color = yellow, inline]{\textbf{To all:} #1}}
% \newcommand{\todoDaniele}[1]{\todo[color = lime, inline]{\textbf{To Daniele:} #1}}
% \newcommand{\todoAldo}[1]{\todo[color = orange, inline]{\textbf{To Aldo:} #1}}
% \newcommand{\todoLeonardo}[1]{\todo[color = lime, inline]{\textbf{To Leonardo:} #1}}

%\newcommand{\complete}[1]{\textcolor{red}{COMPLETE WITH #1}}
%\newcommand{\new}[1]{{\color{blue}#1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{pdfcomment}
%\usepackage{soul}
%\newboolean{sottolinea}
%\setboolean{sottolinea}{false}
%\newboolean{risolto}
%\setboolean{risolto}{true}
%\newcommand{\sottolinea}[2]{\ifthenelse{\boolean{sottolinea}}{\pdfmarkupcomment[markup,color=yellow!30!]{#2}{#1}}{#2}}
%\newcommand{\risolto}[3]{\ifthenelse{\boolean{risolto}}{\pdfmarkupcomment[markup,color=green!30!]{#3}{(#1)\\ #2}}{#3}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\cmd}[1]{\texttt{#1}\xspace}
%l2p
\newcommand{\codeRegion}[1]{c_{#1}}
\newcommand{\codeRegionSpace}{C}
\newcommand{\reducedCodeRegionSpace}{\codeRegionSpace^*}
\newcommand{\source}[1]{\operatorname{source}(\codeRegion{#1})}
\newcommand{\sLine}[1]{\operatorname{sl}(\codeRegion{#1})}
\newcommand{\eLine}[1]{\operatorname{el}(\codeRegion{#1})}
\newcommand{\protection}[1]{P_{#1}}
\newcommand{\protectionInstantiation}[1]{p_{#1}}
\newcommand{\protectionInstantiationSpace}{\mathbb{P}}
\newcommand{\protectionInstantiationSpaceLOneP}{\protectionInstantiationSpace|_{\text{AP}}}
\newcommand{\prot}[1]{\operatorname{protection}(\protectionInstantiation{#1})}
\newcommand{\appliedProtectionInstantiation}[2]{\protectionInstantiation{#1}/\codeRegion{#2}}
\newcommand{\biSet}{\{ 0, 1 \}}
\newcommand{\overh}[1]{\operatorname{\mathscr{O}}_{#1}}
\newcommand{\overhead}[3]{\overh{#1}(\appliedProtectionInstantiation{#2}{#3})}
\newcommand{\overheadd}[4]{\overh{#1}(\appliedProtectionInstantiation{#2}{#3}, \metric{1}{#3}, \metric{2}{#3}, \dots)}
\newcommand{\localOverhead}[3]{\operatorname{\omega}_{#1}(\appliedProtectionInstantiation{#2}{#3})}
\newcommand{\metric}[2]{\operatorname{\mathcal{M}}_{#1}(\codeRegion{#2})}
\newcommand{\protectionInstantiationSpaceMax}{\Gamma}
\newcommand{\overheadMax}[1]{\Omega_{#1}}
\newcommand{\techniques}{\mathbb{T}}
\newcommand{\replication}{\mathcal{R}}
\newcommand{\enlargement}{\mathcal{E}}
\newcommand{\shadowing}{\mathcal{S}}
\newcommand{\confusion}[3]{\operatorname{cnf}_{#1}(\appliedProtectionInstantiation{#2}{#3})}
\newcommand{\confusionLong}[3]{\operatorname{cnf}_{#1,\protectionInstantiation{#2}}(#3)}
\newcommand{\confusionShadowing}[3]{\operatorname{cnf}_{\shadowing}(\appliedProtectionInstantiation{#1}{#3},\appliedProtectionInstantiation{#2}{#3})}
\newcommand{\confusionShadowingLong}[3]{\operatorname{cnf}_{\shadowing,\protectionInstantiation{#1},\protectionInstantiation{#2}}(#3)}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\lOneP}[2]{\operatorname{AP}(\appliedProtectionInstantiation{#1}{#2})}
\newcommand{\rLOneP}[2]{\operatorname{AP^*}(\appliedProtectionInstantiation{#1}{#2})}
\newcommand{\prox}[2]{\operatorname{adj}(\codeRegion{#1}, \codeRegion{#2})}
\newcommand{\mainVariable}[2]{x_{\appliedProtectionInstantiation{#1}{#2}}}
\newcommand{\orderVariable}[3]{y_{\codeRegion{#1}, \protectionInstantiation{#2}, \protectionInstantiation{#3}}}
\newcommand{\proxVariable}[3]{g_{\codeRegion{#1}, \codeRegion{#2}, \protectionInstantiation{#3}}}
\newcommand{\proxSet}[3]{G_{\codeRegion{#1}, \codeRegion{#2}, \protectionInstantiation{#3}}}
\newcommand{\enlargementVariable}[3]{e_{\codeRegion{#1}, \codeRegion{#2}, \protectionInstantiation{#3}}}
\newcommand{\enlargementSet}[2]{E_{\appliedProtectionInstantiation{#1}{#2}}}
\newcommand{\techniqueVariable}[2]{z_{\appliedProtectionInstantiation{#1}{#2}}}
\newcommand{\parent}[1]{\operatorname{parent}(\codeRegion{#1})}
\newcommand{\children}[1]{\operatorname{children}(\codeRegion{#1})}
\newcommand{\ancestors}[1]{\operatorname{ancestors}(\codeRegion{#1})}
\newcommand{\descendants}[1]{\operatorname{descendants}(\codeRegion{#1})}
%\newcommand{\weight}[1]{\operatorname{weight}(\codeRegion{#1})}
\newcommand{\bonus}[3]{\rho^{#1}_{\appliedProtectionInstantiation{#2}{#3}}}
\newcommand{\orderSet}[2]{\Psi_{\appliedProtectionInstantiation{#1}{#2}}}
\newcommand{\LUP}{asset protection\xspace}
\newcommand{\LDP}{asset hiding\xspace}
\newcommand{\High}{\textsc{high}\xspace}
\newcommand{\Low}{\textsc{low}\xspace}
\newcommand{\None}{\textsc{--}}
\newcommand{\Masking}[2]{#1 (#2)}

%latex stuff
\newcommand{\Center}[1]{\multicolumn{1}{c}{#1}}
\newcommand{\header}[2]{\multicolumn{#1}{c}{\textsc{#2}}}

\usepackage[acronym,nomain]{glossaries}
%\makeglossaries
\glsdisablehyper
%metamodel compatibility
\newcommand{\class}[1]{{\footnotesize\sffamily#1}}
\newcommand{\association}[1]{{\footnotesize\sffamily#1}}
\let\attribute\attr
\newcommand{\attribute}[1]{{\footnotesize\sffamily#1}}
%\newcommand{\changed}[1]{#1}
\newcommand{\changed}[1]{{\color{black}#1}}
\definecolor{mypinka}{rgb}{0.858, 0.188, 0.478}
\definecolor{mypinkb}{rgb}{0.708, 0.438, 0.528}
\newcommand{\changeda}[1]{{\color{mypinka}#1}}
\newcommand{\changedb}[1]{{\color{mypinkb}#1}}

% Abbreviations.
\newcommand{\ie}{i.e.\@\xspace} % Id est.
\newcommand{\eg}{e.g.\@\xspace} % Exempli gratia.
\newcommand{\wrt}{w.r.t.\@\xspace} % With respect to.
\newcommand{\etal}{\textit{~et~al.\@}\xspace}

\newcommand{\ekb}{Knowledge Base\xspace}
\newcommand{\esca}{Source Code Analyzer\xspace}
\newcommand{\emf}{Metrics Framework\xspace}
\newcommand{\eptc}{Protection Tools Connector\xspace}
%\newacronym{ear}{EAR}{\gls{ear} Attack Reasoner}\newcommand{\ear}{\gls{ear}\xspace}
\newcommand{\ebad}{Risk Assessment Engine\xspace}
\newcommand{\eape}{Protection Enumerator\xspace}
\newcommand{\eapd}{Risk Mitigation Engine\xspace}
\newcommand{\ehal}{Asset Hiding Engine\xspace}
\newcommand{\esd}{Solution Deployer\xspace}
\newcommand{\eui}{User Interface\xspace}

%ESP data (pis, ecc.)
\newacronym{as}{AS}{Attack Step}\newcommand{\AS}{\gls{as}\xspace}
\newcommand{\ASs}{\glspl{as}\xspace}
\newacronym{ap}{AP}{Attack Path}
\newcommand{\AP}{\gls{ap}\xspace}
\newcommand{\APs}{\glspl{ap}\xspace}
\newacronym{dpi}{DPI}{Deployed Protection Instance}\newcommand{\DPI}{\gls{dpi}\xspace}
\newcommand{\DPIs}{\glspl{dpi}\xspace}
\newcommand{\DPIset}{\DPI set\xspace}
\newcommand{\DPIsets}{\DPI sets\xspace}
\newacronym{pi}{PI}{Protection Instance}
\newcommand{\PI}{\gls{pi}\xspace}
\newcommand{\PIs}{\glspl{pi}\xspace}
\newcommand{\PIset}{\PI set\xspace}
\newcommand{\PIsets}{\PI sets\xspace}
\newacronym{po}{PO}{{Protection Objective}}\newcommand{\PO}{\gls{po}\xspace}
\newcommand{\POs}{\glspl{po}\xspace}
\newcommand{\POset}{\gls{po} set\xspace}
\newcommand{\POsets}{\glspl{po} sets\xspace}
%\newacronym{cr}{CR}{Code Region}\newcommand{\CR}{\gls{cr}\xspace}
%	\newcommand{\CRs}{\glspl{cr}\xspace}
\newcommand{\CR}{code region\xspace}
\newcommand{\CRs}{code regions\xspace}
\newcommand{\CRset}{\CR set\xspace}
\newcommand{\CRsets}{\CR sets\xspace}
%institutions
\newacronym{nist}{NIST}{National Institute of Standards and Technology}\newcommand{\nist}{\gls{nist}\xspace}
\newacronym{gdpr}{GDPR}{General Data Protection Regulation}\newcommand{\gdpr}{\gls{gdpr}\xspace}

%aspire miscellanea
\newacronym{asp}{ASPIRE}{Advanced Software Protection: Integration, Research and Exploitation}\newcommand{\asp}{\gls{asp}\xspace}
\newacronym{accl}{ACCL}{Client-side Communication Logic}\newcommand{\accl}{\gls{accl}\xspace}
\newacronym{ascl}{ASCL}{Server-side Communication Logic}\newcommand{\ascl}{\gls{ascl}\xspace}
\newacronym{actc}{ACTC}{ASPIRE Compiler Tool Chain}\newcommand{\actc}{\gls{actc}\xspace}
\newacronym{esp}{ESP}{Expert system for Software Protection}\newcommand{\esp}{\gls{esp}\xspace}
\newacronym{it}{IT}{Information Technology}\newcommand{\itech}{\gls{it}\xspace}


%software protection acronyms
\newacronym{diablo}{DIABLO}{Diablo Is A Better Link-time Optimizer}\newcommand{\diablo}{\gls{diablo}\xspace}
\newacronym{cff}{CFF}{Control Flow Flattening}\newcommand{\cff}{\gls{cff}\xspace}
\newacronym{api}{API}{Application Programming Interface}\newcommand{\api}{\gls{api}\xspace}
\newacronym{ip}{IP}{Intellectual Property}\newcommand{\ip}{\gls{ip}\xspace}
\newacronym{drm}{DRM}{Digital Rights Management}\newcommand{\drm}{\gls{drm}\xspace}
\newacronym{cve}{CVE}{Common Vulnerabilities and Exposures}\newcommand{\cve}{\gls{cve}\xspace}
\newacronym{cwe}{CWE}{Common Weakness Enumeration}\newcommand{\cwe}{\gls{cwe}\xspace}
\newacronym{mate}{MATE}{Man-At-The-End}\newcommand{\mate}{\gls{mate}\xspace}
\newacronym{sp}{SP}{Software Protection}\newcommand{\softprot}{\gls{sp}\xspace}
\newacronym{aslr}{ASLR}{Address Space Layout Randomization}\newcommand{\aslr}{\gls{aslr}\xspace}
%attestation acronyms
\newacronym{txt}{TXT}{Trusted eXecution Technology}\newcommand{\txt}{\gls{txt}\xspace}
\newacronym{tpm}{TPM}{Trusted Platform Module}\newcommand{\tpm}{\gls{tpm}\xspace}
\newacronym{tcg}{TCG}{Trusted Computing Group}\newcommand{\tcg}{\gls{tcg}\xspace}
\newacronym{sgx}{SGX}{Software Guard Extensions}\newcommand{\sgx}{\gls{sgx}\xspace}

%for old times sake
\newacronym{dec}{DEC}{Digital Equipment Corporation}\newcommand{\dec}{\gls{dec}\xspace}
\newacronym{vax}{VAX}{Virtual Address eXtension}\newcommand{\vax}{\gls{vax}\xspace}

%expert systems
\newacronym{dendral}{DENDRAL}{DENDritic ALgorithm}\newcommand{\dendral}{\gls{dendral}\xspace}
\newacronym{xcon}{XCON}{eXpert CONfigurer}\newcommand{\xcon}{\gls{xcon}\xspace}
\newacronym{ides}{IDES}{Intrusion Detection Expert System}\newcommand{\ides}{\gls{ides}\xspace}
\newacronym{nides}{NIDES}{Next-generation Intrusion Detection Expert System}\newcommand{\nides}{\gls{nides}\xspace}
\newacronym{nidx}{NIDX}{Network Intrusion Detection eXpert system}\newcommand{\nidx}{\gls{nidx}\xspace}
\newacronym{nadir}{NADIR}{Network Anomaly Detection and Intrusion Reporter}\newcommand{\nadir}{\gls{nadir}\xspace}
\newacronym{audes}{AudES}{Expert System for security Auditing}\newcommand{\audes}{\gls{audes}\xspace}

%software acronyms
\newacronym{cfg}{CFG}{Control Flow Graph}\newcommand{\cfg}{\gls{cfg}\xspace}
\newacronym{os}{OS}{Operating System}\newcommand{\os}{\gls{os}\xspace}
\newacronym{dll}{DLL}{Dynamic-Link Library}\newcommand{\dll}{\gls{dll}\xspace}
\newacronym{gnu}{GNU}{GNU is Not Unix}\newcommand{\gnu}{\gls{gnu}\xspace}
\newacronym{gcc}{GCC}{\gls{gnu} C Compiler}\newcommand{\gcc}{\gls{gcc}\xspace}
\newacronym{gdb}{GDB}{\gls{gnu} DeBugger}\newcommand{\gdb}{\gls{gdb}\xspace}
\newacronym{foss}{FOSS}{Free and Open Source Software}\newcommand{\foss}{\gls{foss}\xspace}
\newacronym{cdt}{CDT}{C/C++ Development Tooling}\newcommand{\cdt}{\gls{cdt}\xspace}
\newacronym{ast}{AST}{Abstract Syntax Tree}\newcommand{\astree}{\gls{ast}\xspace}
\newacronym{gui}{GUI}{Graphical User Interface}\newcommand{\gui}{\gls{gui}\xspace}
\newacronym{xml}{XML}{eXtensible Mark-up Language}\newcommand{\xml}{\gls{xml}\xspace}

%metrics acronyms
\newacronym{sloc}{SLOC}{Source Lines Of Code}\newcommand{\sloc}{\gls{sloc}\xspace}
\newacronym{hl}{HL}{Halstead's Length}\newcommand{\HL}{\gls{hl}\xspace}
\newacronym{cc}{CC}{Cyclomatic Complexity}\newcommand{\CC}{\gls{cc}\xspace}

%hardware acronyms
\newacronym{cpu}{CPU}{Central Processing Unit}\newcommand{\cpu}{\gls{cpu}\xspace}
\newacronym{fpu}{FPU}{Floating Point Unit}\newcommand{\fpu}{\gls{fpu}\xspace}
\newacronym{alu}{ALU}{Arithmetic and Logic Unit}\newcommand{\alu}{\gls{alu}\xspace}
\newacronym{gpu}{GPU}{Graphics Processing Unit}\newcommand{\gpu}{\gls{gpu}\xspace}
\newacronym{gpgpu}{GPGPU}{General-Purpose computing on Graphics Processing Units}\newcommand{\gpgpu}{\gls{gpgpu}\xspace}


%programming languages acronyms
\newacronym{lisp}{LISP}{LISt Processor}\newcommand{\lisp}{\gls{lisp}\xspace}
\newacronym{cil}{CIL}{C Intermediate Language}\newcommand{\cil}{\gls{cil}\xspace}

%network acromyms
\newacronym{smb}{SMB}{Server Message Block}\newcommand{\smb}{\gls{smb}\xspace}

%network protection acronyms
\newacronym{mitm}{MITM}{Man-In-The-Middle}\newcommand{\mitm}{\gls{mitm}\xspace}
\newacronym{ddos}{DDoS}{Distributed Denial of Service}\newcommand{\ddos}{\gls{ddos}\xspace}

%malware acronyms
\newacronym{rat}{RAT}{Remote Access Trojan}\newcommand{\rat}{\gls{rat}\xspace}

%network protection
\newacronym{ids}{IDS}{Intrusion Detection System}\newcommand{\ids}{\gls{ids}\xspace}
\newacronym{cysemol}{CySeMoL}{Cyber Security Modeling Language}\newcommand{\cysemol}{\gls{cysemol}\xspace}
\newacronym{camel}{CAMEL}{Cloud Application Modelling \& Execution Language}\newcommand{\camel}{\gls{camel}\xspace}
%machine learning
\newacronym{ml}{ML}{Machine Learning}\newcommand{\ml}{\gls{ml}\xspace}
\newacronym{ai}{AI}{Artificial Intelligence}\newcommand{\ai}{\gls{ai}\xspace}
\newacronym{som}{SOM}{Self-Organizing Maps}\newcommand{\som}{\gls{som}\xspace}
\newacronym{ann}{ANN}{Artificial Neural Network}\newcommand{\ann}{\gls{ann}\xspace}

%optimization
\newacronym{milp}{MILP}{Mixed Integer-Linear Programming}\newcommand{\milp}{\gls{milp}\xspace}

%ontologies
\newacronym{owl}{OWL}{Web Ontology Language}\newcommand{\owl}{\gls{owl}\xspace}
\newacronym{owltwo}{OWL2}{\acrlong{owl} 2}\newcommand{\owltwo}{\gls{owltwo}\xspace}

%other stuff
\newacronym{roi}{ROI}{Return In Investment}\newcommand{\roi}{\gls{roi}\xspace}
\newacronym{byod}{BYOD}{Bring Your Own Device}\newcommand{\byod}{\gls{byod}\xspace}
\newacronym{bsa}{BSA}{BSA | The Software Alliance}\newcommand{\bsa}{\gls{bsa}\xspace}
\newacronym{otp}{OTP}{One-Time Password}\newcommand{\otp}{\gls{otp}\xspace}
\newacronym{pin}{PIN}{Personal Identification Number}\newcommand{\pin}{\gls{pin}\xspace}
\newacronym{sdlc}{SDLC}{Software Development Life Cycle}\newcommand{\sdlc}{\gls{sdlc}\xspace}
\newacronym{kb}{KB}{Knowledge Base}\newcommand{\kb}{\gls{kb}\xspace}
\newacronym{poc}{PoC}{Proof of Concept}\newcommand{\poc}{\gls{poc}\xspace}

\usepackage{tikz}
\usetikzlibrary{
	decorations,
	arrows,
	shapes,positioning,
	patterns,
	fit,
	automata,
	decorations.markings,
	plotmarks,
	decorations.pathmorphing,
	positioning,
	backgrounds,
	fit,
	calc,
	arrows.meta}

\usepackage{pgfplots}
\pgfplotsset{ cycle list={%
		{smooth,black,mark=triangle*},
		{smooth,black,mark=triangle},
		{smooth,black,mark=*},
		{smooth,black,mark=o},
		{smooth,black,mark=square*},
		{smooth,black,mark=square},
		{smooth,black,mark=diamond*},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
		{smooth,black},
	},
	compat=1.3,
	tick label style={ font=\scriptsize,/pgf/number format/set thousands separator={}}}
\usepgfplotslibrary{fillbetween}

\usepackage[draft]{fixme}
\fxsetup{layout=inline,theme=color}
\FXRegisterAuthor{bds}{brds}{\color{purple}bds}
\FXRegisterAuthor{ab}{aab}{\color{brown}ab}
\FXRegisterAuthor{bc}{ebc}{\color{red}bc}
\FXRegisterAuthor{lr}{alr}{\color{orange}lr}
\FXRegisterAuthor{dc}{adc}{\color{green!50!black}dc}

\FXRegisterAuthor{rone}{roner}{\color{pink}reviewer1}
\FXRegisterAuthor{rtwo}{rtwor}{\color{pink}reviewer2}
\FXRegisterAuthor{rthree}{rthreer}{\color{pink}reviewer3}

%%%%%%%%%%%%%%%%%%%%5
% for arxiv only
%\usepackage[pscoord]{eso-pic}
\newcommand{\placetextbox}[3]{% \placetextbox{<horizontal pos>}{<vertical pos>}{<stuff>}
 \setbox0=\hbox{#3}% Put <stuff> in a box
 \AddToShipoutPictureFG*{% Add <stuff> to current page foreground
    \put(\LenToUnit{#1\paperwidth},\LenToUnit{#2\paperheight}){\vtop{{\null}\makebox[0pt][c]{#3}}}%
 }%
}%


==> requisites.tex <==
\if 0

\abnote{write explicitly the research questions in each subsection (give them names!)}
\abnote{split this section in two: use cases and then after research questions}

% The main objective of this thesis is to present a decision support system for automatic software protection, called \acrfull{esp}. As detailed in the introduction, protecting software has been a task reserved to few experts in the field, which manually analyze the application to protect, identify the possible vulnerabilities, and then decide the best mitigations, \ie software protection techniques, to solve them. In doing so, experts base their decisions mainly on their knowledge in the field, their past experience, and ultimately on their instinct. Thus, a decision support system that wants to automatically protect applications needs to mimic how security experts do their job, following the classical approach of expert systems detailed in Section~\ref{sec:background:expSys}, already applied to other aspects of cybersecurity, \eg network vulnerability analysis and mitigation \cite{nidesReq, nidx, nadir, audes}. To the best of the author's knowledge, no prior works in literature apply the expert system methodology in the software protection field.

The software protection process may be more formally defined framing it as a risk management process, a customary activity in various industry sectors, such as finance, pharmaceutics, infrastructure, energy and, of course, information technology. Regarding the latter, the \nist standard for information security \cite{nistSP800-39} outlines a high-level workflow for IT systems risk management, comprising the following phases:
\begin{enumerate}
	\item \emph{risk framing}: establish the scenario in which the risk must be managed;
	\item \emph{risk assessment}: identify threats against the system assets, vulnerabilities of the system, the harm that may occur if such vulnerabilities are exploited, and the likelihood this would happen;
	\item \emph{risk mitigation}: determine and implement appropriate actions to mitigate the risks;
	\item \emph{risk monitoring}: verify that the implemented actions are effective in mitigating the risks.
\end{enumerate}




\subsection{Risk framing}
\label{sec:esp:problem:framing}

% To frame risk, it must be taken into account that this thesis targets \mate scenarios, with software running on untrusted machines, therefore an attacker has complete access to the software binary code, and can monitor its execution. A broad range of tools (\eg debuggers, decompilers, disassemblers, fuzzers) can be used by an attacker to endanger the software assets, whatever its drive may be (\eg financial gain, industrial espionage, or simply personal satisfaction). However, a less experienced attacker may not be able to use effectively these tools, therefore more complex attacks may be executed only by few attackers. Conversely, more experienced attackers may not be interested in attacking the application that must be protected. For example, a seasoned attacker is unlikely to spend time in hacking a low value application, thus protections against more complex attacks may be unnecessary, or even unfeasible from a financial point of view. Spending thousands of dollars to safeguard an application licensing scheme, acquiring licenses of strong proprietary protection schemes, is financially sustainable only if the value of the application and the expected turnover from the application sales justify it. Thus, different attacker profiles, with increasing levels of skill and experience, must be modelled, so that \esp can take this information into account, in order to correctly assess risk depending on the application value.

% Also, as presented in the Introduction, \esp must be designed for two different usage scenarios. First, \esp can be useful to application developers, without specific knowledge in software security, which do not have the financial resources or the will to hire security experts to protect their application. In this case, \esp must implement a completely automated workflow, driving a set of automated protection tools (as the ones presented in Section~\ref{sec:background:softProt:tools}), able to provide the software developer with a protected application binary, limiting as most as possible the interaction required with him or her in the process. Second, \esp can constitute an interesting tool for security experts, which want to obtain a first solution to the problem, which they can analyze to assess its effectiveness, and further manually refine if necessary. Thus, insights on the results of all the workflow phases must be provided.

% Finally, as pointed out by security experts interviewed in the \esp design phase, the target application life-cycle must be taken into account. Prior to software release, enough time is available to carry out a thorough assessment of the application risks and to infer and apply the possible mitigations. However, after distribution of the application, possible bugs may surface. After users encounter such problems and report them, a patch that solves these issues must be released as soon as possible. Thus, the amount of time to find possible threats or vulnerabilities introduced in the new version of the application by the aforementioned patches is limited, and a more shallow assessment of risk must be performed. Therefore, \esp must provide different usage profiles. Accuracy of results produced by its reasoning processes will depend on the time available to perform them. Thus, the user can choose the more appropriate profile, given the software life-cycle phase in which \esp is employed.

%\todoAll{peculiarity of software protection for risk framing}

\abnote{risk framing: objective: Define the context where risk analysis will be performed, it's about procedures and also about the definition of the basic elements of the risk analysis, models models models blahblah}

\abnote{the objective of this itemize is to prove that there's nothing usable, so it is worth defining a standard or just sketching a standard software risk framing procedure, the ADSS is pioneering the field}

\begin{enumerate}

\item what is an assets? (data, code itself, intellectual properties, what you can do with the software, ...)
\bdsnote{attack model from ASPIRE is initial answer}

\item what are the security requirements? Are the ones in SP800-39 enough?
\bdsnote{requirements from ASPIRE attack model}
\abnote{attack model from ASPIRE, standards are needed but are not our job, involvement of industry, similar to what happened in past cases }
\dcnote{The ADSS models only two basic requirements: confidentiality and integrity.}


\item How software assets and their security requirements may be formally described in order to enable a more automated risk assessment procedure (as by risk framing RQ)? (sub-RQ: How software assets may be identified by stakeholders?)
\bdsnote{annotating source code is definitely formal}

\item is there any way to (automatically) locate assets? \bdsnote{not completely, the application assets are too specific to the business model of the company. As for hooks (fragments that become assets because attackers know they can help in locating the real assets), that is another matter. To some extent a pre-defined catalogue can be maintained, and taint analysis can probably be used. The same holds for the parts of protections that become assets under attacks.}
Is it possible to have a catalogue and to maintain it up to date with new releases of the software? \bdsnote{tough question} \dcnote{If we really want to talk about this we should explain why we don't do it in the ADSS or, a better idea, put it as a future work.}

\item are there standard attacker models? \bdsnote{more than one is needed, depending on business models different levels of expertise can be expected} MATE is detailed enough to allow precise risk analysis? \bdsnote{no, e.g., whenever we use worst-case assumptions, the precision goes down. But maybe that is okay?} \dcnote{The ADSS models the attacker by letting you choose his/her expertise level (geek, amateur, professional, guru). Changing the expertise level alters the coefficients used in the internal formulas (e.g. increase/decrease the attack probabilities).}


\item How the relationships between software assets and non-assets (apparently non-sensitive portion of code) may be formally modelled? Is there any way to mark them as sensitive also if they are not assets? In the perspective of attack and protection processes... \bdsnote{see my note in bullet 4}

\item what are mitigations in this context? Are software protections the only viable way to mitigate? (e.g., protect the server of RA) \bdsnote{I don't understand the question, as it is not clear how broadly or narrowly the author of this questions interprets the term "software protections"}

\item How software protections, their applicability to the target application, their effectiveness against attacks (\eg Collberg's potency), and their potential side-effects may be formally modeled in order to drive the risk mitigation procedure? \bdsnote{We have a meta-model that can handle this, don't we? at least as an initial attempt, and yielding enough precision for the time being. See also the presentation of Yuan Gu in Dagstuhl: protecting is not only injecting protections, but also designing and architecting the software upfront to be protectable. No idea how that fits in our design, and whether the ADSS would hence give different results on a well-designed app and an app with a problematic architecture.}
\abnote{the ADSS does not see the difference now, the fact that an application has not been designed to be protectable should be evident during the risk analysis, when evaluating how difficult are the attacks. Therefore, it is an open issue to be mentioned but that we didn't address in our prototype.} \dcnote{The only side-effects that we take into account are the overheads. BTW, we also compute/estimate the new complexity metrics whenever we simulate a protection deployment, so if a side-effect can be computed from these values it can be easily added to the ADSS.}

\item Are the result of risk management procedures useful for software security experts? \bdsnote{yes, even if it is only to confirm or help them rather than replacing their decision processes} 

\item Are risk analysis management procedures compatible with the software lifecycle? \bdsnote{currently not I guess, and extending everything we can do now for one version of a program to also consider the case of evolving protections in future versions (Richard Clayton mentioned interesting license check features in Dagstuhl that come close) is a whole other thing. But needed!}
\abnote{to be discussed: all the knowledge base associated to the protection of an application needs to be stateful, especially for diversification purposes. \eg the seeds used to init protections, the parameters for diversity, the used protections for each assets to apply different protections at in close versions; evolution of assets could be considered.}

\item are there standards and standard procedures that define the risk management for software?
\abnote{a new check needs to be done}

\item Is it possible to adapt risk management procedures and standards (\eg the ones developed for network security or for SCADA systems) to the MATE scenario? $\rightarrow$ peculiarity of software protection for risk framing

\item RQ: May such procedures  be implemented in a completely automated fashion so that non expert programmers may use them?

\item RQ: May such procedures be implemented to allow non-SoftwareProtection-experts to use them? Non necessarily automated, also assisted

\end{enumerate}


\abnote{risk assessment: in the context, identify vulnerabilities and attack vectors, estimate impacts and reach some estimation in a ridiculously small dynamic range}

\subsection{Risk assessment}
\label{sec:esp:problem:assessment}

\begin{enumerate}
\item what is a violation of security requirements? Is this an attack? \bdsnote{no, I think it is a successful attack} \abnote{agreed, thus any successful attack is by definition an attack that breaches a security requirement among the ones declared on the identified assets.}

\item what is vulnerability assessment? Is there any automated process to determine the vulnerabilities exposed by the code? Are there procedures to/methodologies to discover and patch these vulnerabilities?
\bdsnote{why do we suddenly care about vulnerabilities (in the meaning of bugs that can be exploited by, e.g., buffer overflows? Or do you mean weaknesses of existing protections? Certainly "patching" those cannot be automated, right?}
\abnote{discussing what is a vulnerability in the new context can be an outcome of the paper. The NIST docs use vulnerabilities, if we want to use the same framework we have to extend it or redefine vulneratility}

\item is penetration testing always needed? Are there techniques to automatically exploit applications? E.g., Automatic Exploit Generation \bdsnote{my gut feeling: automated techniques can be developed that assess how easy attack might be, i.e., that analyse the application or protections to check if they have features (such as invariants) that ease certain types of attacks. For risk management, no exploits are needed, only the possibility of building an exploit. This is similar to remote exploit attack models, where it is assumed that any attacker that can write a chosen value to a chosen address has sufficient power to hijack control of the program completely. No full exploit needs to be engineered to prove the existence of a weakness in that case.}
\abnote{agreed on the philosophical side, penetration testing is an ex-post activity. We need vulnerability assessment/weaknesses assessment. On the other hand, an expert system needs estimates of the risks. Thus the question needs to be rewritten in a different form, how can we find the weakness is penetration testing is not the way to go? We don't have ideas on it now.
The ADSS looks for potential attack strategies, but they are too coarse grained to make precise decisions. Then the question is: what are the data needed to make accurate enough decisions? Open issue!}


\item how exploitation happens? What is the level of expertise? Is there any way to model the experts' abilities? (i.e., the under embargo ASPIRE deliverable?)  How the expertise of a likely attacker (see related risk framing RQ), and its proficiency in using existing attack tool (or in developing ad-hoc ones) impacts the risk of the application? \bdsnote{see my previous note: technical details of exploit need not be known completely for assessment, only existence of weakness and ease with which it may lead to an exploit. Note that weaknesses can either cause the attack identification phase to become easier, or the attack exploitation phase (see ASPIRE economic model), both need to be considered separately I think in an overall risk management process. Plus of course the impact that a successful exploit might have on the company or the profit that an attacker might have from it, again considering both an identified attack and an exploited attack (i.e., scaled up from one instance in the lab to many instances in the field) as separate cases.}
\abnote{on the easy side: I was implying another link the the ASPIRE attack model...}

\item what is the proper level of details of an analysis of the attack paths against the assets? To be usable for mitigations and to make decisions about the best mitigations? \bdsnote{depends on what the aim of the tool support is: identify weaknesses to help experts with decision making, or automate their work to replace them} \dcnote{I agree. If the goal is to aid the developers in fixing the attacks I think that the level of details must be pretty high. If we are only interested in guiding the ADSS I think that we don't need so much information (we are only interested in knowing that an attack can be done, not really all its implementation intricacies).}

\item May existing mathematical methods to quantitatively evaluate risk in computer networks be adapted for software security? It is possible to obtain an estimation of the time needed by an attacker to breach the application asset security requirements? \bdsnote{still an open research question I think}


\item How mental processes of an hypothetical human attacker may be formally described in order to drive the risk assessment procedure? $\rightarrow$ economic value of software exploits (with adaptability of exploits to other target applications) vs. economic value of protected application vs. attacker expertise \bdsnote{I think my previous notes combined provide an answer to these questions: if we model weaknesses and potential exploitability instead of concrete exploits, this can all be done.}
\abnote{at least for risk assessment purposes, more challenging for automatic decision support}

\item How existing risk assessment techniques may be adapted for software security (\ie attack graphs)? \bdsnote{well, with attack graphs indeed, or some more complex versions to enable tool support for, e.g., simulating attackers to draw statistical conclusions, such as Petri Nets}
\abnote{We need to elaborate more on the future research directions here.}

\item are there historical/statistical info that can be used in order to assess the impact of attacks? \bdsnote{no idea}

\end{enumerate}

% \esp needs to include a risk assessment phase, where possible threats against the application are identified, given a set of asset security requirements specified by the application developer. Requesting this information from the latter has been deemed reasonable by experts interviewed in the design phase of \esp, and, to the best of the author's knowledge, there is no prior work in literature automatically identifying assets. To ease developers in this preliminary task, a method must be devised to include requirement definitions in the source code, so that this may be done during the application development and not with an a-posteriori analysis, which can be cumbersome and error-prone, especially with complex applications.

% Regarding risk assessment, a first fundamental activity is defining what is an asset in software security, and which security requirements it may have. A software asset is any code or data comprised in the application that, if successfully attacked, involves a damage for the software proprietors, for example financial losses (\eg lost sales due to an unlicensed version of the application illicitly distributed) or reputation damage (\eg disclosure of sensitive data of the application users). To model assets, specific asset security requirements, \ie asset properties that must be safeguarded against attacks, must be defined, in order to infer possible attacks against them and the appropriate mitigations. Following \cite{nistSP800-39}, two possible security requirements\footnote{The \nist standard identifies an additional requirement, \emph{availability}, defined as ``Ensuring timely and reliable access to and use of information.'', which is applicable for a network scenario, for example hardening the system against \ddos attacks. However, in a \mate scenario, this requirement can be safely ignored, since attacks on the target application remain confined to the attacker machine, not endangering the application availability for legitimate users.} are defined:
% \begin{itemize}
% 	\item \emph{confidentiality}: preventing the disclosure of parts of the application that must remain unintelligible to the attacker, such as proprietary algorithms or cryptographic keys;
% 	\item \emph{integrity}: preserving code that must not be altered by the attacker, for example licensing schemes.
% \end{itemize}

% Then, \esp needs a way to assess risk. Following the classic structure of expert systems, \esp must include a knowledge base, containing all the information needed to correctly infer the threats against assets, and an inference engine, which must model the attacker mental processes in devising actual attacks having as target the breaching of at least one asset security requirement. %Also, we need a way to represent the threats against application assets found with the inference engine. A well-known approach in literature to threat modelling is the use of \emph{attack graphs}, first proposed by Swiler\etal \cite{attackGraphs} for computer networks risk assessment. Each threat is modelled with a tree, having as root node the target of threat (in the \esp case, an asset security requirement), while other nodes correspond to indivisible \emph{attack steps}, simple attacker actions (\eg executing the application, debugging a function); each attack step has a set of preconditions that must hold for the attacker to execute it (\eg to debug a function, a debugger must be attached to the application) and a set of effects if the attacker succeeds in carrying out the task (\eg debugging the function, the attacker understands its business logic, or finds values of local variables at runtime). Starting from the root of the graph, \emph{attack paths} can be inferred, \ie ordered sequences of specific actions that an attacker may execute to substantiate its threat against an asset, breaching a specific security requirement of the latter. Thus, to implement an inference engine able to build attack graphs for each application asset, a set of simple tasks that an attacker may execute in a \mate scenario must be enumerated (\eg analyze execution traces, find a function in the binary code), associated with a set of preconditions and results, in order to obtain meaningful paths. The attack steps level of detail must be also set carefully, so that attack steps are neither too vague or unnecessarily specific: on one hand, using too much generic attack steps can lead to paths lacking expressiveness, with the risk of overlooking possible mitigations, while on the other hand, too detailed attack steps would lead to an impractical high number of equivalent attack paths, which could be solved with the same mitigations, with a detrimental effect on the performances of the inference engine, and increasing the effort needed to manually analyze the inferred attack paths, if the \esp user wants to assess them prior to the mitigation phase. Thus, this \esp phase must be validated: the level of detail of attack steps must be tuned accordingly, by evaluating the accuracy of automatically inferred attack paths on test applications in describing actual attacks executed by security practitioners against such applications.

% %Taking as example a confidential variable, a generic path to breach this security requirement may comprise two steps, executing the application, and searching at run-time the value of the variable in memory; thus, the \esp can infer, as mitigation for this attack path, which the variable value must be obfuscated, \eg with the Tigress technique reported in Section~\ref{sec:background:softProt:antiRevEng:dataObf}; 

% % Also, relationships between generic attack steps and the application structure must be defined, to model realistic attack steps (and consequently paths) that represents the real actions that an attacker must execute to endanger the analyzed applications: for example, if an attacker wants to change the initialization value of a local variable of a function, he may first locate the latter in binary code, and then focus its analysis on the function code to locate the specific variable and subsequently tamper with the initialization code. Finally, \esp must be able to quantify the probability of an attacker succeeding in the attack must be assessed, taking into account the attacker skills, but also the application code characteristics: for example, the effort needed to understand the logic of a function increases with its complexity, in terms of number of instructions comprised in the function code, amount of nodes, edges and possible paths in the \cfg, and number of different memory locations accessed by the instructions. This leads to another requisite for \esp: it must be able to assess the complexity of code constituting application assets. Abundant research has been done in the field of software engineering regarding this issue, with the definition of various software metrics devised to analyze various aspects of code, in order to obtain quantitative measures that summarize its complexity: notable examples are metrics proposed by Halstead \cite{halstead} and McCabe \cite{mccabe}.

% \todoAll{peculiarity of software protection for risk assessment}

\subsection{Risk mitigation}
\label{sec:esp:problem:mitigation}

\begin{enumerate}
\item how to model what protections do and their relations to security requirements? can we simplify by assuming that categories of protections depends on the security requirements? e.g. anti-tampering $\rightarrow$ integrity, obfuscation $\rightarrow$ confidentiality \dcnote{We kinda do that. More precisely we also use an efficacy level (low, medium, high). For instance in our KB we can write obfuscation $\rightarrow$ "high" confidentiality. This approach is described in the meta-model that we published.}

\item what are the assets that can be protected with a given protection and how are they structured? \dcnote{What do you mean be structured?}

\item is there any way to automatically assess what are asset protectable by a new protection? forecast? are they a duty of the protection owners? can we trust protection owners? \bdsnote{as for the latter: we need to trust them because automating this completely seems undoable at first sight. On the other hand, in the ASPIRE security evaluation work, I do propose how the effect of integrity protection and other protections on attack complexity might be measurable (and hence learnable automatically}

\item how to determine synergies, dependencies, incompatibilities, etc. among protections? is it a human decision? is there any way to determine if they could clash? 
(representing them it's easy: a meta-model) \bdsnote{clashing: ML can learn that combining them doesn't work for some reason, dependencies: I think it is possible to build general meta-models in which all kinds of dependencies can fit}

\item how to assess the goodness of a solution? potency? hence, how to find the golden solution? \dcnote{In my mind you can do it (formally) only in two ways. The first is to treat this as an optimization problem (with an unknown objective function) and this is what we do in the ADSS. The alternative is to use a humongous amount of inference/logical rules to mimic what security expert thinks, but my guts tells me that this is probably unfeasible (due to its sheer complexity).}

\item what is the role of empirical assessment? \bdsnote{validating proxies, assumptions, metrics}

\item what is the impact of protections on the application? what are the types of changes it operates on the application to protect? \bdsnote{I don't understand the latter question} \dcnote{From the ADSS point of view each time you apply a protection, the asset metrics change. In turn this means that overheads, the protection index, etc. change since they are based on the metrics.}

\item how to take into account the user experience? \bdsnote{user of the final protected app or of the tool flow?} how can we estimate the overheads? \bdsnote{yes} \dcnote{Currently we estimate the overheads by using the Diablo metrics only. This is a very huge over-simplification and to do it properly I think that a ML-based approach might work (this is a tough one!).}

\item how to model external entities and their security in estimating the effective risk? is the assumption that the servers are trusted valid in the real world? \bdsnote{yes, and we refer to SP800-39 on how to do that}

\item how to model the correlation between protections and attacks (and the attacker expertise)? \bdsnote{If the proxies we use (see above note on attack model assumptions and potential weaknesses that might lead to attacks) are accurate, and if the metrics I mentioned above work, the this can to some extent be automated.}

\item how to take into account the fact that a protection can be defeated or circumvented by an attacker? \bdsnote{dig a hole} \dcnote{We don't model that in the ADSS.}

\item what is the business model used to make decisions? \bdsnote{we are not in the business}

\item how to determine the suitable protections? \bdsnote{obviously with some design space exploration} \dcnote{For me space exploration is more about finding the optimum (golden solution). The solution space in my mind it is the set of all the suitable (valid) solutions. In order to find if a solution is suitable we have to enforce a set of constraints on its protections (like the ADSS does). For instance the ASPIRE code mobility works only on whole functions, it doesn't like smaller code regions.}

\item how to assess the overall impact of the protections seen on the whole application (not just individual assets)? \bdsnote{some weighted combination} \dcnote{This is basically our protection index (which, incidentally, is a weighted combination).}

\item ALDO? identifying protections and guessing assets/content/security properties implied \bdsnote{what is this about? Computer says no}

\item if we want to do everything automatically, how to avoid recompiling entire applications? just estimate everything? \bdsnote{ML and some form of training and validation}

\item how to estimate residual risk and justify what you accepted and why? \bdsnote{good question!}

\item (L2P) can we find a way to mislead the attacker away from the assets? by placing protections on some strategically selected non-assets code regions? \bdsnote{if the goal is delaying an attacker, and it is, then techniques to let them waste time should definitely be considered, see EMSE2019 paper specifically on how attackers develop and execute strategies on the fly. I don't know, however, if such considerations will ever outweigh other ones such as how simple attacks with the (oracle given, worst case assumption) best strategy are.  }

\end{enumerate}


% Given the threats modelled in the risk assessment phase, \ie the attack paths against the security requirement, \esp must be able to infer the possible mitigations against these requirements. Indeed, software protections, as provided in the overview in Section~\ref{sec:background:softProt}, are designed to safeguard the security requirement of assets, countering possible attacks against them. However, it should be noted that in a \mate scenario, an attacker with sufficient motivation and resources will be ultimately able to find a way to remove or circumvent protections, thus succeeding in breaching such security requirement: in other terms, there is no perfect software protection, as it has been formally proved for obfuscation techniques by Barak\etal in \cite{barakImpossibility}. However, protections may be still effective, if they succeed in deferring an attacker (given its profile, as defined in Section~\ref{sec:esp:problem:framing}) for a sufficient amount of time: for example, protections safeguarding a license check embedded in a proprietary application may be deemed effective, if the software remains un-cracked for a time sufficient to provide an economic return (\ie applications sales) that justifies the previous investments in the application developing. So, the objective of \esp, targeting a \mate scenario, is to infer a set of protections that must be used to safeguard the application assets, deferring for the longest time possible the substantiation of threats against them, \ie successful attacks.

% Therefore, \esp must be able to find, for each attack path inferred in the risk assessment phase (see Section~\ref{sec:esp:problem:assessment}), a set of possible mitigation that can be effective in defending the asset endangered by the threat. In other terms, each attack path against one or more security requirement of an asset must be countered by applying the appropriate protections to asset code. %To do so, a mapping between the available protection techniques and the security requirements that such protections are able to safeguard is indeed useful: however, it is not sufficient, since the objective is deferring a possible attacker for as long as possible. This involves defining a method to quantify the effectiveness of protections able to counter the attack paths, in order to compare possible mitigations and infer the ones among them that are most suitable to protect the analyzed application against assessed threats. The concept of \emph{potency} of transformation, introduced by Collberg\etal \cite{collberg1997taxonomy}, is a good starting point to solve this problem, since it binds protection effectiveness with software metrics of the asset code on which the protection is applied, quantifying it with the increase of metrics in the protected application \wrt the original one: in the aforementioned work, Collberg\etal propose a set of metrics that can be used to evaluate the efficiency of code obfuscation (see Section~\ref{sec:background:softProt:antiRevEng:codeObf}), while more general metrics are proposed by Tonella\etal \cite{tonellaPoster}. Thus, building on this prior research, software metrics appropriate to assess the real effectiveness of protection techniques, evaluating their performance when applied on the specific application assets that must be protected; furthermore, such metrics must be evaluated by \esp in an automated fashion, analyzing the source code of the target application.

% It should be also noted that applying protections to the application code has the side-effect of slowing it down. An application is useless if it is well protected but too slow to appeal to the user. The \esp mitigation process will take this problem into account, aiming to find an optimal trade-off between the achieved security for the assets, and the performance overhead introduced by the selected mitigations. %Overhead can clearly be assessed after protecting the application, executing a previously instrumented protected binary, and measuring the additional time, memory and network bandwidth needed to execute the application. However, this execution test should be done automatically: this would require the developer to provide a set of tests for the application, and also would be problematic if the target program has a \gui; furthermore, the application should be tested for each possible set of mitigation inferred by \esp, and this would lead to unfeasible times, especially in the case of big applications, with many assets and a non-negligible time for execution. Thus, a method to approximate the introduced performance overhead on the analyzed application, without actually executing it must be devised: for this purpose, the use of software metrics for overhead estimation will be investigated.

% Also, as detailed in Section~\ref{sec:esp:problem:framing}, \esp must be able to drive a set of automated protection tools, in order to protect the code without requiring user intervention. %To do so, the information needed to operate such tools must be modelled. First, tools are able to enforce various protections (\eg \diablo supports different code obfuscation techniques, as reported in Section~\ref{sec:background:softProt:antiRevEng:codeObf}), so each protection technique must be mapped to the tools enforcing them. Then, for each specific implementation of a technique provided by a tool, all the necessary configuration parameters for the latter must be identified: this is necessary also to infer realistic mitigations, since these parameters may influence the obtained security level and performance overhead after using a tool to protect an asset. For example, \diablo provides a parameter to specify the percentage of basic blocks that must be obfuscated: clearly, setting a high value for this parameter will result in a thorough obfuscation, but will also incur in a considerable slow-down when the obfuscated code is executed. So, different usage profiles for these automated protection tools must be modelled, so that \esp can take them into account in its reasoning processes, and can subsequently drive the automated protection tools with the appropriate values for their parameters.

% Another characteristic of mitigations that must be modelled is that interactions among different protections applied to the same assets must be modelled. As emerged in talks with security experts in the \esp design phase, some protections are able to amplify the effectiveness of other, when applied to the same code: %for example, if a local variable is protected with Tigress data obfuscation technique (see Section~\ref{sec:background:softProt:antiRevEng:dataObf}), the variable value is stored in an encoded form, and decoded on the fly when the variable must be accessed; obfuscating the decoding instructions can certainly increase the effort needed by the attacker to comprehend the encoding schema and compute the real variable value. Conversely, there are cases of incompatibilities among protections: for example, after protecting a function with remote attestation (see Section~\ref{sec:background:softProt:antiTamp:RA}), further modifications cannot be made to the protected code, since this would be erroneously identified by the attestation technique as a tampering attempt by an attacker: so, protecting the same code with remote attestation, and subsequently for example with \cff (a code obfuscation technique described in Section~\ref{sec:background:softProt:antiRevEng:codeObf}), leads to a non working application; however, the inverse order of application of protections is perfectly legal. So, \esp must infer also the order of protections that must be applied to the code, trying to leverage the aforementioned ``amplification effect'' to improve the protected application security level, while illegal sequences of protections must be avoided.

% Finally, there is another side effect of protections that must be considered by \esp. Some protections expose a ``fingerprint'', an introduced code structure or run-time behavior that can be recognized by the attacker, when he or she analyzes the protected binary: thus, an attacker may look for these fingerprints introduced by protections, easily finding the protected assets in code, and thus concentrating its effort on a more limited amount of code. %Examples may be the large \cfg introduced by \cff, or the increased network activity of an application protected against tampering with code mobility (see Section~\ref{sec:background:softProt:antiTamp:codeMobility}). This problem was highlighted by security experts involved in the preliminary design phase of \esp. The solution to this problem adopted in software security companies is obfuscating as much code as possible, applying this protection even on areas of code not sensitive from a security point of view (\ie non-assets), and then executing the application to assess its performances: if the additional obfuscation introduced too much overhead, the cycle is repeated, diminishing the areas of application of the technique and testing again the program: indeed, this is a tiresome manual process, which involves potentially multiple cycles of obfuscation and testing, until assets are hidden from the attacker with acceptable application performances. So, a set of strategies must be devised and implemented in the \esp risk mitigation phase, in order to limit this side effect of protections, finding ways to hide assets and confuse the attacker when he or she analyzes the target program; also, having an automated asset hiding phase would be an appealing plus for software security experts using \esp.

% Summarizing, the \esp risk mitigation phase should propose a comprehensive \emph{protection solution}, an ordered set of protections that must be applied to the application to increase the effort needed by the attacker to implement the threats found in the risk assessment phase; application of each protection must be detailed with the specific assets targeted and the specific automated tool that must be used to enforce the protection, with the values for the parameters requested by the tool. Also, each solution must be associated with a score, indicating its effectiveness in mitigating possible threats, so that solutions can be compared with each other, and a \emph{best solution} can be inferred and suggested to the user.

% \todoAll{peculiarity of software protection for risk mitigation}

\subsection{Risk monitoring}
\label{sec:esp:problem:monitoring}

\begin{enumerate}
\item how to take into account what an attacker can do after that an application is released? (all about remote attestation and software attestation)
\item is penetration testing really necessary?
\item \bdsnote{does one need to track the spread of hacked versions?}
\item \bdsnote{can protections such as watermarking and fingerprinting help?}
\item \bdsnote{does one need to track how potential attackers tools evolve to reassess risks? I think so, because we know that many protections contain hacks that only mitigate certain versions of attacker tools}
\item continuous monitoring?
\item tamper reaction (e.g., for gaming), is a part of monitoring
\end{enumerate}

% Monitoring the risk of software in a \mate scenario means essentially constantly verifying that the application has not been hacked after its distribution: this is indeed a complex matter, involving for example monitoring torrent distribution websites for unauthorized redistribution of the protected software; however, this is a task that goes beyond the scope of this thesis. However, software security companies, prior to distribution of a protected application, test its resilience against possible threats on the fields: \emph{tiger teams}, composed by highly skilled white-hat hackers, execute a \emph{penetration testing} phase \cite{penetrationTesting}, trying to breach the assets security requirements, impersonating a possible attacker. The objective of this phase is assessing the security introduced in the software with the mitigation phase: if attacks carried out in this phase are successful, exposing security flaws overlooked by the chosen mitigations, the appropriate corrective measures are taken, with a new mitigation phase aiming at countering possible attacks found by penetration testers. \esp aims to mimic the security experts methodologies: while a real execution of the attack paths found in the risk mitigation phase as been deemed not feasible, since it would require a way to automatically write scripts driving real attack tools to test the protected application. However, the idea of testing the found solutions with the attack paths found in the risk mitigation phase can be applied to assign a more realistic score to inferred protection solutions: since attack steps must be associated with a probability of success, dependent on the attacker profile and the assets code complexity metrics, and since deploying protections to code increase such metrics, the score of inferred protection solutions can be bound to their effectiveness in reducing the probability for an attacker to succeed in the attack paths found in the risk assessment phase, reflecting \esp main objective, \ie increase the time and effort needed by the attacker to successfully implement its threats against the asset security requirements.

\abnote{peculiarity of software protection for risk monitoring}

\subsection*{Challenges and research questions and why this problem is important}

based on the risk assessment steps in Section~\ref{sec:requisites}:
\begin{itemize}
    \item correctly estimate the risks
    \item correctly estimate the risk mitigation given by the sw protection used
\end{itemize}

\subsubsection*{correctly estimate the risks}
identify the attacks, recognize strategies, model human brain and activities, do it with reasonable performance

trade-off between performance and accuracy (granularity)

model sw application, 

known your asset, know their importance, know how to estimate the overall impact of breaches/attacks, muert-tue

side attacks and strategies, dependencies of code fragments and external libraries (and OS) with the asset, identify pre-targets

do it automatically

developers should known how to crack as well as how to protect the code 

AEG / darpa grand challenge / 

platform where the app is executed may change tutt quand


automatically identify assets, even if it just looks like a dream


\subsubsection*{correctly estimate the risks mitigation}

how to relate the changes operated by protections to attack success probability

how to model the changes to probability of success after application of protections

how to model the impact of protections on the attacker behaviour and available attack paths (e.g., tamper proof vs. obfuscation)

how to evaluate suitable protections

interactions among protections:
how to evaluate synergies and conflicts and side-effects: have valid solutions

impact on performance / overheads and user experience


multiple lines of defence

multiple protections on the same pizz d cod

impact of protections depending on the specific app: relate to some objective something

optimizing is a marginal problem if you have a measure: maybe huge solution space but you have heuristics or whatever non c n futt nudd a nu, vaffammocc a chivemmurtproprie

hide assets as much as you can, even if it will be impossible to perfectly protect

how protections interact with assets (e.g., some protections cannot be applied on certain assets) and on the security requirements

how the protection mitigates depending on the asset and on the whole application, i.e., link some objective measures of the fucking app

\subsubsection*{some functional blahblha implementation etc.}

give answers in limited time

trade-off accuracy vs. completion time: 

\fi

